CAN-D: A Modular Four-Step Pipeline for Comprehensively Decoding Controller Area Network Data

CANs are a broadcast protocol for real-time communication of critical vehicle subsystems. Original equipment manufacturers of passenger vehicles hold secret their mappings of CAN data to vehicle signals, and these definitions vary according to make, model, and year. Without these mappings, the wealth of real-time vehicle information hidden in the CAN packets is uninterpretable, impeding vehicle-related research. Guided by the 4-part CAN signal definition, we present CAN-D (CAN-Decoder), a modular, 4-step pipeline for identifying each signal's boundaries (start bit, length), endianness (byte order), signedness (bit-to-integer encoding), and by leveraging diagnostic standards, augmenting a subset of the extracted signals with physical interpretation. We provide a comprehensive review of the CAN signal reverse engineering research. Previous methods ignore endianness and signedness, rendering them incapable of decoding many standard CAN signal definitions. Incorporating endianness grows the search space from 128 to 4.72E21 signal tokenizations and introduces a web of changing dependencies. We formulate, formally analyze, and provide an efficient solution to an optimization problem, allowing identification of the optimal set of signal boundaries and byte orderings. We provide two novel, state-of-the-art signal boundary classifiers-both superior to previous approaches in precision and recall in three different test scenarios-and the first signedness classification algorithm which exhibits a $>$97\% F-score. CAN-D is the only solution with the potential to extract any CAN signal. In evaluation on 10 vehicles, CAN-D's average $\ell^1$ error is 5x better than all previous methods and exhibits lower ave. error, even when considering only signals that meet prior methods' assumptions. CAN-D is implemented in lightweight hardware, allowing for an OBD-II plugin for real-time in-vehicle CAN decoding.

==> CAN-D IEEE/01-packages.tex <==
% %%% packages:
% \usepackage{graphicx}
\usepackage[dvipsnames]{xcolor}  % Coloured text etc.
\usepackage{subcaption}
% to be able to draw some self-contained figs
\usepackage{tikz,caption}
% to be able to draw captions inside of figs
\usetikzlibrary{calc}
\DeclareCaptionFormat{overlay}{\gdef\capoverlay{#1#2#3\par}}
\DeclareCaptionStyle{overlay}{format=overlay}

% theorems, math symbols, etc: 
\usepackage{amsmath, amsthm, amssymb, mathrsfs}
% \usepackage{mathtools}
\usepackage{tikzsymbols} 

\usepackage[colorlinks=true, linkcolor = blue,
            urlcolor  = blue,
            citecolor = blue,
            anchorcolor = blue]{hyperref}
\usepackage{url} %% clickable links 

\usepackage{lipsum} %% Placeholder text generation 

%% table tools: 
\usepackage{multirow}
\usepackage{multicol}
\usepackage{booktabs}% For formal tables
\usepackage[para,online,flushleft]{threeparttable}

\usepackage{authblk}
\renewcommand\Authand{, }
\renewcommand\Authands{, }

\graphicspath{ {figs/} } % The path where the images that we are using are located
\usepackage{float}

\usepackage[numbers,sort&compress]{natbib} %% so ieeetrans displays citations as [1-5] instead of [1],[2], ...

\usepackage{wrapfig}
\usepackage{enumitem} %% allows specification of the tab size in enumerate, itemize, ... environments 

%reduce space between bib entries
\usepackage{natbib}
\setlength{\bibsep}{8.0pt}

%% custom symbols: 
\newcommand\norm[1]{\left\lVert#1\right\rVert}
\newcommand{\smalltilde}{\raise.17ex\hbox{$\scriptstyle\mathtt{\sim}$}} 
\newcommand{\cupdot}{\mathbin{\mathaccent\cdot\cup}} %% disjoint union, inline

% \usepackage[ruled]{algorithm}
% \usepackage[noend]{algpseudocode}
% \makeatletter
% \renewcommand{\ALG@beginalgorithmic}{\small}

\usepackage[ruled,vlined]{algorithm2e}
\SetAlFnt{\small}
\SetAlCapFnt{\small}
\SetAlCapNameFnt{\small}

% \setlength{\abovedisplayskip}{0pt}
% \setlength{\belowdisplayskip}{0pt}

% \usepackage{cleveref} %% includes name of reference, i.e. "lemma" 1.1 or "theorem" 2.3

\usepackage{caption}
\usepackage{subcaption}
\captionsetup{font=small} %% makes captions not look like part of the paper's prose and saves space
% \captionsetup[sub]{font=footnotesize}
\captionsetup[sub]{font=small}
\setlength{\abovecaptionskip}{1.5pt}
\setlength{\belowcaptionskip}{2.5pt}

\setlength{\textfloatsep}{0.1cm}%Try to reduce space after tables/figures 
\setlength{\intextsep}{.7\baselineskip}%Try to reduce space after tables/figures 
\setlength{\parskip}{1.5pt}
\newcommand{\squeezeup}{\vspace{-2mm}} % for after wraptable w/ no caption. 

% \usepackage{todonotes}
\usepackage{xargs}                      % Use more than one optional parameter in a new commands


\usepackage[colorinlistoftodos,prependcaption, textsize=small]{todonotes}
\newcommandx{\unsure}[2][1=]{\todo[disable, inline,linecolor=red,backgroundcolor=red!25,bordercolor=red,#1]{#2}}
\newcommandx{\add}[2][1=]{\todo[disable, inline,linecolor=green,backgroundcolor=green!25,bordercolor=green,#1]{#2}}
\newcommandx{\fix}[2][1=]{\todo[disable, inline,linecolor=blue,backgroundcolor=blue!25,bordercolor=blue,#1]{#2}}
% \newcommandx{\thiswillnotshow}[2][1=]{\todo[disable,#1]{#2}}


\usepackage{enumitem} %% allows specification of the tab size in enumerate, itemize, ... environments 

% \usepackage{paralist} %% needed for compact itemize
% to define compact enumerate/itemize and w/ nicer bullets: 
\newenvironment{enumeratesqueeze}%
  {\begin{enumerate}%
    leftmargin = *
    \setlength{\itemsep}{0pt}%
    \setlength{\parskip}{0pt}}%
  {\end{enumerate}}
  

% \definecolor{BurntSienna}{rgb}{0.91, 0.45, 0.32}


\newcommand{\I}{\mathcal{I}}


\newtheorem{example}{Example} %% creates example envrionment. 

\newtheorem{prop}{Proposition}
\newtheorem{thm}{Theorem}
\newtheorem{cor}{Corollary}
\newtheorem{lem}{Lemma}
\newtheorem{defn}{Definition}
\newtheorem{rmk}{Remark}



\usepackage{wasysym}

%% dashed midrule magic maneuver: 
\usepackage{arydshln}

\makeatletter
\def\adl@drawiv#1#2#3{%
        \hskip.5\tabcolsep
        \xleaders#3{#2.5\@tempdimb #1{1}#2.5\@tempdimb}%
                #2\z@ plus1fil minus1fil\relax
        \hskip.5\tabcolsep}
\newcommand{\cdashlinelr}[1]{%
  \noalign{\vskip\aboverulesep
           \global\let\@dashdrawstore\adl@draw
           \global\let\adl@draw\adl@drawiv}
  \cdashline{#1}
  \noalign{\global\let\adl@draw\@dashdrawstore
           \vskip\belowrulesep}}
\makeatother

\definecolor{brightgreen}{rgb}{0.4, 1.0, 0.0}


\setlength{\bibsep}{1pt plus .9ex}

%for making compact comparison table
\usepackage{wasysym}

\usepackage{adjustbox}
\usepackage{array}

\newcommand*{\full}{\CIRCLE}
\newcommand*{\prt}{\LEFTcircle}
\newcommand*{\none}{\Circle}
\newcommand*{\na}{}

\newcommand*{\setuptable}{
	\renewcommand{\arraystretch}{1.1}
	\setlength{\arrayrulewidth}{0.1em}
	\setlength\tabcolsep{3.75pt}
	\centering
}
\newcommand*\rot{\rotatebox{90}}
\newcommand*{\headrow}[1]{\multicolumn{1}{c}{\adjustbox{angle=35,lap=\width-0.5em}{#1}}}
\newcommand*{\headline}[1][3cm]{\adjustbox{angle=35,lap=\width-.3mm}{\rule{#1}{0.075em}}}
\newcommand{\hc}{\cellcolor[gray]{1}}
\newcommand*{\headcol}[2]{\multirow{#1}{*}{\rot{#2}}}

\usepackage{xhfill}

\usepackage{framed}

%make sure qed square appears onlast line of proof
\newenvironment{myproof}[1][\proofname]{%
  \begin{proof}[#1]$ $\nobreak\ignorespaces
}{%
  \end{proof}
}

\usepackage{microtype}

==> CAN-D IEEE/02-title.tex <==
 

% \title{Automotove CAN Tokenization \& Translation (ACTT) 2.0
% \thanks{\scriptsize{This manuscript has been co-authored by UT-Battelle, LLC, under contract DE-AC05-00OR22725 with the US Department of Energy (DOE). The US government retains and the publisher, by accepting the article for publication, acknowledges that the US government retains a nonexclusive, paid-up, irrevocable, worldwide license to publish or reproduce the published form of this manuscript, or allow others to do so, for US government purposes. DOE will provide public access to these results of federally sponsored research in accordance with the DOE Public Access Plan (http://energy.gov/downloads/doe-public-access-plan).}}}
% \author{
%     \IEEEauthorblockN{Miki E. Verma\IEEEauthorrefmark{1}, Jordan J. Sosnowski\IEEEauthorrefmark{2}, Robert A. Bridges\IEEEauthorrefmark{1}, Samuel C. Hollifield\IEEEauthorrefmark{1}}
%     \IEEEauthorblockA{\normalsize{\IEEEauthorrefmark{1} Cyber \& Applied Data Analytics Division, Oak Ridge National Laboratory, Oak Ridge, TN} 
%     \\{\normalsize{\{vermake, bridgesra,hollifieldsc \}@ornl.gov}}}
%     \IEEEauthorblockA{\normalsize{\IEEEauthorrefmark{2}Department of Computer Science and Software Engineering, Auburn University}
%     \\{\normalsize{jjs@auburn.edu}}}
% }


% \date{\today}


%don't want date printed
\date{}

% make title bold and 14 pt font (Latex default is non-bold, 16 pt)
\title{\LARGE \bf CAN-D: A Modular Four-Step Pipeline for Comprehensively Decoding Controller Area Network Data
\thanks{\small{%ACTT 2.0 is an equal endian employer. 
%Organizational legal disclaimer redacted.
Copyright (c) 2015 IEEE. Personal use of this material is permitted. However, permission to use this material for any other purposes must be obtained from the IEEE by sending a request to \href{mailto:pubs-permissions@ieee.org}{pubs-permissions@ieee.org}.
This manuscript has been co-authored by UT-Battelle, LLC, under contract DE-AC05-00OR22725 with the US Department of Energy (DOE). The US government retains and the publisher, by accepting the article for publication, acknowledges that the US government retains a nonexclusive, paid-up, irrevocable, worldwide license to publish or reproduce the published form of this manuscript, or allow others to do so, for US government purposes. DOE will provide public access to these results of federally sponsored research in accordance with the DOE Public Access Plan (\url{http://energy.gov/downloads/doe-public-access-plan}).
}}}

% \author{
% % {\rm Author names redacted}\\
% % Author affiliations redacted }
% \def\andname{,} 
% \author[1]{Miki E. Verma}
% \author[1]{Robert A. Bridges}
% \author[2]{Jordan J. Sosnowski}
% \author[1]{Samuel C. Hollifield}
% \author[1]{Michael D. Iannacone}
% \affil[1]{\textit{Cyber \& Applied Data Analytics Division, Oak Ridge National Laboratory, Oak Ridge, TN}\\

% \textit{\{vermake, bridgesra, hollifieldsc, iannaconemd\}@ornl.gov}}

% \affil[2]{\textit{Department of Computer Science \& Software Engineering, Auburn University}\\

% \textit{jjs0029@auburn.edu}}
% }


\author{
    % {\rm Author names redacted}\\
    % Author affiliations redacted 
    \IEEEauthorblockN{
    Miki E. Verma\IEEEauthorrefmark{1}, 
    Robert A. Bridges\IEEEauthorrefmark{1}, 
    Jordan J. Sosnowski\IEEEauthorrefmark{2}, 
    Samuel C. Hollifield\IEEEauthorrefmark{1}, 
    Michael D. Iannacone\IEEEauthorrefmark{1}} \\
    \IEEEauthorblockA{\IEEEauthorrefmark{1}\small Cyber \& Applied Data Analytics Division, Oak Ridge National Laboratory, Oak Ridge, TN
    \\\{vermake, bridgesra, hollifieldsc, iannaconemd\}@ornl.gov} \\
    \IEEEauthorblockA{\IEEEauthorrefmark{2}Department of Computer Science \& Software Engineering, Auburn University
    \\jjs0029@auburn.edu}
}




==> CAN-D IEEE/03-abstract.tex <==
\begin{abstract}
Controller area networks (CANs) are a broadcast protocol for real-time communication of critical vehicle subsystems. 
Original equipment manufacturers of passenger vehicles hold secret their mappings of CAN data to vehicle signals, and these definitions vary according to make, model, and year.  
Without these mappings, the wealth of real-time vehicle information hidden in the CAN packets is uninterpretable, severely impeding vehicle-related research, including CAN cybersecurity and privacy studies, aftermarket tuning, efficiency and performance monitoring, and fault diagnosis to name a few. 

Guided by the four-part CAN signal definition, we present CAN-D (CAN-Decoder), a modular, four-step pipeline for identifying each signal's boundaries (start bit and length), endianness (byte ordering),  signedness (bit-to-integer encoding), and by leveraging diagnostic standards, augmenting a subset of the extracted signals with meaningful, physical interpretation. 
En route to CAN-D, we provide a comprehensive review of the CAN signal reverse engineering research.
All previous methods ignore endianness and signedness, rendering them incapable of decoding many standard CAN signal definitions. 
Incorporating endianness grows the search space from 128 to 4.72E21 signal tokenizations and introduces  a  web  of  changing dependencies. 
In response, we formulate, formally analyze, and provide an efficient solution to an optimization problem, allowing identification of the optimal set of signal boundaries and byte orderings. 
In addition, we provide two novel, state-of-the-art signal boundary classifiers---both of which are superior to previous approaches in precision and recall in three different test scenarios---and the first signedness classification algorithm, which exhibits a $>$ 97\% F-score. 
Overall, CAN-D is the only solution with the potential to extract any CAN signal that is also the state of the art. 
In evaluation on 10 vehicles of different makes, CAN-D's average $\ell^1$ error is five times better (81\% less) than all previous methods and exhibits lower average error, even when considering only signals that meet prior methods' assumptions. 
Finally, CAN-D is implemented in lightweight hardware, allowing for an on-board diagnostic (OBD-II) plugin for real-time in-vehicle CAN decoding. 
\end{abstract}

% allowing accurate conversion of CAN data into multi-variate time series (tokenization). 
%is the only method to accommodate big and little endianness as well as signed and unsigned encodings\textemdash thus it

==> CAN-D IEEE/10-intro.tex <==

\begin{figure}[!b]
   \centering
    \includegraphics[width=.5\textwidth]{figs/cand_pipeline_detail_vertical.pdf}
    \caption{CAN-D Pipeline: A four-step modular pipeline that takes a CAN log (capture of CAN data) as input and outputs a DBC with signal definitions, thus providing vehicle-agnostic CAN signal reverse engineering. Italicized processes outlined in dotted red lines indicate modular pieces that can be any algorithm that satisfies the input/output requirements. Descriptions of our choices for these pieces are provided. Greek letters $\alpha$--$\delta$ denote tuning parameters (possibly) needed for Steps $1$--$4$, respectively.}
    \label{fig:pipeline}
\vspace{-.6cm}
\end{figure}

\section{Introduction \& Background}
\label{sec:intro}
\vspace{-.2cm}
Modern automobiles rely on communication of several electronic control units (ECUs) (internal computers) over a few controller area networks (CANs) and adhere to a fixed CAN protocol. 
Sensors readings, such as accelerator pedal angle, brakes, fuel injection timing, wheel speeds---as well as less important readings, such as radio settings---are all communicated as signals encoded in the CAN messages.  
For passenger vehicles, the encodings of these signals into CAN messages are proprietary: one can monitor (and send) CAN messages but generally cannot understand their meaning. 
Furthermore, these encodings vary by make, model, year, and even trim, and in practice, reverse engineering of signals is currently a tedious, per-vehicle effort. 
Because CAN data is sent at a rapid rate and carries a wide variety of real-time vehicle information, a vehicle-agnostic solution for decoding CAN signals promises a vast resource of streaming, up-to-date information for analytics and technology development on any vehicle.\looseness=-1

Each CAN message has up to 64 bits of data containing (usually) multiple signals (Fig. \ref{fig:dbc_editors}).  
Automotive CAN signals are characterized by four defining properties (discussed in detail in Section \ref{sec:can-basics}): (1) signal boundaries (start/end bit), (2) endianness (byte order), (3) signedness (bit-to-integer encoding), and (4) physical interpretation. The signal definitions for each message (a message definition) are defined in a vehicle's CAN database file (the industry standard is Vector's \texttt{.dbc} or ``DBC'' file format). We use this industry-standard, four-part signal definition to frame our understanding of previous works and guide our approach. 
\textit{The goal is a vehicle-agnostic CAN decoder that can discover these four defining properties for each signal from CAN data from any vehicle---that is, to reverse engineer the signal definitions in the vehicle's DBC. }\looseness=-1


Recently, the research community has focused on reverse engineering signals from automotive CAN data. This research is summarized in Section \ref{sec:related-works}, and Table \ref{tab:related-works} catalogs each work's efforts to identify the four defining signal characteristics.
Notably, all current approaches focus only on identifying signal boundaries (1)
% with simple heuristics 
and/or matching signals to observable sensor data (4), while ignoring endianness (2) and signedness (3), meaning they are unable to decode many standard CAN signals.
% In short, they simply do not apply to much CAN data in use. 
% Furthermore, extending current approaches to incorporate these schemes is not possible as their methods rely on this oversimplifying assumption. 


% \begin{table*}[]
% \centering
% \caption{Automotive CAN signal reverse engineering algorithms for each of the four signal properties. CAN-D is the only comprehensive algorithm that determines all four properties.}
% \label{tab:related-works}
% \begin{threeparttable}
% \begin{tabular}{lcccc}
% \toprule
%  & \textbf{Signal Boundary} & \textbf{Endianness } & \textbf{Signedness } & \textbf{Interpretation} \\ 
%  \cmidrule{2-5}
% Huybrechts et al. \cite{huybrechts2017automatic} & \Circle  & \Circle & \Circle & 
%  RMS error, machine learning \\
%  Markowitz \& Wool \cite{markovitz2017field} & unsupervised optimization & \Circle  & \Circle  & \Circle  \\
%  Nolan et al.'s \textbf{TANG} \cite{nolan2018unsupervised} & unsupervised heuristic & \Circle  & \Circle & \Circle \\ 
% Marchetti \& Stabili's \textbf{READ}  \cite{marchetti2019read} & unsupervised heuristic & \Circle & \Circle & \Circle  \\
% Verma et al.'s \textbf{ACTT} \cite{verma2018actt} & grid search  & \Circle & \Circle & sensor matching, regression \\
% Pes\'{e} et al. \textbf{LibreCAN} \cite{Pese2019librecan} & unsupervised heuristic & \Circle & \Circle & sensor matching, cross correlation\\
% Young et al. \cite{young2020towards} & \Circle & \Circle & \Circle & \\
% \cdashlinelr{1-5}
% \multirow{2}{*}{\textbf{CAN-D}} & supervised learning  & \multirow{2}{*}{custom optimization} & \multirow{2}{*}{unsupervised heuristic} & \multirow{2}{*}{sensor matching, regression} 
% \\
%     & or unsupervised heuristic &&&\\
% \bottomrule
% \end{tabular}
% \end{threeparttable}
% \vspace{-.5cm}
% \end{table*}

All previous works have developed and tested algorithms on limited CAN data, often from a single make. 
Targeting a vehicle-agnostic solution, we compile a much more varied collection of labeled CAN data from 10 different makes (see Section \ref{sec:dataset}). 
Equipped with this robust, labeled dataset for development and testing, we pursue the first comprehensive and most accurate signal reverse engineering pipeline (see Fig. \ref{fig:pipeline}). 
Before describing our contributions, we introduce necessary background information. 






==> CAN-D IEEE/12-can-basics.tex <==
\begin{figure}[hb]
    % \vspace{-.2cm}
    \includegraphics[width=.48\textwidth]{figs/CAN_Frame.pdf}
    \caption{
       CAN 2.0 frame depicted: Arbitration ID indexes the frame; Data Field  carries message content up to 64 bits.
        }
    \label{fig:CANframe}
    \vspace{-.76cm}
    \end{figure}  

\subsection{CAN Fundamentals \& Notation}
\label{sec:can-basics}
CAN 2.0 defines the physical and data link layers (Open Systems Interconnection [OSI] layers 1 and 2) of a broadcast protocol \cite{bosch1991can}. 
In particular, it specifies the standardized  CAN frame (or packet) format represented in Fig. \ref{fig:CANframe}.  
For semantic understanding of a CAN frame, only two components of the frame are necessary:
\begin{itemize}[leftmargin = *,topsep=3pt,itemsep=2pt,parsep=2pt]
\item \textit{Arbitration ID}, an 11-bit header  used to identify the frame and  %at the physical layer, 
for arbitration (determining frame priority when multiple ECUs concurrently transmit)
\item \textit{Data Field} or \textit{Message}, up to 64 bits of content
\end{itemize}
Each ID's data field comprises signals of varying lengths and encoding schemes packed into the 64 bits (Fig. \ref{fig:dbc_editors}). 
A \texttt{.dbc} file (standard file type) provides the definitions of signals in the data field for each ID, thus defining each CAN Message. 


% \subsubsection{CAN Messages} 
CAN frames with the same ID are usually sent with a fixed frequency to communicate updated signal values, although some are triggered by an event (e.g., ID \texttt{0x3A2} occurs every 0.1 s, ID \texttt{0x45D} occurs every 0.25 s). 
We partition CAN logs into \textit{ID traces},  the time series of 64-bit messages for each ID. 
An ID trace is denoted  by
$[ B_0(t) \dots, B_{63}(t) ]_t$, a time-varying binary vector of length 64. 
%, and  $B_i^{id}(t)$  dons its ID index, $id$,  when multiple ID traces are considered. 
We assume each message is 64 bits by padding with 0 bits if necessary. 


\subsubsection{Byte Order (Endianness) and Bit Order} The significance of a signal's bits within a byte (contiguous 8-bit subsequences) decreases from left to right: the first bit transmitted is the most significant bit (MSB), and the last (eighth) bit is the least significant bit (LSB).
This is defined in the CAN Specification \cite{bosch1991can, provencher2012controller} but has been misrepresented \cite{Pese2019librecan} and misunderstood  \cite{nolan2018unsupervised, verma2018actt} by previous signal reverse engineering works. 
The confusion results from use of both big endian and little endian \textit{byte} orderings in CAN messages. Big endian (B.E.) indicates that the significance of bytes decreases from left to right; whereas
little endian (L.E.) reverses the order of the bytes, but maintains the order of the bits in each byte.
%\cite{endianness}.
For clarity, we list the bit orderings for a 64-bit data field under both endiannesses, and parentheses demarcate the bytes \cite{provencher2012controller}: 
\begin{equation} 
    \begin{aligned} 
    \label{eq:bit-orderings} 
    \hspace{-.25cm} \text{B.E.: }  & (B_{0\phantom{5}}, \dots, B_{7\phantom{5}}), (B_{8\phantom{5}} \dots, B_{15}), \dots , (B_{56}, \dots, B_{63})\\
    \hspace{-.25cm} \text{L.E.: }  & (B_{56}, \dots, B_{63}), (B_{48}, \dots, B_{55}), \dots , (B_{0\phantom{1}}, \dots, B_{7\phantom{1}}) 
    \end{aligned} 
\end{equation} 
% See Examples \ref{ex:big-lil-endian} \& \ref{ex:boundary} for how this affects signal definitions. 

% \begin{figure}[b]
%     \centering
%     \begin{subfigure}[t]{0.275\textwidth}
%         \centering
%       \includegraphics[width=\textwidth]{figs/dbc_layout_eg_small.pdf}
%     \end{subfigure}%
%     \begin{subfigure}[t]{0.225\textwidth}
%         \centering
%       \includegraphics[width=\textwidth]{figs/can_programming_gui_eg.pdf}
%     \end{subfigure}
%     \caption{DBCs visualized through DBC Editor GUIs. \textbf{Left:} A \textit{signal layout plot} visually represents a CAN Message tokenization, depicting an ID's 64-bit data field as an $8\times8$ array containing CAN Signal(s). Each signal's constituent bits are shown in a unique color and unused bits are shown in white. (\textit{CANdb++} Database Editor) \cite{hackaday} \textbf{Right:} Signal definition of first 16-bit \textcolor{Dandelion}{\textbf{yellow}} signal, defined by properties as follows: start bit, length, signedness, endianness, scaling factor, offset, unit. (\textit{NI-XNET Database Editor}) \cite{signal_api} }
%     \label{fig:dbc_editors}
% \end{figure}


\begin{figure}[t]
\vspace{-.3cm}
    \centering
      \includegraphics[width=.48\textwidth]{figs/DBC.pdf}
    \caption{A \textit{signal layout plot} represents a CAN message tokenization, depicting an ID's 64-bit data field as an $8\times8$ array containing CAN signal(s). Each signal's constituent bits are shown in a unique color, and unused bits are shown in white. This representation is similar to visualizations that would be provided by DBC editing software.}
    %The signal definition of first 16-bit \textcolor{Orchid}{\textbf{lavender}} signal is defined as follows: start bit (0), length (16), signedness (unsigned), endianness (big), scaling factor (1/65), offset (0), unit (RPM).}
    \label{fig:dbc_editors}
\end{figure}

\subsubsection{CAN Signals} The specifications for decoding each ID's message into a set of signal values is defined by the original equipment manufacturer (OEM) and held secret. The \texttt{.dbc}  format furnishes the components required to define a CAN signal. Below, the bullet and text colors match those of Fig. \ref{fig:pipeline}.   
\begin{itemize}[leftmargin = *,topsep=3pt,itemsep=1pt,parsep=2pt]
    \item[\textcolor{Plum}{\textbullet}] \textbf{Start bit} and \textbf{length} indicate signal position in the data field.
    \item [\textcolor{Plum}{\textbullet}] \textbf{Byte ordering}: If the signal crosses a byte boundary, \textit{little endian} signals reverse the order of the bytes, whereas \textit{big endian} signals retain byte order (see Eq. \ref{eq:bit-orderings}).
    \item[\textcolor{SeaGreen}{\textbullet}]  \textbf{Signedness}: \textit{Unsigned}, the usual base 2 encoding, vs. \textit{signed}, two's complement encoding \cite{2s-complement}.
    \item[\textcolor{RoyalBlue}{\textbullet}] \textbf{Label} and \textbf{unit} give the physical meaning of the signal and its units (e.g., speed in mph). 
    \item[\textcolor{RoyalBlue}{\textbullet}] \textbf{Scale} and \textbf{offset} provide the linear mapping of the signal's tokenized values to the appropriate units. 
\end{itemize} 
%  It is implicit in the DBC signal definition that (non-constant) signals are contiguous sequences of non-constant bits. 

 The above definitional components provide the required learning tasks  for reverse engineering signal definitions. %Use colors and regard \ref{fig:pipeline} to match CAN-D's pipeline and signal definitional components to terms below. 
\begin{itemize}[leftmargin = *,topsep=3pt,itemsep=1pt,parsep=2pt]
\item \textit{\textcolor{Plum}{\textbf{Tokenization}}}: Learning signals' constituent bits (start bit, length) and byte orders (endianness)---Steps 1 and 2. % and provides the start bit, length and endianness parts of the signal definition. 
\item \textit{\textcolor{SeaGreen}{\textbf{Translation}}}: Converting a signal's sequence of bits to integers (signedness)--- Step 3. % and provides the signedness component of the signal definition. 
\item \textcolor{RoyalBlue}{\textit{\textbf{Interpretation}}}: Linearly mapping (scale, offset) a translated signal to a meaningful measurement (label, unit)---Step 4.% and provides the label, unit, scale, and offset components of the signal definition.  
\end{itemize}

% (Our goal is to reverse engineer the signal definitions (DBC) for any vehicle from ambient CAN data from that vehicle.) 

% \begin{figure}
%     \centering
%     \includegraphics[width=.48\textwidth]{figs/can_programming_gui_eg.png}
%     \caption{NI-XNET CAN interface for programming signals \cite{signal_api} }
%     \label{fig:gui}
% \end{figure}

\begin{example}
\label{ex:big-lil-endian} 
Consider in Fig. \ref{fig:dbc_editors} the first two-byte \textcolor{Orchid}{\textbf{lavender}}  signal.
To tokenize the signal, or know its sequence (implying order) of bits, we must know endianness. 
If bytes 1 \& 2 are big endian, we obtain MSB-to-LSB bit indices, $I = (0, \dots, 15)$ whereas if they are little endian, the bytes are swapped, obtaining MSB-to-LSB bit indices $I = (8, \dots, 15, 0, \dots, 7)$, notably with $B_{15}\to B_0$.
Next, the signal's signedness furnishes the translation of that bit sequence to an integer. 
The information needed for interpretation is the label and unit of the signal (in this case, engine rpm) and the linear transformation to convert the translated values (a two-byte signal can take $ 2^{16}-1 = 65,535$ values) to the appropriate physical value (e.g., in the $0$--$10,000$ rpm range). 
\end{example}

Fig. \ref{fig:qual_compare_paylods_signals}
%illustrates signals that have been correctly and incorrectly decoded. 
illustrates time series of CAN data that have been decoded using both correct and incorrect signal definitions.
%and demonstrates how noisy an incorrectly decoded signal can be.
Fig. \ref{fig:qual_compare_paylods_signals}(a) plots \textcolor{green}{\textbf{green}} and \textcolor{cyan}{\textbf{blue}} CAN signals tokenized with correct (middle) vs. incorrect (right) signedness, and
Fig. \ref{fig:qual_compare_paylods_signals}(b) plots CAN signals tokenized with correct (top) vs. incorrect (bottom, and in particular, the \textcolor{MidnightBlue}{\textbf{navy}} signal) endianness. The clear discontinuities in these mistokenized and mistranslated signals demonstrate the importance of knowing the endianness and signedness for extracting meaningful time series. 

% Understanding endianness and encoding is essential for meaningful signal extraction, e.g., see Fig. \ref{fig:qual_compare_paylods_signals}.  
% The consequences of misunderstanding this are illustrated in Fig. \ref{fig:qual_compare_paylods_signals}, where we show plots of correctly (bottom) and incorrectly (top) parsed signals with little endian (left), signed (middle) and both little endian and signed (right) encodings. 
%The consequences of a failure to identify little endian and signed signals are illustrated in \ref{fig:qual_compare_paylods_signals}, where we show plots of correctly (bottom) and incorrectly (bottom) parsed signal time series. 
% ACTT 2.0 is the only work that provides this capability. 





% \subsubsection{Unified Diagnostic Services} 
\subsubsection{On-Board Diagnostics} 
\label{sec:dids} 
% data. J1979: subset of info is required for emmissions testing. Backdoor approach, but utilizes data that exists on all cars from x year range and does not require bringing together multimodal streams collected on different devices: 
% - UDS interrogation gives direct access to vehicle states, 
In the United States, all vehicles sold after 1996 include an on-board diagnostic (OBD-II) port, which generally allows for open access to automotive CANs, and emissions-producing vehicles sold after 2007 also include a mandatory, standard interrogation schema for extracting diagnostic data using the J1979 standard \cite{J1979_201702}. 
This OBD service  is an application layer protocol by which one can query diagnostic data from the vehicle  by sending a CAN frame. 
A CAN response is broadcasted 
%ECUs (electronic control units, the compute nodes on the CAN) broadcast one or more response frames, 
with the requested vehicular state information. 
There is a standard set of possible queries available via this call--response protocol (e.g, accelerator pedal position, intake air temperature, vehicle speed), along with unit conversions, each corresponding to a unique diagnostic  OBD-II PID (DID). 
%\cite{obd2pids}. 
Specific examples of how to perform the call and response are available \cite{smith_2016, Pese2019librecan}. 
Previous CAN decoding works have iteratively sent DID requests
%(at an appropriate rate to not overwhelm the bus), 
and parsed the responses from CAN traffic to capture valuable, real-time, labeled vehicle data without using external sensors \cite{huybrechts2017automatic, verma2018actt, Pese2019librecan}.  
$D(t)$ denotes these time series of diagnostic responses, or \textit{DID traces}. 
Inherent limitations exist: the set of available DIDs varies per make, and electric vehicles need not conform to this standard \cite{verma2018actt, Pese2019librecan}. 
 
 
 % \begin{wrapfigure}[17]{r}{.25\textwidth}
% \vspace{-.1cm}
%     \centering
%     \includegraphics[width=.25\textwidth]{figs/dbc_layout_eg_small.pdf}
%     \caption{A signal layout plot, generated by DBC editor \textit{CANdb++}, depicts an ID's 64-bit data field as an $8\times 8$ array \cite{hackaday}. 
%     Each signal's constituent bits are shown in a unique color and unused bits are shown in white. 
%     E.g., the first 16 bits encodes an RPM signal (\textcolor{Dandelion}{\textbf{dandelion-colored}}), next 5 bits encode a speed signal (\textcolor{NavyBlue}{\textbf{navy}}), etc. }
%     \label{fig:dbc_eg_layout}
% \end{wrapfigure}

==> CAN-D IEEE/14-problem.tex <==
\vspace{-.2cm}
\subsection{Problem, Assumptions, and Challenges}
\label{sec:problem} 
\subsubsection{Problem}
The goal is to  to recreate the \texttt{.dbc} file's signal definitions (i.e., discover the four properties for each signal) from a sufficient capture of a vehicle's CAN data, for any vehicle. 
% Following Sec. \ref{sec:can-basics}, the problem is to (1)
% \textcolor{Plum}{\textit{tokenize}}\textemdash learn each signal's ordered sequence of bits (start bit, length, and  endianness), 
% (2) \textcolor{SeaGreen}{\textit{translate}}\textemdash  identify signedness, 
% and (3) \textcolor{RoyalBlue}{\textit{interpret}}\textemdash
% determine the linear transformation (scale factor and offset) converting the translated integers into physically meaningful values, and label the signal with units (e.g., speed in MPH).

\subsubsection{Assumptions} 
We make five fundamental assumptions: 
% \begin{wrapfigure}[11]{l}{.25\textwidth}
% \vspace{-.25cm}
%     \centering
%     \includegraphics[width=.25\textwidth]{figs/can_programming_gui_eg_2.png}
%     \caption{NI-XNET CAN interface for programming signals \cite{signal_api} }
%     \label{fig:gui}
% \end{wrapfigure}
\textbf{(A0)} Observed constant bits are unused.\\ 
\textbf{(A1)} Both  big and little endian byte orders are possible.
%(\texttt{.dbc} use \texttt{0}/\texttt{1} to indicate big/little endian, respectively). \\
%Note that both  big and little  endian signals occur. \\
\textbf{(A1.a)} Both endiannesses can occur in a single ID.  
We have not observed this, but it is permitted by protocol and DBC syntax. DBC editor GUIs allow per-signal endianness specification with a checkbox or pull-down menu, implying that both byte orderings can co-occur in a message. \\
\textbf{(A1.b)} A single byte cannot have  bits used in a little endian signal while also containing bits used in a big endian signal; otherwise, the byte orders indicated by the  signals are contradictory.\\
\textbf{(A2)} Signed signals are possible and are encoded using a two's complement encoding. 
% (DBCs use \texttt{+}/\texttt{-} to indicate unsigned/signed, respectively).




\subsubsection{Challenges} 
In practice, it is difficult to exercise the MSBs of a signal, resulting in errors in determining signal boundaries (a Step 1 challenge). 
For example, consider the two-byte (16-bit) engine rpm signal in Example \ref{ex:big-lil-endian} with translated values of $0$--$10,000$.
As 5,000 rpm is rarely reached, the MSB of this signal is likely to be observed as a constant 0 bit, causing the signal start bit to be mislabeled. 
% Similarly,, if 2,500 RPM is not surpassed implies the top two MSBs will be constant 0s. 
Though this challenge is easily surmountable for engine rpm (e.g., rev engine in neutral during collection), it is far more difficult to solve this for latent sensors, (e.g, engine temperature). 

Secondly, because continuous signals are sampled periodically, those with high-resolution signals (e.g., a two-byte signal has $2^16 > 65,000$ values) have LSBs flipping seemingly randomly (a Step 1 challenge). 
Our results indicate that the TANG algorithm \cite{nolan2018unsupervised} suffers from the overly strict assumption that flip frequencies decrease monotonically with bit significance. 
%that assuming the negative correlation between bit significance and flip frequencies (LSBs flip more than others) too strictly. 


Thirdly, considering both big and little endianness greatly increases the complexity of the problem: bits on the byte boundaries have unknown neighbors (albeit in a fixed set of possibilities). For example, simply comparing the bit flip probabilities of neighboring bits now requires custom rules that incorporate all possible neighbors according to  \textbf{(A1)} and \textbf{(A1.a)} given the constraints imposed by \textbf{(A1.b)} (a Step 2 challenge). 
% See  details in Sec. \ref{sec:endianess_opt}. 

Fourthly, considering both signed and unsigned encodings adds another hurdle. In particular, the order of bit representations mod $2^n$ is the same for both signed and unsigned encodings: half the bit strings represent different integers (a Step 3 challenge). 

Finally, many CAN signals communicate sensor values that are hard to measure with external sensors. Therefore, identifying the physical meaning, the unit and the linear mapping (scale and offset) can be difficult (a Step 4 challenge). 








%Note that unlike with the endianness assumption, the assumption of normal unsigned encoding does not appear to break the tokenization schemes put forth by \cite{marchetti2019read}\cite{Pese2019librecan}. 



% \add{Explain why we make this assumption and shortcomings: It is imperative that we capture CAN data that encompasses all of the vehicles functionality so that all the bits are being exercised in their defined signals. If not, some signals' most significant bits may not change and seem to appear constant, and get discarded mistakenly. }


%We make several fundamental assumptions, about the nature of signals and how they are encoded that differentiate our method from the existing methods in this area. Some of these assumptions are 
% some dictated by the CAN protocol, while others are based on our experience working with CAN data.
% and based on what is feasible given the limitations of the data. 
% Notably, there are implicit and unfounded assumptions made by other methods that we do not make, allowing our algorithm to be more robust. 

% (Endianness): The significance of bytes within a signal can be either Big Endian (Motorola), meaning the bytes are transmitted from least significant to most significant, or Little Endian (Intel), meaning the bytes are transmitted from least significant to most significant. All of the existing methods assume a fixed byte order (Big Endian), and thus, would necessarily split Little Endian signals along byte boundaries (see \ref{sec:eval-compare}). 

%based on our observation of data and examination of crowdsourced DBCs\cite{comma_opendbc}, it is very rare to have  
% \add{Need to motivate why the lengths gone to in step 2 are necessary considering we've never seen mixed endianness in the wild..maybe with the fact that programming is often done in a GUI where its just a box to check little endian, so programmers could easily do this without thinking?} 
% Fixed Signal Endianness within a Byte: 



    
    
%  Signal Continuity: \add{@bobbyb add something about how we use this assumption in building features, and how this relates to the different categories of signals explained in Intro. Also, perhaps the contiguous non-constant bits is just an extension of this?}



==> CAN-D IEEE/15-contributions.tex <==
\vspace{-.2cm}
\subsection{Contributions} 
We make six contributions to the area of automotive CAN signal reverse engineering. 

\textbf{C1. Comprehensive signal reverse engineering pipeline} Our primary contribution is a modular, four-part pipeline, depicted in Fig. \ref{fig:pipeline},  for learning all four components of a CAN signal definition. 
The pipeline is modular in that 
Step 1 can accommodate any signal boundary classification method,
Step 3 can accommodate any signedness classification algorithm,
%for determining if signed or unsigned encoding is used;  
and Step 4 can accommodate any signal-to-time-series matching algorithm for physical interpretation. 
Instantiating our pipeline with our signal boundary classification heuristic and (separately) our trained machine learning (ML) classifier for Step 1 and the diagnostic sensor matching of Verma et al. \cite{verma2018actt} for Step 4, we present a quantitative comparative evaluation of our signal reverse engineering pipeline vs. previous methods. 
We demonstrate that CAN-D exhibits less than a fifth of the average error exhibited by all previous methods (Section \ref{sec:eval-l1-error} and Table \ref{tb:compare}, bottom), and we qualitatively illustrate the pitfalls and limitations of previous methods (Section \ref{sec:qual_results} and Fig. \ref{fig:qual_compare_paylods_signals}) that our four-step pipeline circumvents. 
\textit{Overall, CAN-D is the first CAN signal reverse engineering effort that can accommodate all signals as defined in automotive DBC files, and it is far more accurate than any previous effort. Furthermore, it provides a framework for future research developments to improve and plug in advancements to each step.}

\textbf{C2. Introduction of two state-of-the-art signal boundary classification algorithms and comparative study of previous algorithms} 
We develop two signal boundary classifiers, a supervised machine learning model, and an unsupervised heuristic (Section \ref{sec:cutprob}). We implement the previous state-of-the-art classification methods % all of which are unsupervised heuristics, 
and provide the first quantitative comparison of all methods (Section \ref{sec:eval-boundary-quant} and Table \ref{tb:compare}, top) on a more comprehensive and robust dataset than any previous work. 
%of data under multiple test scenarios. 
We demonstrate that our algorithms are significantly more accurate than previous methods, superior in both recall and precision in three testing scenarios.
%both exhibiting $>10\%$ higher recall than any other method. 
% Our heuristic outperforms all previous methods, with similar computational advantages (no training required and similarly fast), and our supervised classifier exhibits the highest F1 and recall, but of course requires a one-time training. 

\textbf{C3. Endianness optimization formulation and solution} 
All previous works are \textit{based on an assumption of big endian byte ordering}
(to perform tokenization and/or signal-to-time series matching), and there is no simple remediation for adapting the previous algorithms to perform correctly in the presence of both big and little (reverse byte order) endian signals. 
The second step of our pipeline presents a novel procedure that was crafted to use the predictions from any signal boundary classification algorithm from Step 1 as input and determine the optimal set of endiannesses and signal boundaries from all possible tokenizations (Section \ref{sec:endianess_opt}).
We formulate an objective function to be optimized and provide a formal mathematical proof for reducing the search space to a very tractable grid search algorithm for optimization.
Overall, this insight allows all signal boundary classification algorithms to be leveraged for extracting both little and big endian signals---which has thus far been ignored and/or unachievable. 

\textbf{C4. Signedness classification} 
We provide the first algorithm for determining signal signedness (bit-to-integer encoding) (Section \ref{sec:signed_class}), allowing translation of signals to time series. 
Testing shows this simple heuristic achieves an F-score of $>97\%$.




\textbf{C5. Prototype OBD-II plugin for in-situ or offline use}
The pipeline can be run offline for postdrive analysis  or during driving (to feed online analytics such as a CAN Intrusion Detection System (IDS) with translated CAN data). 
We discuss our design and implementation of a lightweight OBD-II port plugin device (Section \ref{sec:hw} and  Fig. \ref{fig:hw-pic}) for use in any vehicle where a CAN is accessible via the OBD-II port (this is true for most vehicles). 
In a signal learning phase, the device automatically logs CAN data while periodically querying supported DIDs, and then it runs the algorithmic pipeline to learn signal definitions and write a DBC file. 
This allows the real-time decoding of CAN signals on future drives, such as feeding a novel analytic technology leveraging the vehicle's signals online or offline uses, such as  analyzing CAN captures in postcollection analysis. 
This prototype bridges the gap between the algorithmic research in the literature and actual online use with any vehicle. 
% For in-situ use, ACTT 2.0 is implemented as prototype OBD-II plugin. 
% Details of the implementation and the small form factor hardware (depicted in Fig. \ref{fig:hw-pic}) is discussed in Sec. \ref{sec:hw}. 

\textbf{C6. Survey} We provide the first comprehensive survey of works on reverse engineering CAN signals (Section \ref{sec:related-works} and Table \ref{tab:related-works}), outlining the progression of the field and documenting the benefits and limitations of each contribution. 

 

% \label{sec:contributions}
% ACTT 2.0 has a four-step algorithmic pipeline that, given a CAN log, will tokenize and translate (ideally all) signals from sufficiently occurring IDs and can interpret any signals that match diagnostics. 
% See Fig. \ref{fig:pipeline} for an overview of the workflow, and  Sec. \ref{sec:algo}, which details  each step. 
% % Development and evaluation required a dataset of CAN logs. 
% % We describe data used from seven different makes and years in Sec. \ref{sec:dataset}. 
% We evaluate our signal extraction algorithm in Sec. \ref{sec:eval},  comparing head-to-head with the previous state-of-the-art methods on signal boundaries identification (partial tokenization), average error of translated signals, and finally qualitative analysis to examine translation difficulties incurred by variations in endianness and signedness.  
% This evaluation leverages a dataset of CAN logs from seven makes and years, described in Sec. \ref{sec:dataset}.  
% ACTT 2.0 can be run offline for post-drive analysis,  or during driving e.g., to feed online analytics such as a CAN IDS with translated CAN data. 
% For in-situ use, ACTT 2.0 is implemented as prototype OBD-II plugin. 
% Details of the implementation and the small form factor hardware (depicted in Fig. \ref{fig:hw-pic}) is discussed in Sec. \ref{sec:hw}. 
% To use ACTT 2.0, the supervised model for learning signal boundaries (see Step 1 of Fig \ref{fig:pipeline} and Sec. \ref{sec:cutprob}) would be trained offline in advance (once). 
% Next, upon plugging the device into the OBD-II port, it automatically determines the supported (responsive) DIDs, and logs CAN traffic log while iteratively requesting each supported DID. 
% At this point the driver would ideally exercise as much of the vehicle's functionality as possible. 
% Once the CAN log is captured, the algorithmic pipeline processes the log and builds a \texttt{.dbc} file giving the signal definitions (learned tokenization, translation, and interpretation) for each ID. 
% This process of collecting CAN data and running the algorithmic pipeline to produce a .dbc file will occur once per vehicle.  
% Finally, ACTT 2.0 uses the Python cantools module \cite{cantools} and the produced \texttt{.dbc} file to decode CAN data in real-time on future drives. 

% This work provides the following contributions: 

% \begin{enumerate}[leftmargin = *,topsep=5pt,itemsep=2pt,parsep=4pt]
    % \textbf{ACTT 2.0 employs state of the art signal boundary extraction}: Previous works have proposed hand-crafted heuristics for identifying signal boundaries based on two main features---bit flip count features,  and the cardinality of a proposed signals' range \cite{markovitz2017field, nolan2018unsupervised, marchetti2019read, Pese2019librecan}.   
    % ACTT 2.0 applies supervised machine learning algorithms with a  set of 85 features, allowing the well-developed statistical machinery to furnish likelihood of signal boundaries. 
    % We provide experimental results 
    % %results testing a variety of features and supervised algorithms, and empirical results 
    % showing the superiority of this boundary extraction in head-to-head comparisons with previous methods. 
    
    % \textbf{ACTT 2.0 is the lone signal-extraction method accommodating both big and little endian signals}:  No previous work has attempted to correctly extract signals with little endian byte ordering. 
    % Accommodation of how signals can wrap across byte boundaries under both possibilities significantly increases the complexity of the problem.
    % ACTT 2.0 can identify both little and big endian byte orderings within a single ID's message. 
    % To accomplish this, we formulate and solve an optimization problem using signal boundary probabilities to identify both little and big endian signals.  
    % We provide empirical results showing the efficacy and superiority of ACTT 2.0 in extracting both big and little endian signals. 

    % \textbf{ACTT 2.0 is the lone signal-extraction algorithm to accommodate and identify both signed and unsigned signals}: 
    % While  previous extraction algorithms \textit{theoretically} may identify boundaries of both signed and unsigned signals, all previous works have assumed unsigned encodings.  
    % ACTT 2.0 extracts signals accurately regardless of sign, and then identifies each signal's signedness. 
    % The ability to extract and classify both big and little endian as well as both signed and unsigned encodings allows translation of nearly all signals into their numerical values. 
   
%   \textbf{ACTT 2.0  leverages diagnostic information (or other sensor readings) to identify a signal's physical meaning and its linear mapping to the appropriate units}: 
%     Building on  [Redacted citation] and similar to recent advancements of Pes\'{e} et al. \cite{Pese2019librecan}, ACTT 2.0 uses linear regression and a correlation measure to match a subset of extracted signals with diagnostic (DID) time series (or that of another given sensor). 
%     This provides the signal's offset and scale factors providing a real-world interpretation with units. 

    % \textbf{ACTT 2.0 is prototyped as a lightweight OBD-II plugin device for real time CAN decoding}: 
    % In a signal learning phase, the device automatically logs CAN data while periodically querying supported DIDs, and then runs the algorithmic pipeline to learn signal definitions. 
    % This allows the real-time decoding of CAN signals on future drives. 
    % This prototype bridges the gap between the algorithmic research building in the literature and actual online use with any vehicle. 

    % \textbf{We provide the first comprehensive literature review of CAN signal extraction literature}: Previous works often have failed to cite the (relatively few) related works in this area. 
    % We provide, to the best of our knowledge, an overview of every work in the area and their contributions and influence on each other showing the field's progression. 
    



==> CAN-D IEEE/16-impact.tex <==
\vspace{-.4cm}
\subsection{Impact} 
\label{sec:impact} 

Unveiling CAN signals will provide real-time measurements of vehicle subsystems, offer a rich stream of data that promises to fuel many vehicle technologies, and put development and analytics in the hands of consumers (in addition to OEMs).
%, and open the door to developing solutions applicable to vehicles that are currently in use. 

Multiple research works---through direct and even remote access to CANs---have managed to manipulate a few manually reverse engineered signals, resulting in life-threatening effects\textemdash most notably, the remote Jeep hack by Miller and Valasek \cite{checkoway2011comprehensive, koscher_experimental_2010, miller_valasek_2014, miller2015remote}. 
These works demonstrate that CAN reverse engineering is possible on a per-vehicle basis with ample effort and expertise and that it will not inhibit the determined adversary. 
However, the obscurity of CAN data does hinder vulnerability analysis research necessary for hardening vehicle systems, 
and automated CAN reverse engineering will greatly expedite vehicle vulnerability research. 

In parallel, CAN defensive security research is growing quickly; we found 15 surveys of the area published since 2017 (e.g.,  \cite{lokman2019intrusion, wu2019survey}) and over 60 works on CAN intrusion detection published between 2016 and 2019.  
Yet these works are impeded by obfuscated CAN data, forced to use either side-channel methods that ignore message contents \cite{moore2017modeling, lee2017otids, choi2018identifying} or black-box methods ignorant of message meanings \cite{Tyree_Bridges_Combs_Moore_2018, Pawelec_Bridges_Combs_2019, taylor2016anomaly},  arduously reverse engineer a few signals for a specific vehicle \cite{narayanan_secure_2016}, or rely on an OEM for signal definitions \cite{hanselmann2019canet}, which keeps CAN security in the OEM's hands and develops per-make, not vehicle-agnostic, capabilities. 
A vehicle-agnostic CAN signal reverse engineering tool promises to remove these limitations and provide rich, online, time series data for advancements in detection and other security technologies. 
Furthermore, this CAN signal decoding will promote universally applicable technologies to address cars currently on the road, as well as remove reliance on the vehicle OEMs for CAN security. 

Another emerging subfield of research is driver fingerprinting \cite{enev2016automobile, wakita2006driver}, developing methods to identify drivers based on their driving characteristics such as braking, accelerating, and steering. 
Access to the decoded CAN data will allow these works to be ported to plugin technologies for nearly any vehicle, impacting, at a minimum, driver privacy and insurance strategies, and potentially forensic (e.g., criminal) investigations and vehicle security to name but a  few benefits. 


In addition,  access to CAN signals will potentially assist development of aftermarket tuning tools for enhanced efficiency and performance, fuel efficiency monitoring and guidance, fleet management, vehicle fault diagnosis,  forensics technologies, and aftermarket vehicle-to-vehicle capabilities. 
As a final  example, we note that aftermarket technologies to provide autonomous driving capabilities to current vehicles are appearing. In particular, Open Pilot (\url{https://comma.ai/}) provides latitudinal and longitudinal control for many vehicles on the road using a few presumably manually reverse engineered CAN signals. 
Automated, accurate, and universally applicable CAN de-obfuscation will promote and expedite development of such vehicle technologies, especially aftermarket solutions for many vehicles currently in use. 


% The need for decoding in-vehicle CAN data has driven a new and promising sub-field (see  our Related Works Sec. \ref{sec:related-works}).  

% As vehicles are increasingly reliant on electronic communication, it follows that adversarial manipulation of CAN signals have potentially severe consequences. 
% While lightweight, the CAN protocol is bereft of basic security features, e.g., encryption and authentication. 
% Moreover, vehicle CANs are exposed to exploitation\textemdash 
% the now-mandatory OBD-II port often gives direct access to the CAN bus, and the proliferation of vehicle-to-X  interfaces increases the attack surface.
% The current paradigm for passenger vehicle CANs is ``security by obscurity''\textemdash 
% OEMs hold the CAN signal definitions secret, and vary them across years and models. 
% Yet, multiple researchers have, through direct and even remote access to CANs, managed to manipulate a few manually reverse engineered signals, manifesting in life-threatening effects \textemdash most notably, the remote Jeep hack of Miller \& Valasek \cite{checkoway2011comprehensive, miller_valasek_2014, miller2014survey,  miller2015remote, woo2016practical, cho2016error}. 
% These works demonstrate that CAN reverse engineering is possible on a per-vehicle basis with ample effort and expertise, and will not inhibit the determined adversary. 
% The obscurity of CAN data does however hinder vulnerability analysis research necessary for hardening vehicle systems. In parallel, defensive in-vehicle CAN research is a burgeoning subfield. 
% Our literature review revealed 18 surveys on vehicle CAN security, 15 of which occurred in 2017 or later, e.g., \cite{studnia2013survey, lokman2019intrusion, loukas2019taxonomy, wu2019survey}, as well as dozens of papers on CAN security-related areas, e.g.,  \cite{enev2016automobile, Kulandaivel2019canvas, cho2016fingerprinting, brown2018can}.  
% The CAN security literature is dominated by intrusion detection systems (IDS) research for in-vehicle CANs with  $\smalltilde75$ total publications by mid 2019, 60 of which were published since 2016.  

% The inability to translate CAN data  has pigeon-holed CAN IDS developments into a few lanes of contribution. 
% Early works implemented rules akin to signature-based detection \cite{muter2010structured, hoppe2008security}, followed by algorithms leveraging packet header information (e.g., message frequency anomalies \cite{moore2017modeling, Gmiden_Gmiden_Trabelsi_2016, Song_Kim_Kim_2016}), 
% as well as side-channel detection using physical or other timing-based observables \cite{cho2016fingerprinting, choi2018identifying, lee2017otids}. 
% % Muter et. al. \cite{muter2010structured} introduce the concept of ``payload-inspection" IDSs,

% % \begin{figure}[t]
% % \includegraphics[width=.48\textwidth]{figs/canlog_snippet_redacted.png}
% % \caption{CAN log in standard format, depicting one CAN frame per row, with the columns from left to right showing: unix timestamp, user-given network name, and  AID (3 hex characters) + data field (up to 16 hex characters) delimited by \texttt{\#}. 
% %Note AIDs have been anonymized.
% % }
% % \add{Placeholder diptych of raw Canlog and decoded data. Need to anonymize so cant be identified by AIDs}

% % \label{fig:canlog}
% % \end{figure}  


% Other developments include ``payload-inspection'' \cite{muter2010structured} IDSs, those that leverage the actual message carried in the packet. Most of these have a naive approach, that, unable to translate the CAN payloads into constituent signals, apply black-box techniques to learn patterns in the bits and identify anomalies \cite{Stabili_Marchetti_Colajanni_2017, Pawelec_Bridges_Combs_2019, Tyree_Bridges_Combs_Moore_2018, taylor2016anomaly, wang2018distributed, tomlinson2018using}. 
% % Other developments use ``naive'' payload-inspection, that, unable to translate the CAN payloads to constituent signals, apply black-box techniques to learn patterns in the bits and identify anomalies \cite{Stabili_Marchetti_Colajanni_2017, Pawelec_Bridges_Combs_2019, Tyree_Bridges_Combs_Moore_2018, taylor2016anomaly, wang2018distributed, tomlinson2018using}. 
% However, a subset of payload-inspection methods are ``signal-based'' 
% %(referred to as ``semantic-based'' by \cite{muter2010structured}),
% %these ``signal-based'' IDS works, 
% in which real-time decoded CAN data informs detectors,  although these works are either vehicle-specific\textemdash requiring pairing with an OEM who shares the CAN translations or manually reverse engineering a few signals\textemdash or  use ``chipping tools'' to extract some CAN signals  \cite{wasicek2017context, hanselmann2019canet, Li2017intrusion}.
% Alternative approaches have been used to acquire real-time vehicle data that attempt to circumvent the obstacle of decoding CAN data altogether, namely by using external sensors (e.g., an accelerometer) \cite{ganesan2017exploiting, levi2018advanced}; 
% however, this approach not only requires supplementary, often expensive hardware, but exogenous data cannot be used as a proxy for translated in-vehicle data for several use cases that necessitate reading and writing intra-vehicle messages over CAN, e.g., cybersecurity monitoring or aftermarket tuning, among other vehicle technologies. 
% Notably, Markowitz \& Wool \cite{markovitz2017field} are the lone work to attempt to decode CAN signals in a data-driven manner to inform an intrusion detector. 
% % The quintessential idea that cannot be explored in CAN IDS research is that the interdependence of vehicle subsystems must be changed 

% % In summary, CAN security research has thus far worked blind to wealth of diverse vehicle information transmitted in CAN data. 
% Access to these real-time data streams promises to accelerate vulnerability discovery \cite{Pese2019librecan} and open novel avenues for detection. 
% To meet this need, our contribution, ACTT 2.0 provides an algorithmic pipeline that exhibits state-of-the-art CAN signal extraction, and a lightweight hardware integration allowing OBD-II plugin for real-time CAN decoding. 



==> CAN-D IEEE/17-related-works.tex <==

\section{CAN Signal Reverse Engineering Survey}
\label{sec:related-works} 
This section provides the first comprehensive survey of  methods for decoding automotive CAN data into constituent signals. 
We seek to show the progression of the literature, and we provide more detailed descriptions of the methods that we evaluate in Section \ref{sec:eval} with authors/methods in bold. 
Table \ref{tab:related-works} provides a quick reference for the signal reverse engineering contributions of each work. 
% , and the few papers in the area exhibit a steady progression. 

%  \subsection{Signal Categories} Previous works have referred to the following signals categories:  
% \textit{Constant} -  bits that never change; 
% \textit{Categorical} - a categorical variable, i.e. taking on only a few values;
% \textit{Counters} -  value is incremented with each message; 
% \textit{Continuous} -  values of a discretely sampled continuous variable;  
% \textit{CRCs} (cyclic redundancy checks) - checksums occurring within the data frame and in addition to the CAN-specified CRC field.


% \subsection{Survey}
Early work by Jaynes et al. \cite{jaynes_automating_ecu} explored supervised learning to identify CAN messages that control body-related events, but the approach did not account for the fact that data fields comprise multiple disparate signals. Thus, this method simply labels entire messages with a general physical meaning. 

Markowitz and Wool \cite{markovitz2017field} focuses on CAN anomaly/intrusion detection but pursues signal extraction as a preprocessing step. 
They were the first to introduce the basic assumption that each arbitration ID's data field is ``a concatenation of positional [signals].''
%Further, they provide a well-adopted tetrachotomy of signal types as constant, categorical, counters, continuous (See Sec. \ref{sec:can-basics}). 
Implicitly, Markowitz and Wool's algorithm  assumes only big endian and unsigned signals; thus, their algorithm need only identify the start bit and length of a signal. 
The algorithm considers all 2,080 possible  signals (indexed by start bit and length) in an ID's 64-bit data field, and based on the cardinality of each candidate signal's range, the count of observed distinct values. It then categorizes the signal as constant, categorical (taking on only a few values), or continuous (values of a discretely sampled continuous variable) based on the range and assigns a score. 
% decides the signal type (constant, categorical, ...) based on its range, and then assigns a score to each candidate signal based on its type and the number of distinct values observed. 
Finally, the method identifies a nonoverlapping partition of the 64 bits based on category and a optimization of the signals' scores. 
%into signals based on a greedy method that first keeps constant signals, then selects non-overlapping, high-scoring categorical signals, and lastly non-overlapping, high scoring counter and continuous signals. 
% Quantitative evaluation of the accuracy of extracted signals is not straight-forward, and a contribution of Markowitz \& Wool's initial work is to score each ID's predicted signals by counting the number of bits given an incorrect signal type label (up to 64), and the number of incorrect signal boundaries (up to 63) and summing these two figures. 
% For evaluation, they build a generative model to synthesize CAN messages with known signals. 
% While the seminal work in the area, Markowitz \& Wool either ignored or were unaware of the variety of byte orderings (endianess), bit encodings (signed/unsigned signals), and checksums that appear in automotive CAN frames. 
% Theoretically, signed and unsigned big-endian signals should be extracted by this method. 

Huybrechts et al. \cite{huybrechts2017automatic} published the first work to leverage DIDs to annotate CAN data and identify signals. 
Their algorithm converts bytes/byte-pairs in CAN messages to integers and identifies those that are similar to the concurrently collected DID responses, but it operates under the self-acknowledged false assumption that CAN signals are limited to only one- or two-byte signals. 
No linear transformation of extracted signals to the DID sensor values is given. 


The next three works, TANG by Nolan et al. \cite{nolan2018unsupervised}, 
ACTT by Verma et al. \cite{verma2018actt},  
%(the precursor to this work), 
and READ by Marchetti and Stabili \cite{marchetti2019read} appear to have occurred independently and concurrently, and we present them chronologically by publication date.

\textbf{Nolan et al.} \cite{nolan2018unsupervised} focus solely on extracting continuous signals by considering transition aggregated $n$-grams (\textbf{TANG}). 
Given an ID trace $[B_0(t), \dots, B_{63}(t)]_t$, Nolan et al. define a TANG vector as $(T_0, \dots, T_{63})$ with 
$T_i = \sum_{t} B_i(t_j) \bigoplus B_i(t_{j+1})$, where $\bigoplus$  denotes XOR. 
Note that this is simply a computationally efficient way to obtain the bit flip count; thus, if an $n$-bit signal's subsequent values change by unit increments, then the LSB will exhibit $T_i = 2^n + 1$, and each next significant bit will have TANG values decreasing by a factor of $2$. 
% As the TANG value will roughly decrease when walking from most to  least significant bit, a greedy algorithm walks the bits' TANG values to identify signal boundaries. 
% This gives a clever and computationally efficient way to extract boundaries of signed and unsigned continuous signals. 
Roughly speaking, the algorithm for identifying continuous signal boundaries computes the TANG vector from an ID trace, identifies the bit with maximal TANG value as a signal's LSB, and walks left (respectively right for reverse bit order), absorbing bits into the signal until the TANG value increases.
% (0) compute the TANG vector from an ID's trace; 
% (1) reverse sort bit indices by the TANG value (largest to smallest) and store them in a list $l$.   
% (2) label the highest TANG value as new signal's LSB and pop this index from $l$;
% (3) so long as subsequent bits to the left (right if considering reverse bit orderings) have decreasing TANGs, incorporate them as a signal and pop their indices from $l$.  
Nolan et al. consider both forward and reverse bit orderings to attempt to take little and big endian encodings into account. 
However, since endianness refers to \textit{byte} (not bit) order, this method cannot accommodate true little endian signals, and in fact violates the fixed bit order defined by the standard. 
% While we have identified little and big endianness and signed and unsigned encodings in data, 
% We have not identified reverse bit orderings in any CAN data. 
% Note that the forward/reverse bit ordering seems to be an input to the system, and not decided by the system. 
Overall, this method assumes big endian, unsigned, and continuous signals.\looseness=-1
%but theoretically can accommodate signed and unsigned encodings but not little endian. 
% It cannot distinguish which encoding is used. 
% Presumably plotting both and encodings and manually deciding is used in post-analysis. 
% Nolan et al. note that quantitative measurement of the accuracy of CAN signal extraction may hard to interpret and even misleading; ergo, they provide qualitative evidence on real CAN data of extracted unsigned, big endian signals. 

\begin{table}[t]
\centering
\caption{Automotive CAN signal reverse engineering algorithms for each of the four signal properties. CAN-D is the only comprehensive algorithm, determining all four properties.}
\label{tab:related-works}
\begin{threeparttable}
\setuptable
\vspace{-.4cm}
\begin{tabular}{lccccccc}
		\multicolumn{1}{l}{}
	    & \headrow{Boundary} 
		& \headrow{Endianness} 
		& \headrow{Signedness} 
		& \headrow{Interpretation}
		\\ 
		\toprule
		Jaynes et al. (2016) \cite{jaynes_automating_ecu}                    &\none	&\none	&\none	 &\prt \\
		Markowitz \& Wool (2017) \cite{markovitz2017field}                   &\full	&\none	&\none	 &\none \\ 
		Huybrechts et al. (2017) \cite{huybrechts2017automatic}              &\prt	    &\none	&\none	 &\prt \\
		Nolan et al.'s \textbf{TANG} (2018) \cite{nolan2018unsupervised}     &\full	&\none	&\none	 &\none \\ 
		Marchetti \& Stabili's \textbf{READ} (2018) \cite{marchetti2019read} &\full	&\none	&\none	 &\none \\
		Verma et al.'s \textbf{ACTT} (2018) \cite{verma2018actt}             &\full	&\none	&\none	 &\full \\
		Pes\'{e} et al. \textbf{LibreCAN} (2019) \cite{Pese2019librecan}     &\full	&\none	&\none	 &\full \\
		Young et al. (2020) \cite{young2020towards}                          &\none	&\none	&\none	 &\prt \\
		\cdashlinelr{1-5}
		\textbf{CAN-D}                                                &\full	&\full	&\full	 &\full \\
		
    \bottomrule
	\end{tabular}
\end{threeparttable}
\end{table}



\textbf{Marchetti and Stabili} \cite{marchetti2019read} propose the Reverse Engineering of Automotive Dataframes (\textbf{READ})  algorithm to extract signals
%a trichotomy of signal categories \textemdash  counters, CRCs, and a catch-all bin, ``physical" signals\textemdash
using heuristics based on a 64-length vector that contains each bit's observed flip probability---that is, $[ P(B_i(t_j) \neq B_i(t_{j+1}) ) ]_{i = 0}^{63}$.   
First, signal boundaries are identified using $m_i := \lceil \log_{10}( P(B_i(t_j) \neq B_i(t_{j+1}) )) \rceil$, the ceiling function of the log probabilities. 
% (Note: $\lceil \log_{10}(\cdot)\rceil$ is an integer-valued function that jumps when the input changes by a factor of 10). 
READ follows intuitive logic similar to that of TANG; for continuous signals, an LSB flips \textit{much} more often than an adjacent signal's MSB. Thus, READ places signal boundaries between bits $i$ and $i+1$ iff $m_i > m_{i+1}$---or equivalently if the the bit flip probabilities cross a factor of 10 (e.g., from above $.01$ to below).  
Unlike TANG, READ does not claim to assume only continuous signals, and it in fact builds on Markowitz and Wool's signal categorization efforts. It considers three signal categories---counters (increments by 1 with each message), checksums (hashes for checking whether messages are properly transmitted), and a catch-all bin, ``physical" signals---binning the extracted signals with further heuristics relating to bit flips.
%Using further heuristics relating to bit flips, extracted signals are then categorized. 
% Within these signal boundaries, a few heuristics are run (also using to identify counters and checksum. 
% Specifically, a counter signal's least significant bit flips every frame ($P = 1$), and each subsequent bit has probability that is a multiple of 1/2 of the previous. 
% Similarly, as checksums appear as noise, CRC bits have a probability of flipping of approximately 1/2.
%yielding a  heuristic for possible labeling. 
% Finally, to identify the remaining ``physical'' signals' boundaries, READ looks at $m_i := \lceil \log_{10}( P(B_i(t) \neq B_i(t+1) )) \rceil$ the ceiling function of the log probabilities. 
% (Note: $\lceil \log_{10}(\cdot)\rceil$ is an integer-valued function that jumps when the input changes by a factor of 10). 
% For the remaining uncategorized bits, READ places ``physical'' signal boundaries if $m_i > m_{i+1}$, following the intuition for continuous signals that a least significant bit ($m_i$) flips \textit{much} more often than another signals most significant bit ($m_{i+1}$). 
Ultimately, READ partitions an ID's 64-bit data frame into signals with categorical labels. 
The algorithm ignores little endian and signed encoding possibilities and cannot be easily amended to accommodate little endian signals. 
% In theory, this algorithm will usually cut little endian signals on byte boundaries, but will correctly find boundaries of signed big-endian signals. 
% Although, for any little-endian or signed signals, it will not translate the bits to values correctly. 
% READ is evaluated on synthetically generated CAN data and real CAN data for two metrics, (1) the count of correct signal boundaries identified and (2) the percent of correctly bounded signals that were labeled as counter, CRC, or ``Physical''. 
Marchetti and Stabili's evaluations with real and synthetic CAN data compared with Markowitz and Wool's method reveal that READ is far more accurate at finding signal boundaries.\looseness=-1 

\textbf{ACTT} by \textbf{Verma et al.}  \cite{verma2018actt} 
%the precursor to this work,  
takes an approach fundamentally different from all previous works. Instead of partial tokenization and translation---learning to identify signal boundaries under limiting assumptions (e.g., assuming big endian and unsigned encodings) in an unsupervised fashion---ACTT simultaneously tokenizes, translates, and \textit{interprets} CAN signals. 
The method automatically identifies which DIDs (see Section \ref{sec:dids}) respond on the particular vehicle and then collects ambient CAN data during driving while periodically querying DIDs. 
These diagnostic responses provide labeled time series and DID traces alongside the CAN data, setting up a supervised decoding algorithm. 
For a given ID trace, the constant bits are labeled, and all possible signals (start bit, length) from the remaining nonconstant bits are considered. 
For each possible signal and for each DID trace, linear regression is performed, and a score of linear fit is assigned. 
A scheduling algorithm using dynamic programming then identifies a nonoverlapping set of signals that maximize the fitness score. 
The output is twofold: (1) a list of constant signals, and (2) a subset of signals equipped with linear mappings to a known physical unit that matches a DID  (start bit, length, scale, offset, physical unit, sensor label). 
% While this algorithm does not attempt to partition all 64-bits into signals, it does both tokenize and translate the signals it extracts. 
% Because the signal learning process is a minimization of error between the extracted signal and a DID's  sensor values, the translated signal's generally give high fidelity matches to a physical sensor's values even in the presence of tokenization errors; 
% e.g., a 16-bit speed signal, taking translated values between 0-120 MPH has such high resolution that truncating the least significant bits changes the translated value only negligibly. 
% the LSB and the offset maybe both be slightly off, but the translated signal's values are nearly identical to the DIDs. 
As in all previous works, this method assumes unsigned encodings, and following TANG by Nolan et al., mistakenly considers reverse bit order as little endian (not \textit{byte} order). 
Because this method relies on DID matching to tokenize signals, only a small subset of signals can be extracted, but all extracted signals are interpretable.\looseness=-1
% Because only signals matching a DID are extracted, it has low recall, but translated signals are high fidelity. 
%of the translated signals to sensors are high. 
% The optimal scores of the extracted signals gives a quantitative measure (explained variance) of the signal's fit to physical data. 
% Further, quantitative analysis is given showing near exact matches are often found and not-so-exact matches can provide easily discernable signal that are not in the DIDs. 
% Note that this method is directly applicable for  use with external sensors in place of/addition to DIDs sensor readings. 


\textbf{Pes\'{e} et al.} \cite{Pese2019librecan} present \textbf{LibreCAN}, a three-phase process.
(Phase 0) LibreCAN makes tweaks to READ's algorithm for identifying signal boundaries and categorizing extracted signals. 
Specifically, whereas READ identifies signal boundaries by finding where adjacent bit flip probabilities decrease across a multiple of 10, LibreCAN identifies whether adjacent bit flip probabilities drop by a factor of $T_{p0,2}$, a tunable input parameter. 
(Phase 1) LibreCAN next leverages ideas similar to those of Verma et. al. \cite{verma2018actt}, using cross-correlation to match signals to sensor readings from both DIDs and external sensors, then using linear regression to learn the scale and offset. 
% LibreCAN has an algorithm based on cross correlation of extracted signals against sensor time-series to decide a match, then uses linear regression 
(Phase 2) LibreCAN incorporates a novel, semiautomated method for identifying  body-related signals (e.g., door locks, windshield wipers) by filtering IDs based on changes in data fields before and after a user actuates the body-related feature. 
Pes\'{e} et al. note that little endian signals exist, but like all previous methods, their algorithm assumes big endian byte order and unsigned encodings and does not have a natural extension to accommodate little endian signals.

Lestyan et al. \cite{lestyan2019extracting} focus on CAN signal extraction in support of a data-driven driver fingerprinting method. 
Using neighboring bits' probabilities, the authors propose a method to identify signal boundaries yet settle on considering only one- or two-byte signals. 
Supervised learning to match a few  signals (e.g., rpm, speed, and braking) is trained on just one car's (manually labeled) signals  and tested on seven other vehicles. 
This work seems unaware of most other works in the area. 

The most recent CAN reverse engineering work, by Young et. al. \cite{young2020towards}, uses an approach similar to LibreCAN (Phase 2) to match vehicular functions (based on a hand-labeled time series) to CAN IDs using a data change identification algorithm. They use a clustering algorithm to group related IDs, labeling the remaining unknown IDs based on those labeled in the matching step. However, similar to Jaynes et al., this work attempts to assign physical meaning to an entire CAN ID rather than tokenize, translate, and then identify (assign meaning to) constituent signals; thus, we do not consider it (nor the work by Jaynes et al.) to be a true signal reverse engineering algorithm. 

% \subsection{Limitations of Previous Works}
All previous works suffer from significant limitation.
Most notably, all assume both big endian byte order and unsigned encodings.
%among other limiting assumptions.
Although some may theoretically correctly identify signed signals' boundaries, this has not been mentioned or tested. % and no previous method provides a means for determining signedness. 
Worse, there is no natural extension to little endian and/or signed signals. 
To identify signedness, an additional algorithm is needed\textemdash a fairly straightforward binary classification problem that is not difficult once well formed.
On the other hand, including endianness poses a far harder problem for two reasons: 
(1) signal boundary algorithms depend on flip
counts of 
``neighboring'' bits, but bit orderings change with endianness, so neighboring bits cannot be determined; and
(2) without considering both endiannesses, signal boundary identification is 
computationally simple (the same binary classification is independently repeated 64 times per ID), but considering all byte orderings grows the search space combinatorially ($2^{64}$ boundary options $ \times\ 2^8$ byte orders $> \ 4.72\mathrm{E}21$ tokenizations per ID!) with a web of changing dependencies. 


==> CAN-D IEEE/20-algorithm.tex <==
\section{Algorithm}
\label{sec:algo}
% As shown in Fig. \ref{fig:pipeline}, ACTT 2.0's algorithmic pipeline involves machine learning and an optimization process to learn signal boundaries and  endianness (\textcolor{Plum}{tokenizes}), then classifies signals as signed or unsigned (\textcolor{SeaGreen}{translates}), and finally matches as subset of signals with the diagnostic information (\textcolor{RoyalBlue}{interprets}). 

We present CAN-D, a four-step modular pipeline (depicted in Fig. \ref{fig:pipeline}) that provides the first comprehensive and vehicle-agnostic CAN signal reverse engineering solution. 
%In this section, we present a general framework for \textcolor{Plum}{\textbf{tokenizing}}, \textcolor{SeaGreen}{\textbf{translating}}, and optionally \textcolor{RoyalBlue}{\textbf{interpreting}} CAN signals, thus fully defining each signal. 
We describe the needed inputs and outputs for the modular components---a \textit{signal boundary classifier} (Step 1, Section \ref{sec:cutprob}), a
\textit{signedness classifier} (Step 3, Section \ref{sec:signed_class}), and a \textit{signal to time series matcher} (Step 4, Section \ref{sec:diag-matching})---as well as our novel \textit{endianness optimizer} (Step 2, Section \ref{sec:endianess_opt}), which we consider to be the unique component that provides the glue for the interchangeable components. 


==> CAN-D IEEE/21-boundary-labeling.tex <==
\subsection{Step 1: Signal Boundary Classification}
\label{sec:cutprob}
Given an ID trace as input, a signal boundary classifier makes
%, the problem of identifying signal boundaries can be viewed as 
64 binary classification decisions. It predicts whether each of the 64 bits is the LSB of a signal, effectively deciding whether a signal boundary or ``cut'' occurs between each bit and the following bit.  
% For each ID, the 64-bit message has 63 ``bit gaps'' indexed $(i,i+1)$ for $i = 0, \dots, 62$, and bits $i$ and $i+1$ are either contained in the same signal or span two signals. 
Almost all previous works have focused on signal boundary classifiers that use hand-crafted heuristics that leverage only one feature, the probability of each bit flipping.
%computed from an ID trace: %or the range of values a candidate signal realizes.
%\textemdash and depended on the overly simplifying assumption that all signals are big endian and unsigned. 
In this section, we pursue the same goal but use a wider set of features. 
In addition to a novel, unsupervised heuristic,  we leverage supervised ML and deliver two superior signal boundary classifiers. 
% The datasets used for training and testing is described in Sec. \ref{sec:dataset}, and

For the reverse engineering pipeline, outputs of the signal boundary classifier in Step 1 are inputs to the endianness optimizer in Step 2. 
Although we frame signal boundary identification as a set of binary classifications, the input for Step 2 of the CAN-D pipeline is  %and therefore needed as an output from this step, is not a binary label (boundary or non-boundary), but
the estimated probability---in $\{0,1\}$ for binary heuristics or in $[0,1]$ for ML---of a signal boundary for each bit. 
Algorithms developed in previous works \cite{markovitz2017field,marchetti2019read, nolan2018unsupervised, verma2018actt} and \cite {Pese2019librecan} (Phase 0) could be used as the signal boundary classifier for this step, all of which produce binary label outputs. 
Section \ref{sec:eval} presents results comparing our signal boundary classifiers against the previous state of the art. 


% This subsection sets up signal boundary identification as a binary classification problem, describes our feature set, details experiments with supervised machine learning classifiers, and finally presents a simple unsupervised heuristic. 

\subsubsection{Data and Notational Setup}  %%% condensed data training and notation
Both unsupervised and supervised predictions are based on statistics that describe how a particular bit and its neighboring bits flip.  
We use a ground-truth DBC (see Section \ref{sec:dataset}) to create a target vector, 
%$y^{id}\in \{0,1\}^{m_{id}-1}$, 
providing a 0/1 label for each bit to indicate whether it is a signal's LSB (boundary).   
% While this is straightforward for big endian signals, little endian signals have adjacent bits with non-adjacent indices at byte boundaries (see Eq. \ref{eq:bit-orderings}). 
To deal with the issue that neighboring bits at byte boundaries are conditioned on endianness, we split little endian signals on byte boundaries for training the supervised models and testing all models. 
In use, the classifier (heuristic or ML) will be applied to ID traces under both byte orderings (see Eq. \ref{eq:bit-orderings}), creating two sets of predictions. 
Both sets of predictions are input to Step 2, which determines the endianness of each byte. 
\looseness=-1


Here we introduce two views of the data used for training and then scoring/tuning the ML in this section. (Both are also used for testing all methods in Section \ref{sec:eval-boundary-quant}.) 
For training, we remove the constant bits (obvious boundaries) forming a ``condensed trace.''
The motivation for %using these condensed traces in training is multifold: 
this is threefold:
(1) Based on assumption \textbf{(A0)} (see Section \ref{sec:problem}), observed constant bits necessarily delimit signals, so a simple rule suffices to identify these obvious signal boundaries. 
The algorithm's goal is to learn signal definitions from a given set of CAN data; thus, unused bits are limitations in the data that is present. Having ample and varied CAN  data promises to enhance the accuracy of the overall CAN-D pipeline when used for training and to provide more thorough examination of the algorithm's abilities when used in testing. 
(2) Our features encode neighboring bits' values and flips, so when nearby bits are constant, features are either trivial or undefined. 
Removing the constant bits prior to feature building yields a better feature set. 
(3) Classes are highly biased toward the negative class; most bits are not an LSB (not on a signal boundary). 
By removing constant bits, we not only get better features, but we also artificially increase the number of nonobvious signal boundaries and decrease class bias, particularly for the nonobvious examples for which a classifier is needed. Note this is the ``c'' set described in Section \ref{sec:eval-boundary-quant}.
% Sec. \ref{sec:boundary_classification_data} discusses the many reasons for this.
%Denote this ``condensed'' ID trace $B^{\prime id} \in \{0,1\}^{n_{id}\times{m_{id}}}$ where $m_{id}$ is the number of non-constant bits for a given arbitration ID $id$. 
Using this condensed trace, we build a feature array
%$X^{id} \in \mathbb{R}^{m_{id}-1\times n_f}$, $X^{id}$ 
with shape $m$ nonconstant bits by $n_f$ features (features described below for each method).

Second, for tuning the ML classifiers in this section, we only consider their performance on the nonobvious boundaries in the original data\textemdash those boundaries not abutting constant bits in the noncondensed ID traces. 
% the original, non-obvious boundaries\textemdash those not abutting constant bits in the non-condensed ID traces. 
Note that this set is the ``f$-$'' set described in Section \ref{sec:eval-boundary-quant}.
We tune our supervised model on this set because we ultimately wish to apply the model to full 64-bit traces and optimize performance for this situation. 
% When tuning the model, we only score examples that were non-obvious---not abutting a constant bit in the ``full'' non-condensed trace---since we ultimately wish to apply the model to full 64-bit traces and want to optimize performance for this scenario. 
% This is reconciled in CAN-D's step 2 (Sec. \ref{sec:endianess_opt}), which considers bit orderings of both endianness.



\begin{wraptable}[9]{r}{3cm}
\vspace{-.2cm}
 \fbox{%
   \begin{minipage}{\dimexpr2.9cm-2\fboxsep}
    \small
    \caption{Local bit-flip features; $F_i$ denotes a flip of bit $i$.}
    %Local Bit Flip Features ($t$ and $t'$ denote subsequent timestamps)}
    \label{tb:features}
    \begin{tabular}{l}      %\addtolength{\tabcolsep}{-2pt}
            \toprule
            % \textbf{Bit Flip Features}\\
            % \midrule
            % $P(B_i(t) \neq B_i(t'))$\\
            % $P(B_i(t) \neq B_i(t') \mid B_{i+1}(t) \neq B_{i+1}(t'))$\\
            % $P(B_{i+1}(t) \neq B_{i+1}(t') \mid B_i(t) \neq B_i(t') )$\\
            % $P(B_i(t) = B_i(t') \mid B_{i+1}(t) = B_{i+1}(t'))$\\
            % $P(B_{i+1}(t) = B_{i+1}(t') \mid B_i(t) = B_i(t'))$ \\
            $P(F_i)$\\
            $P(F_i \mid F_{i+1})$\\
            $P(F_{i+1} \mid F_i)$ \\
            $P(\neg F_i \mid \neg F_{i+1})$\\
            $P(\neg F_{i+1} \mid \neg F_i)$ \\
            % \bottomrule
        \end{tabular}
   \end{minipage}}
\end{wraptable} 
\subsubsection{Supervised Classification}
\hspace{5cm} To describe features conceptually, we use $i\pm1$ to denote bit $i$'s neighbors, notationally neglecting the varying neighbors based on endianness (see Eq. \ref{eq:bit-orderings}) when it presents unnecessary complications. %, although we are mindful that neighbors depend on byte order  . 
For each bit $i$, %$m_{id}-1$ bit gaps in the condensed trace $B^{\prime id}$,
we generate a set of 15 features. 
% five features are ``local'' to the gap, examining only bits $i$ and its neighboring bit on the right, the next five are analogous for the bit on the right, and the final five are the differences in these two sets.  
The first five features are  ``local'' to bit $i$ and its relationship to bit $i+1$, and are denoted by $v^{id}_i \in \mathbb{R}^{5}$.
These features (listed in in Table \ref{tb:features}) are %based on the 
estimated probabilities of a ``bit flip'' based on observations in data over time. The flip of bit $i$---alternating value in subsequent messages $B_i(t_j) \neq B_i(t_{j+1})$---is denoted by $F_i$. 


The guiding principle is that a signal's LSB generally alternates value much more often than an adjacent signal's MSB; thus, the bit flip features should provide good indicators for boundaries. 
Specifically, the first feature should identify LSBs ($P(F_i) \approx 1$) and MSBs ($P(F_i) \approx 0$). 
This is essentially the feature on which previous works \cite{nolan2018unsupervised, marchetti2019read, Pese2019librecan} base their heuristic. 
The next four conditional bit flip features are expected to differ significantly for adjacent bits contained in the same signal versus those that are part of separate signals because the former are likely dependent while the latter are likely independent. 

Next, we look to the neighboring bit on the right, bit $i+1$, and add the five local features for this bit  $v^{id}_{i+1}$ to our feature set for bit $i$. 
Finally, we add five difference features $\delta(v^{id}_{i+1}, v^{id}_{i})$, yielding a total 15-length feature vector for bit $i$. 

Initially, we experimented with adding a wider variety of features based on bit values, two-bit distributions, and entropy, as well as more left/right neighboring features. However, we found that these features did not improve classification performance and in fact resulted in overfitting. 


\begin{table}[t]
    \small
    \centering
    \begin{threeparttable}[]
        % \caption{Aggregated Classification Metrics using LOOCV by CAN log, only scoring non-obvious boundary decisions (f$-$ set). \textbf{Top}: Classifiers with default Scikit-learn parameters. \textbf{Bottom}: The top performing Random Forest Model, with optimal parameters chosen using a grid search.}%
        \caption{Aggregated classification metrics of signal boundary classifiers scoring only nonobvious boundary decisions (f$-$ set). The best supervised method and unsupervised heuristic (bolded) are used in the CAN-D pipeline. \textbf{Top:} Supervised classifiers are run with default scikit-learn parameters using LOOCV by CAN log. Top-performing models (italicized) are tuned with optimal parameters chosen using a grid search. 
        \textbf{Bottom:} The unsupervised heuristic (see Alg. \ref{alg:boundary-heuristic}) performs only slightly worse than the best supervised method.}%
        %Note that the results from models with balanced class weights are not shown since these yielded worse F-scores.
        % \textbf{Bottom:} Performance metrics for top performing classifier with optimal parameters chosen using a Grid Search and LOOCV.}
        \label{tb:boundary_classifier_results}
        \begin{tabular}{lccc}
        \toprule
        {Classifier} &  {F-Score\phantom{m}} &  {Precision\phantom{m}} &  {Recall\phantom{m}} \\
        \midrule
        AdaBoost            &     87.6 &       82.6 &    93.3 \\
        Decision Tree       &     78.5 &       67.8 &    93.3 \\
        \textit{KNN}                 &     88.1 &       81.3 &    96.2 \\
        \textit{KNN (Tuned)}           &     89.7 &       82.6 &    98.1 \\
        Logistic Regression &     86.9 &       82.1 &    92.3 \\
        \textit{MLP\tnote{1}}                 &     88.4 &       82.5 &    95.2 \\
        Naive Bayes          &     71.6 &       57.6 &    94.7 \\
        \textit{Random Forest}       &    90.2 &      85.4 &    95.7 \\
        \textit{\textbf{Random Forest (Tuned)\tnote{2}}}       &    \textbf{ 91.2} &      \textbf{ 87.6} &    \textbf{95.2}\\
        SVC Linear          &     85.5 &       78.6 &    93.8 \\
        \textit{SVC Poly}            &     88.7 &       85.3 &    92.3 \\
        \textit{SVC Poly (Tuned)}      &     88.9 &       85.4 &    92.8 \\
       \textit{SVC RBF\tnote{1}}             &     89.0 &       84.8 &    93.8 \\
        SVC Sigmoid         &     46.4 &       42.3 &    51.4 \\
        \cdashlinelr{1-4}
        \textbf{Heuristic} & \textbf{89.6}    &   \textbf{89.9}        & \textbf{89.4}\\
        % SVC Poly (Tuned)      &     88.9 &       85.4 &    92.8 \\
        % SVC RBF (Tuned)       &     89.0 &       84.8 &    93.8 \\
        % KNN (Tuned)           &     89.7 &       82.6 &    98.1 \\
        % MLP (Tuned)           &     88.2 &       81.0 &    96.6 \\
        % Random Forest (Tuned)\tnote{1}       &    \textbf{ 91.2} &      \textbf{ 87.6} &    \textbf{95.2}\\
        \bottomrule
        \end{tabular}
        \begin{tablenotes}
        \small
        \item[1] Default parameters were optimal
        \item[2]\texttt{max\_features=$\sqrt{n_f}$,  
        min\_samples\_Leaf=3, n\_estimators=200,
        max\_depth=5}
        \end{tablenotes}
            
    \end{threeparttable}
\end{table} 



We tested the performance of several binary classifiers: 
naive Bayes, logistic regression, support vector classifiers (SVC), decision trees, random forests (RFs), k-nearest neighbors (KNNs), multilayer perceptrons (MLP), and AdaBoost.
After experimenting with different weighting schemes to combat the bias class issue, as well as the fact that we only score the nonobvious boundaries, we settled on a sample weighting scheme of nonobvious-positive:negative:obvious-positive of 8:4:1 (no weighting scheme used for KNN and MLP). 
% We also tried using balanced class weights, since we have high bias towards the negative class (non-boundary gaps). 
%(See Sec. \ref{sec:dataset} statistics on dataset).
To test the accuracy of the classifiers, we used leave-one-out cross-validation (LOOCV), holding out one CAN log per fold and aggregating the results, and the f$-$ set, only scoring nonobvious boundaries. 
The results are shown in Table
\ref{tb:boundary_classifier_results}. Focusing only on the best classifiers (those that achieved $\geq 88\%$ F-score using default scikit-learn parameters), we found the optimal parameters for these top-performing  models using a grid search and LOOCV. The best-tuned model is the RF classifier, which yields an overall 88\% precision and 95\% recall for an F-score of 91\%. 
We selected this tuned RF model for our ML classifier.
% Finally, since the next step of the pipeline accepts soft probabilities rather than binary labels, so 
Finally, as an input to Step 2, we output the classifier's predicted probability of a bit $i$ being a signal's LSB. 


% \begin{figure}[!ht]
% \centering
% \subfloat{%
%   \caption{A caption for figures \protect\subref{subfig2}.}
% }%
% \qquad
% \subfloat{%
%     \label{subfig2}%
%     \includegraphics[width=.4\linewidth]{figs/boundary_hueristic_plot.pdf}%
% }
% \label{myfig}
% \end{figure}

% \vspace{.1cm}
% \begin{minipage}{.74\linewidth}%
% % \vspace{-.5cm}  
% % \centering
% \includegraphics[width=\textwidth]{figs/boundary_hueristic_plot.pdf}%
% \end{minipage}
% \begin{minipage}{.20\linewidth}%
% \captionof{figure}{Vis-ualization of Heuristic Signal Boundary Classifier (Alg. \ref{alg:boundary-heuristic}) based on conditional bit flip probabilities, with $\alpha_1 = .01$, $\alpha_2 = .5$.}%
% \label{fig:boundary_heuristic}%
% \end{minipage}%
    
\subsubsection{Unsupervised Heuristic} 
As an alternative to ML, %  that requires a one-time computationally expensive training, 
we further explored the feature set to develop a simple heuristic relating to bit flip probabilities.
We found that the conditional bit flip probability $P(F_{i+1}| F_{i})$ and the difference between successive conditional bit flip probabilities $P(F_{i+2} \mid F_{i+1}) -  P(F_{i+1} \mid F_{i})$  are better indicators of a signal ending at bit $i$ than the difference of unconditional bit flip probabilities  $P(F_{i+1}) - P(F_i)$ used by most related works. 

% \begin{wrapfigure}{r}{.33\textwidth}
% %\begin{figure}[]
%     % \vspace{-.5cm}  
%     % \centering
%     %\includegraphics[width=.45\textwidth]
%     \includegraphics[width=.33\textwidth]
%     {figs/boundary_hueristic_plot.pdf}
%     % \caption{Visualization of Heuristic Signal Boundary Classifier (Alg. \ref{alg:boundary-heuristic}) based on conditional bit flip probabilities, with $\alpha_1 = .01, \alpha_2 = .5$.}
%     \label{fig:boundary_heuristic}
%     % \vspace{-.25cm}  
% %\end{figure} 
% \end{wrapfigure} 

% \begin{minipage}{.20\linewidth}%
% \captionof{figure}{\protect\raggedright{Vis-ualization of Heuristic Signal Boundary Classifier (Alg. \ref{alg:boundary-heuristic}) based on conditional bit flip probabilities, with $\alpha_1 = .01$, $\alpha_2 = .5$.}}%
% \label{fig:boundary_heuristic}%
% \end{minipage}%
% \begin{minipage}{.76\linewidth}%
% % \vspace{-.5cm}  
% % \centering
% \hspace{.4cm}%
% \includegraphics[width=\textwidth]{figs/boundary_hueristic_plot.pdf}%
% \end{minipage}

% \begin{minipage}{.20\linewidth}%
% \captionof{figure}{\protect\raggedright{Vis-ualization of Heuristic Signal Boundary Classifier (Alg. \ref{alg:boundary-heuristic}) based on conditional bit flip probabilities, with $\alpha_1 = .01$, $\alpha_2 = .5$.}}%
% \label{fig:boundary_heuristic}%
% \end{minipage}%


We developed a heuristic based on these findings, detailed in Alg. \ref{alg:boundary-heuristic} and visualized in Fig. \ref{fig:boundary_heuristic}.
Based on observations of data, we found that setting parameters $\alpha_1 = .01, \alpha_2 = .5$ splits the feature space well and yields a $90\%$ F-score and precision and $89\%$ recall (also on the f$-$ set). 
Note that our heuristic was developed and tuned based on a small preliminary dataset, but we found that it generalized well to all of our data. 

The heuristic's main advantage is that it requires no training while achieving similar accuracy to that of the ML, as shown in Section \ref{sec:eval-boundary-quant}.
Though simple, intuitive, and computationally efficient, one drawback %of the heuristic versus %labeling vs. prediction using 
%ML 
is that the outputs are binary labels with no way of determining probabilities properly in $(0,1)$,  
% Therefore, when using a heuristic in Step 1, probabilities in $\{0,1\}$ are fed to Step 2, 
thereby removing some of the flexibility offered by the following step.
\begin{algorithm}[h]
     \caption{Heuristic signal boundary classifier}
     \label{alg:boundary-heuristic}
     \textbf{Inputs} $P(F_{i+1} \mid F_{i})$, $P(F_{i+2} \mid F_{i+1})$, $\alpha_1$ , $\alpha_2$\\
     \eIf{$P(F_{i+1} \mid F_{i}) < \alpha_1$ or $P(F_{i+2} \mid F_{i+1}) -  P(F_{i+1} \mid F_{i}) > \alpha_2$}{
       \Return \texttt{True}
      }{\Return \texttt{False}}
    \end{algorithm}
 \vspace{-.4cm}  
 
\begin{figure}[t]
    \vspace{-.5cm}  
    \centering
    \includegraphics[width=.48\textwidth]{figs/boundary_hueristic_plot.pdf}
    \caption{Visualization of heuristic signal boundary classifier (Alg. \ref{alg:boundary-heuristic}) based on conditional bit flip probabilities, with $\alpha_1 = .01$, $\alpha_2 = .5$.}
    \label{fig:boundary_heuristic}
\end{figure}




==> CAN-D IEEE/22-endianness-optimization.tex <==
\subsection{Step 2: Endianness Optimization}
\label{sec:endianess_opt}  
Armed with the probability of a boundary or ``cut'' between adjacent bits of a message, we constructed an optimization problem to simultaneously determine the most likely packing of signals into the 64-bit data field and most likely endiannesses of each of the eight bytes. 

\subsubsection{Valid Tokenizations}
$I$ denotes a candidate signal, represented by the list of signal bit indices ordered from MSB to LSB.   
%(bit $I[0]$ is the MSB; bit $I[1]$ the next most significant bit, etc.) 
Given a signal $I$, let $LSB(I)$ (or simply $LSB$ if no ambiguity is present)   denote the least significant bit. 
We consider constant bits as 1-bit signals. 
Each ID has eight bytes indexed $j = 0, \dots, 7$ with byte $j$ composed of bits  $8j, \dots, 8(j+1) - 1$  (e.g., byte 2 refers to bits $16, 17, \dots 23.$) Refer to Fig. \ref{fig:endianness_probs} (bottom) payload plot, where each row denotes a byte with labeled bit indices. 
Let $E(j)\in \{B, L\}$ denote that byte $j$ is big, little endian, respectively. 

\begin{defn}[Valid Tokenizations]
\label{def:valid-tokenization}
For a given ID trace, define a \textit{valid tokenization}
$T$ as a tuple of candidate signals $\{I_k\}_k$ and endiannesses of each byte $ \{E(j)\}_{j=0}^7$ such that \\
(1) $\bigcup I_k = \{$0, \dots, 63$\}$ (all 64 bits are used),\\% \{$non-constant bits$\}$ (all non-constant bits are used),\\
(2) $I_k \bigcap I_l = \emptyset$ for all $k\neq l$ (signals do not overlap), \\
(3) Assumption (A1.b), one endianness per byte, is satisfied (implicit in the notation $E(j)$). 
\end{defn}

\begin{example}
\label{ex:boundary} 
Consider Fig. \ref{fig:endianness_probs} (bottom), a signal plot layout depicting a valid tokenization with one color per signal (and constant bits in grey).  
The \textcolor{Blue}{\textbf{navy}} signal, a 10-bit little endian signal starting at bit 0, is denoted 
% $I = (B_{14}, B_{15}, B_0, \dots, B_7)$;
$I = ({14}, {15}, 0, \dots, 7)$. 
Because, $B_{15}\to B_0,$ necessarily $ E(0) = E(1) = L$. 
\end{example}

Example \ref{ex:boundary} shows that if a signal $I$ crosses a byte boundary, the endianness of both bytes  is determined by the order of the indices according to Eq. (\ref{eq:bit-orderings}). 
This leads to the following definition and proposition, which will play an important role in the computational tractability of our optimization problem. 
% Such implications lead to important limitations in the sequences of valid endianness sequences $E(j).$

\begin{defn}[Byte Boundaries]
\label{defn:bytejoins} 
For $j = 0, \dots, 7$ let $v(j) \in \{J_B, J_L, C\}$ denote whether byte boundary $j$ is
\begin{itemize} 
\item a cut $(C)$: bit $[8(j+1)-1]$ ends a signal or is constant,
\item a big endian join ($J_B$): $[8(j+1)-1]\to 8(j+1), $ or
\item a little endian join $(J_L)$: $[8(j+1)-1]\to 8(j-1)$
\end{itemize}
and $V:= \{v \in \{J_B, J_L, C\}^8 \mid v$ is valid byte boundary set$\}.$
\end{defn}

For bits not on a byte boundary ($i\notin S:= \{8j-1\}_{j=0}^7$), there are only two options: cut or join $B_i \to B_{i+1}$. Both are valid possibilities regardless of endianness. 

\begin{prop} 
\label{prop:joins}
A valid tokenization $T$ has $v$ satisfying: 
\begin{enumerate}
\item $v(j) = J_B \implies %[8&(j+1)-1]\to 8(j+1) 
 E(j) = E(j+1) =  B $
\item $v(j) = J_L \implies %[8&(j+1)-1]\to 8(j-1)  
E(j-1) = E(j) =  L $
\item $v(0) \neq J_L$ 
\item $v(7) \neq J_B$
\item $v(j) = J_B \implies v(j+1) \neq J_L, v(j+2) \neq J_L$
\end{enumerate}
\end{prop}
\begin{proof}
(1) and (2) follow directly from Eq. (\ref{eq:bit-orderings}) (endianness definition) and assumption \textbf{A1.b} (one endianness per byte). 

For (3), $v(0) \neq J_L$ else $0\to -8\notin [0,63]$---similarly for (4). 

For (5), if $v(j) = J_B$ and either $v(j+1) = J_L$ or $v(j+2) = J_L$, then (1) and (2) imply $E(j+1)$ is both big and little endian, a violation of assumption \textbf{A1.b}. 
\end{proof} 
\vspace{-.25cm}
\begin{rmk}
\label{rmk:v}
Proposition \ref{prop:joins} can be summarized by defining $V:= \{v\in\{J_B, C\} \times \{J_B, J_L, C\}^6 \times \{J_L, C\}$ with no consecutive subsequences of the form $(J_B, J_L)$ or $(J_B,  * , J_L) \}$.
\end{rmk}

\begin{defn}[$\mathcal{T}$ \& $\mathcal{T}_v$]
Let $\mathcal{T}$ denote the set of valid tokenizations.
For $v\in V$  let  $\mathcal{T}_v \subset \mathcal{T}$ be the tokenizations with byte boundaries defined by $v$.  
\end{defn}

\begin{cor}
\label{cor:counting} 
There are 
$|\mathcal{T}| =  |V| \times |\mathcal{T}_v| = 577\times 2^{64-8} \ \approx 4.16\mathrm{E}19$ valid tokenizations. 
\end{cor}
\begin{proof} 
 $| \{J_B, C\} \times \{J_B, J_L, C\}^6 \times \{J_L, C\}| = 2^2 \times 3^6,$ and removing subsequences of the form $(J_B, J_L)$ or $(J_B,  * , J_L)$ leaves 577.  $|\mathcal{T}_v| = 2^{64-8}$ as the remaining $64-8 $ bit gaps have two valid options: cut or join. 
\end{proof} 
\vspace{-.25cm}

%% -- -- -- -- %%

\subsubsection{Optimization Formulation}
The output from Step 1 provisions $f(i | E(j_i))$ = $P ($cut to the right of bit $i$ for endianness $E(j_i))$, with $j_i = \lfloor i/8 \rfloor$ denoting the corresponding byte index for bit $i$. 
We set $f(i, e) = \infty$ if bit $i$ is to the left of a mandatory cut (e.g., the next bit is a constant bit).   
For intuition in the formulation below, consider $f(i| E(j_i) )$, not as the likelihood of a cut, but as penalty for not cutting, and let $\beta$ be a fixed cut penalty parameter. 

The idea for our cost function is to let signals accrue a join penalty---the sum of the probabilities $f(i|E(j_i))$ for each bit that is not cut in order to form the signal. 
Because the candidate signal entails a cut to the right of its LSB, we swap $f(LSB, E(j_i))$ for $\beta$, the cut penalty.
Thus, the $\beta$ controls how liberal to be with cuts. 

The intuition is to find the optimal balance between partitioning the message into too many signals and joining multiple disparate signals by balancing the cut penalty ($\beta$) with the likelihood of a cut (join penalty $f$). 
Setting $\beta = 1$ will lead to cutting only where $f(i|\cdot) = \infty$ (signals demarcated by constant bits), and $\beta = 0$ will lead to a cut at every gap, resulting in 64 1-bit signals. 

% We achieve this by balancing the join and cut penalties. 
% In computing the \textit{signal penalty}, we sum the probabilities of all but the last bit bit in the signal, incurring the join cost of the signal, and we replace the boundary probability of the least significant bit, with the cut penalty, ensuring that a signal with a low penalty will consist of low probabilities for in between internal bits, and a high probability for the a cut to the right of the least significant bit. 

\begin{defn}[Costs]
Define the \textit{Signal Cost} as 
\begin{equation*} 
\label{eq:signal-penalty} 
\phi (I, E) :=   
\underbrace{ \sum_{i \in I\backslash\{LSB\}} f(i |E(j_i)) }_{\text{\textit{join penalty}}} \  + \underbrace{\vphantom{\sum_{i \in I \backslash \{LSB\}}} \beta}_{\text{\textit{cut penalty}}}.
\end{equation*} 
% where parameter $ \beta \in [0,1] $ is tunable parameter.  
Extending to a Tokenization Cost, we have
\begin{align*}
\label{eq:schema-cost} 
\Phi(T):    &= \sum_{I \in T} \phi(I,E) \\
            &= \sum_{\chi_T(i) = 0} f(i| E(j_i)) + \sum_{\chi_T(i) = 1} \beta\\
            &= \sum_{i=0}^{63} (1-\chi_T(i))f(i| E(j_i)) + \chi_T(i) \beta
\end{align*}
% \clearpage
with $\chi_T(i) = 1 $ if $i$ is an LSB of a token in $T$, else $0$. 
\end{defn}

The above definition sets up our optimization problem: identify the \textit{optimal tokenization}
% $T_0 := {\arg\min}_\mathcal{T}  \Phi(T).$ 
\begin{equation}
\label{eq:optimization-problem}
  T_0 := \underset{T \in\mathcal{T}}{\arg\min }\  \Phi(T) \; .
\end{equation}

% \vspace{3cm}

\begin{example}
% Consider Fig. \ref{fig:endianness_probs} .
Refer to Fig. \ref{fig:endianness_probs} and
consider using the cost function to make a local endianness decision for byte 4, comparing the two overlapping 11-bit candidate signals that both contain byte 4 (bits 32 to 39 as numbered in the bottom %right 
plot): 
a big endian signal $I_0 = (29, \dots, 31, 32,\dots, 39)$ and a little endian signal $I_1 = (32, \dots ,39, 24,\dots, 26)$.  
Using the big $f(\cdot | E = B)$ and little $f(\cdot | E = L)$ endian probabilities depicted in the left and right plots, respectively, penalties for these candidate signals are $\phi_{\beta, f}(I_0, B ) = .02+.01+.98 + \beta = 1.01 + \beta$ and  $\phi_{\beta, f}(I_1, L) =.01 + \beta$. Because $ .01 + \beta < 1.01 + \beta$, $(I_1, L)$ has a lower penalty (regardless of the choice of $\beta$), it is locally optimal. 
In fact, $(I_1, L)$ turns out to be in the globally optimal $T_0$, which is shown in the bottom plot in \textcolor{SeaGreen}{\textbf{teal}}. 
\end{example}
% If we consider the signal penalties (Eq. \ref{eq:signal-penalty}) of the two possible 16-bit signals (bytes 4 and 5), $I_0 = [32, \dots, 47]$, $I_1 = [40, \dots ,47, 32,\dots, 39]$, we get $\phi_{\beta, f}(I_0, 0 ) = 1 -.2 + \beta = .8 + \beta$, and  $\phi_{\beta, f}(I_1,1) = 1.1 - 1 + \beta = .1 + \beta$, thus the the big endian signal has a lower signal penalty for all $\beta$.
%Since $.8 + \beta > .1 + \beta$ for all $ \beta In [0,1]$, we would choose the big endian signal which has a lower penalty, regardless of the choice of $\beta$. 

\vspace{-.2cm}
\begin{figure}[t]
    \centering
    \includegraphics[width=.21\textwidth]{figs/endianness_opt_prob_be_eg_payload.pdf}
    \includegraphics[width=.21\textwidth]{figs/endianness_opt_prob_le_eg_payload.pdf}
    \includegraphics[width=.25\textwidth]{figs/endianness_opt_eg_payload.pdf}
    \caption{\textbf{Top:} Probabilities of boundaries according to big endian ordering \textbf{(left)}, little endian ordering (\textbf{right)}. \textbf{Bottom:} The resulting optimal tokenization using $\beta=.6$ is three little endian (\textcolor{Blue}{\textbf{navy}}, \textcolor{Cerulean}{\textbf{blue}},  \textcolor{SeaGreen}{\textbf{teal}}), one big endian (\textcolor{SpringGreen}{\textbf{lime}}) and a 4-bit (\textcolor{Maroon}{\textbf{maroon}}) signal.}
    \label{fig:endianness_probs}
\end{figure}

%% -- -- -- -- %%

\subsubsection{Finding an Optimum} 
Given a cut penalty $\beta\in [0,1]$ and 
precomputed cut probabilities---$f(i | E(j_i) )$ for all $i \in\{0, \dots, 63\}$ and both endiannesses $E(j_i)$ (see Step 1, Section  \ref{sec:cutprob})---our goal is to identify an optimal tokenization (Eq. \ref{eq:optimization-problem}) from the $4.2\mathrm{E}19$ valid options.

\begin{thm}
\label{thm:optimization} 
Fixing $v\in V$, where $v$ gives cuts/joins at byte boundaries (bits in $S = \{8(j+1)-1\}_{j=0}^7$), the subproblem
$$\underset{T \in\mathcal{T}_v}{\arg\min }\  \Phi_{\beta, f}(T) $$ is realized by $T_{0,v}$, the tokenization: for all $i\in [0,63]\backslash S$, bit $i$ is an LSB (cut to the right of bit $i$) iff $\beta < (f(i|E(j_i))$.
% is realized by $T_{0,v}$, the tokenization with an LSB on (cut to the right of) bit $i$ iff $\beta < (f(i|E(j_i))$ for all $i\in [0,63]\backslash S$.
\end{thm} 
\vspace{-.5cm}
\begin{myproof}
Let $T_{0,v}$ be defined as above and $T\in\mathcal{T}_v$. By definition, for $i\notin S,\ T$ will accrue cost $\min(f(i| E(j_i)), \beta)$. 
Because $T, T_{0,v} \in \mathcal{T}_v$ both accrue the same cost for bits $i\in S,$
it follows that
\begin{alignat*}{2} 
\Phi(T)-\Phi(T_{0,v}) &= \sum_{i \notin S} && \big [(1-\chi_T(i))f(i| E(j_i))  \\
& && + \chi_T(i) \beta - \min(f(i| E(j_i)), \beta) \big ] \\ 
&\geq 0 \; . && \phantom{qedspaceqedspaceqedspace} \qedhere
\end{alignat*}
\end{myproof}
% Since $v$ defines the cuts/joins for the byte boundaries, $T$ and $T_0$ may only differ on cuts/joins in the remaining bit gaps,  $S$.
% By definition, $T_0$ will accrue $\min(\beta, f(i, E(j_i)))$ for all $i\in S$, hence $\Phi(T_0)\leq\Phi(T). $

This gives an efficient, constant time search algorithm (689 operations) by (1) storing the optimal cut/join choice for each bit $i\in [0,63]\backslash S$ under each endianness ($56\times 2$ operations), then (2) applying Theorem \ref{thm:optimization} to realize both $T_{0,v}$ and cost $\Phi(T_{0,v})$ for each of 577 $v\in V$ and maintaining the minimum. 

In the case that there are multiple optimal tokenizations, we break ties by choosing the one with the maximum number of cuts, followed by the minimum number of little endian signals, which necessarily furnishes a unique optimal solution. This tie-breaking scheme was chosen because we desired a scheme that involved a simple local decision that favored cutting over joining (less information loss) and big endian signals over little (since big endian signals are far more common). Experimentation indicated that prioritizing the former rule over the latter yielded better results. 

After experimenting with adjusting the tuning parameter $\beta$, we found that $\beta \in [.5, .7]$ yielded fairly consistent and correct tokenizations, so for our pipeline we chose $\beta=.6$. 
Note that the heuristic classifiers in Step 1 provide probabilities in $\{0,1\}$, meaning all choices of $\beta$ yield identical results. Furthermore, note that with binary inputs, a tie-break scheme is often necessary, whereas with high-precision probability inputs, multiple optimal tokenizations with the same cost are virtually impossible. 

The outputs of the endianness optimizer described in this step are tokenized signals. Although in theory another endianness optimizer could be developed and exchanged for this component, we consider this custom optimization to be a fixed and noninterchangeable component of the pipeline. 

% \begin{algorithm}[!h]
%  \caption{Find Optimal Tokenization}
%   \label{alg:optimization}
%  \textbf{Inputs}: f, \beta, V\\
% cuts \gets \{
% T\gets \{\}, Phi \gets \{\}
% \For{i \in [0,63]\backslash S}{
%   If{\beta < (f(i|E(j_i))}{
% \For{v \in V}{
%     T[v] = 

%       T[v]
%       }
%   }
 
    
%   \Return \texttt{Signed}
%   }
%     \If{$P(B_{i_0}, B_{i_1} = 1,0) + P(B_{i_0}, B_{i_1} = 0,1) < \gamma$}{
%   \Return \texttt{Signed}
%   }
%   \Return \texttt{Unsigned}
% \end{algorithm}


% Since endianness defines the neighboring bits, the likelihood of cutting at each gap will, in general, change with endianness assumptions. 





% While the size of $\mathcal{T}$, the set of possible valid signal packing schemes is very large ($\mathcal{O}(2^n)$), this search space can be reduced significantly by using assumption (\textbf{A1.b}), that is, that a single byte cannot contain two signals of different endianness. Equivalently, we can choose the endianness for each byte, so we can then we can solve this optimization problem for each byte independently. This insight making the optimal signal within a byte straightforward. For each within-byte bit (bits $i$ for which $i \% 8 \neq 0 $), we will chose to cut if $f(i, e_i) > \beta$ where $e_i$ is determined by the endianness of the byte. Regardless of the packing scheme, $T$, under consideration, Eq. \ref{eq:signal-penalty} is a sum over each gap of one of three values: $\beta$, $f(i,0)$ or $f(i,0)$. Now, if we know the endianness $e$ of a byte for all within-byte gaps, this is a binary decision between $\beta$ and  $f(i,e)$. Because 
% %the cost for each byte $k$ will simply be $\phi_{\beta, f}([8k,\dots , 8k+7], e_k)$ where $e_k$ is endianness of byte $k$.
% All that remains then, is how to choose the endianness for each byte, and to consider the signals that cross byte boundaries. These in fact both controlled by the following the ternary decision at each byte boundary: join as  big-endian (e.g. $23\rightarrow 24$), join as little endian (e.g. $23\rightarrow 8$), or cut (e.g. $23\rightarrow |$). 

% This decision then determines byte endianness. Explain.

% Note that we are able to say this because of the relatively local scope of our features (none have scope that span more than two bytes)

% Search over byte boundary decisions, and still get globally optimal solution. Explain how this works in practice, leads to why we use max prob = 8. 
% While it may appear at first that the size of $\mathcal{T}$, the set of possible valid tokens is very large ($\mathcal{O}(2^n)$), the search space is in fact significantly smaller than this due to Assumption (A1.b). 
% By leveraging some properties of the sums in the optimization, we are able to reduce the search space to $\approx 200$ schemes. 
%that is, that a single byte cannot contain two signals of different endianness
% To find $T_0$, we simply grid search over these packing schemes and find the one with minimal score. 

% After Step 2 each ID's message is \textcolor{Plum}{tokenized}.   


% Because the probabilities output from Sec. \ref{sec:cutprob} require features that are dependent on bit order, we employ two probabilities for each gap ($i$, one corresponding to the entire ID trace in big endian order, 
%(i.e. $[B_0,\dots, B_{63}]$), 
% and one corresponding to the entire ID trace in little endian order
%(i.e.  $[B_{56},\dots, B_{63}, B_{48},\dots, B_{55}, \dots, B_0, \dots, B_7] $). 
% (see Eq. \ref{eq:bit-orderings}).  
% This allows us to consider both big and little endian signals at each byte boundary. 



% Define byte boundary gaps as $i \% 8 = 0 $ for $i = 0 \dots 63$, all other gaps are within-byte gaps. For the within-byte gaps, the decision is binary: to join ($i\rightarrow i+1$), or to cut ($i\rightarrow |$). However, for the byte boundary gaps, the decision is ternary: join as  big-endian (e.g. $23\rightarrow 24$), join as lil-endian (e.g. $23\rightarrow 8$), or cut (e.g. $23\rightarrow |$). Ref above fig. 

%However, when we look at the actual optimal tokenization $T_0$ in Fig. \ref{fig:endianness_probs} (right), we see that $(32,16,1) \notin T_0$. \fix{This shows that we cannot make this decision locally, we must search over this enormous search space of every possible set of tokens in order to find the optimal solution. This is a $\mathcal{O}(2^n)$ problem, so we seek to reduce the size of this search space while still achieving the global optimal by using some of our assumpuptions listed in \ref{sec:problem}}. 


% If the boundary probability for a particular bit is too high, then we will choose to replace it with the 

% If we consider that each gap label $f(i)$ maps to the 

% that we wish to find a balance between labeling every gap as a boundary, and labeling no gaps as boundaries. This is precisiely 



% \add{Add lambda bounds proof: 
% little proof showing that $\beta = 1$ will lead to cut nowhere (except along constant bits), and $\beta = 0$ }


% \unsure{TBD on whether it is necessary to explain how start bits are indicated differently for little and big endian signals. }



% \subsubsection{Simplification for Shrinking Search Space}
% \textit{Explain how Assumptions inform the "Possible Search Space" and allow for a much smaller search space by just looking at byte boundaries.}


% There are 63 gaps to make a decision on. These can be partitioned into the following: Define byte boundary gaps as $i \% 8 = 0 $ for $i = 0 \dots 63$, all other gaps are within-byte gaps. For the within-byte gaps, the decision is binary: to join ($i\rightarrow i+1$), or to cut ($i\rightarrow |$). However, for the byte boundary gaps, the decision is ternary: join as  big-endian (e.g. $31\rightarrow 32$), join as little endian (e.g. $31\rightarrow 16$), or cut (e.g. $31\rightarrow |$). 
% In the example in \ref{fig:endianness_probs}(left), we see that the gap 31 was joined as little endian ($31\rightarrow 16$). 

% Suppose for the moment we are only using features that depend on bits directly to the left and to the right of a gap. Note, this is well defined for within-byte gaps. The optimal choice for each of these gaps can be independently decided. For byte boundary gaps, the neighboring bits are defined by the endianness of the bytes. However, local optimization even when considering all three options is insufficient. For example, if one chooses to join bit 23 as little endian ($23\rightarrow 8$), one cannot simultaneously choose to join bit 7 as big endian ($7\rightarrow 8$). so the decisions at the boundaries cannot be made independently, must look at all combos for globally optimal. 

% Above bullet leads to def of possible token schemes for byte boundaries (no ys, 8s, or impossible endpts)

% Now remove local feature assumption (altho still limits on this, feature scope is still less than 8 bits). If you have non local features, we must learn cut probabilities for both big endian and little endian neighbors. Specifically, when considering a tokenization schema with a big endian byte boundary, big endian probabilities should be used for joined bytes $\dots$. Then explain choice when cut is made (based on next boundary choice). If cut on both sides, then big endian. Explain how assumption 2b allows this simplification.

% % \begin{itemize}
% %     Item There are 63 gaps to make a decision on. These can be partitioned into the following: Define byte boundary gaps as $i \% 8 = 0 $ for $i = 0 \dots 63$, all other gaps are within-byte gaps. For the within-byte gaps, the decision is binary: to join ($i\rightarrow i+1$), or to cut ($i\rightarrow |$). However, for the byte boundary gaps, the decision is ternary: join as  big-endian (e.g. $23\rightarrow 24$), join as lil-endian (e.g. $23\rightarrow 8$), or cut (e.g. $23\rightarrow |$). Ref above fig. 
% %     % Item Features are the inputs used to decide the probability of a cut in a gap between bits. If features encoded only local information (bits directly to the left and right of the gap), then all of the internal bits in a byte could be independently decided (no optimization needed). 
% %     Item Suppose for the moment we are only using features that depend on bits directly to the left and to the right of a gap. Note, this is well defined for within-byte gaps. The optimal choice for each of these gaps can be independently decided. For byte boundary gaps, the neighboring bits are defined by the endianness of the bytes. However, local optimization even when considering all three options is insufficient. For example, if one chooses to join bit 23 as little endian ($23\rightarrow 8$), one cannot simultaneously choose to join bit 7 as big endian ($7\rightarrow 8$). so the decisions at the boundaries cannot be made independently, must look at all combos for globally optimal. 
% %     Item Above bullet leads to def of possible token schemes for byte boundaries (no ys, 8s, or impossible endpts)
% %     Item Now remove local feature assumption (altho still limits on this, feature scope is still less than 8 bits). If you have non local features, we must learn cut probabilities for both big endian and little endian neighbors. Specifically, when considering a tokenization schema with a big endian byte boundary, big endian probabilities should be used for joined bytes $\dots$. Then explain choice when cut is made (based on next boundary choice). If cut on both sides, then big endian. Explain how assumption 2b allows this simplification.
    
% % \end{itemize} 

% \add{Should be noted somewhere that a signal that does not cross a byte boundary can be encoded as either bit or little endian, although technically this changes the start bit}

% \add{Note that in implementation we encode $Infty$ with an $INF_{PROB}=8$ because this is the max that the the sum over two bytes could differ by}

% % \add{Tie break scheme}

% % \add{We set $\beta = .801$}

==> CAN-D IEEE/23-signed-classification.tex <==
\subsection{Step 3: Signedness Classification}
\label{sec:signed_class}
% For each ID, we now have the optimal packing scheme giving a partition of the 64-bit message into the signals; i.e., we know the signal's  boundaries (equiv., start bit, length) and endianness. 
\vspace{-.15cm}
A signedness classifier takes a tokenized signal (start bit, length, endianness) and makes a binary decision on whether each signal of length greater than two is signed (using two's complement encoding) or unsigned. 
To develop our classifier, we followed a similar workflow to Step 1 (Section \ref{sec:cutprob}), experimenting with supervised classifiers and unsupervised heuristics. 
Because each signal is tokenized, and thus the LSBs and MSBs are now known, this problem is significantly simpler, and features can be developed per signal rather than per bit. 
However, after experimenting with several features and supervised classification methods, we found that a simple heuristic based on the the distribution of the two MSBs of the signal yielded better results than the supervised methods. Using this heuristic, described in Alg. \ref{alg:signed-heuristic}, we obtained almost perfect classification ($97.3\%$ F-score), so we chose to use this heuristic in the CAN-D pipeline rather than a learned model. 
%For the full set of results, see \hyperref[sec:appendix]{Appendix} Table \ref{tb:signed_classification_results}). 


The heuristic is based on how the two MSBs will behave if the signal is signed or unsigned. 
Let $B_{i_0}, B_{i_1}$ denote the MSB and next most significant bit of the signal. 
First, consider the probabilities of the center values, $P[(B_{i_0}, B_{i_1}) = (1,0)]$,$P[(B_{i_0}, B_{i_1}) = (0,1)] $. 
If a signal is signed, values close to zero $(B_{i_0}, B_{i_1})$ will be $(0,0)$ (small positives) or $(1,1)$ (small negatives), whereas values near extremes will be $(1,0)$ (near min) or $(0,1)$ (near max). 
A signal with a small probability of these values is therefore likely signed.
%We simply set a threshold of $.1$, and if the Benford Sum of a signal is below this threshold, we classify it as signed. 
Second, consider the probability of a jump  between extreme values, $P[(B_{i_0}(t_j), B_{i_1}(t_j)) = (0,0) \wedge (B_{i_0}(t_{j+1}), B_{i_1}(t_{j+1})) = (1,1)]$.
If a signal is signed, the two MSBs must flip from $(0,0)$ to $(1,1)$ when changing from a small positive  to a small negative value. 
However, if it is unsigned, flipping is unlikely to ever happen because it would entail changing from a very small value to a large one, resulting in a significant discontinuity. 
If this probability is 0, the signal is likely unsigned. We apply these two ideas as described in Alg. \ref{alg:signed-heuristic}: we set $\gamma = .2$ based on observations of data. 

After Step 3, Signedness Classification, each ID's  64-bit message is partitioned into signals, of which we know the start bits, lengths, endianness, and signedness.
Consequently, each signal can now be translated %\textcolor{SeaGreen}{\textbf{translated}} 
into a time series of integers, denoted by $s(t)$. No previous works have attempted signedness classification, so the signedness classifier presented in this section is currently the sole option for this modular component.

\begin{algorithm}[t]
\small
 \caption{\small Heuristic signedness classifier}
  \label{alg:signed-heuristic}
 \textbf{Inputs}: $\{B_{i_0}(t), B_{i_1}(t)\}_t$, $\gamma$\\
 \If{$P[(B_{i_0}, B_{i_1}) = (1,0)] + P[(B_{i_0}, B_{i_1}) = (0,1)] = 0$}{
   \Return \texttt{True}
  }
  \If{$P[(B_{i_0}(t_j), B_{i_1}(t_j)) = (0,0) \wedge$ $(B_{i_0}(t_{j+1}), B_{i_1}(t_{j+1})) = (1,1)] = 0$}{
   \Return \texttt{False}
  }
    \If{$P[(B_{i_0}, B_{i_1}) = (1,0)] + P[(B_{i_0}, B_{i_1}) = (0,1)] < \gamma$}{
   \Return \texttt{True}
  }
  \Return \texttt{False}
\end{algorithm}
% \vspace{-.5cm}

% \begin{table}[t]
%     \small
%     \centering
%     \begin{threeparttable}[]
%         % \caption{Aggregated Classification Metrics using LOOCV by CAN log, only scoring non-obvious boundary decisions (f$-$ set). \textbf{Top}: Classifiers with default Scikit-learn parameters. \textbf{Bottom}: The top performing Random Forest Model, with optimal parameters chosen using a grid search.}%
%         \caption{Aggregated Classification Metrics using LOOCV by CAN log, run with default Scikit-learn parameters.}%
%         %Note that the results from models with balanced class weights are not shown since these yielded worse F-scores.
%         % \textbf{Bottom:} Performance metrics for top performing classifier with optimal parameters chosen using a Grid Search and LOOCV.}
%         \label{tb:boundary_classifier_results}
%         \begin{tabular}{lrrr}
%         \toprule
%         {Classifier} &  F-Score &  Precision &  Recall \\
%         \midrule
%     Logistic Regression &     79.0 &       88.9 &    71.1 \\
%     SVC Linear          &     71.5 &       71.9 &    71.1 \\
%     SVC Poly            &     83.8 &       90.9 &    77.8 \\
%     SVC RBF             &     83.3 &       89.7 &    77.8 \\
%     SVC Sigmoid         &     43.3 &       45.7 &    41.1 \\
%     Decision Tree       &     91.3 &       89.4 &    93.3 \\
%     Random Forest       &     93.9 &       94.4 &    93.3 \\
%     KNN                 &     82.4 &       87.5 &    77.8 \\
%     MLP                 &     80.2 &       81.6 &    78.9 \\
%     AdaBoost            &     85.4 &       94.6 &    77.8 \\
%     NaiveBayes          &     79.8 &       68.0 &    96.7 \\
%     \midrule
%     \textbf{Heuristic}           &     \textbf{97.3} &       \textbf{95.7} &    \textbf{98.9} \\
%     \bottomrule
%     \end{tabular}
%         % \begin{tablenotes}
%         % \small
%         % \item[1] Default parameters were optimal
%         % \item[2]\texttt{max\_features=$\sqrt{n_f}$,  
%         % min\_samples\_Leaf=3, n\_estimators=200,
%         % max\_depth=5}
%         % \end{tablenotes}
            
%     \end{threeparttable}
% \end{table} 

==> CAN-D IEEE/24-diagnostic-matching.tex <==
\subsection{Step 4: Physical Interpretation}
\label{sec:diag-matching}
% \add{Bobby write this sections:  for each signal (time series) and for each did trace/ sensor trace (time series) (1) interpolate them by sampling on the slower one; (2) fit signal to the sensor w/ linear regression and compute R value (3) accept if $R> \delta$. Mention that large $\delta$ means exact signals only, small $\delta$ allows for related but not exact signals to be discovered. (e.g...). Keep Notes at bottom of current section. 
% Reword what's below b/c it's in our other paper. } 

For our signal to time series matcher, we followed ACTT by Verma et al.  \cite{verma2018actt} to match a subset of the translated signals with diagnostic data. 
This augments matched signals with the necessary information to interpret them as actual measurements in the vehicles. 
We do this by comparing each signal time series $s(t)$ to each DID trace $D(t')$ and determining whether they are linearly related. 
Because the DID traces are sampled at a lower rate than normal CAN traffic, we interpolate the signal values over the diagnostic timepoints, obtaining $s(t')$. 
We then regress $D(t')$ onto $s(t')$ and find the best linear fit, furnishing the coefficients $a, b$ so that $\bar{s}(t) := a s(t') + b \approx D(t')$. 
To score the model's fit, we use coefficient of determination $R^2$, which measures the fraction of total variation in time series $D(t')$ that is explained by $\bar{s}(t')$.
% $\bar{s}(t')_{\{a,b\}}$, 
Thus, $R^2 = 1$ exhibits a perfect fit, and $R^2 = 0$ exhibits the fit of a horizontal line (assuming $D(t)$ is not the horizontal line). 
For each signal $s$, we find the diagnostic $D$ that yields the highest $R^2$ value. 
If $R^2 > \delta$, where $\delta \in [0,1]$ is a tuning threshold, $s$ is matched to $D$.
%%that controls the goodness of fit for match. % By tuning $\delta$, we control can control the fidelity of these matches: 
A $\delta = 1$ will return only perfectly matched signals, whereas a small $\delta$ will allow for signals with a lower $R^2$ score to be matched. % (related but not exactly matching signals to be labeled (BUT DISCLAIMER WE MIGHT BE SUPES WRONG!!!!!!!!). 
For our implementation, we chose $\delta=.5$. We echo Verma et al.~\cite{verma2018actt} that $\delta$ ``can be tightened to isolate near-perfect encodings, or tuned down to discover multiple related signals to each DID.''

It important to note that this matching is based on translated values and thus is independent of how the labeled time series (diagnostics) and signals are formatted or scaled. We reiterate that this means that the matching algorithm is able not only to recover signals that are sent in normal CAN traffic in addition to diagnostics (although often at much higher precision in the normal traffic), but also can recover signals that are not available in the diagnostics at all. For example, a signal relaying a binary indicator of brake pedal depression (not a diagnostic) may match to accelerator pedal position (DID 73) with a negative linear coefficient $a$. 

% Thirdly, the scoring mechanism is quite flexible.
% It can be easily altered to consider other binary encodings, more flexible regression, or other time-varying observations in addition to the DIDs. % or to apply different weighting schemes to increase the importance of certain features (e.g. weight values that changed w.r.t previous message more highly). 
 
For signals that match a diagnostic, we have interpretation,
%\textcolor{RoyalBlue}{\textbf{interpretation}}, 
having procured the label and units, as well as the scale $a$ and offset $b$. 
In additional to ACTT \cite{verma2018actt}, LibreCAN \cite{Pese2019librecan} (Phase 2) proposes signal to time series matching algorithms that could be used interchangeably (or even combined) for this component. 
% Finally, note that for any signals that are not interpreted, the first three steps provide translation into time series, which is indeed valuable in itself, as opposed to handling un- or mis-interpreted bits. 
Finally, note that translated signals that are not augmented with labels through this physical interpretation step are still highly valuable because there are many applications in which these unlabeled translated time series are far more useful than binary data. 


%See Fig. \ref{fig:qual_compare_paylods_signals} (a) middle plots, where each translated signal is annotated with the interpretation information from the matching diagnostic. 


% \begin{algorithm}[t]
%   \caption{Diagnostic Matching}
%   \label{alg:2}
%   \begin{algorithmic}
%   \Function{MakeIntegers}{$X, (j_s, j_e), bitOrder$}
%     % \For{$(j_s, j_e) \in V$}
%         \For{$i \gets 1, ..., n$}
%                 \State $x_{i} \gets \sum_{j=j_s}^{j_e}X_{i,j}2^{j_e-j}$ 
%         \EndFor 
%     % \EndFor
%     \State $\mathbf{x} \gets [x_1, \dots, x_n]$
%     \State \textbf{return} $\mathbf{x} $
%   \EndFunction
%   \end{algorithmic}
  
%   \smallskip
  
%   \begin{algorithmic}
%   \Function{CoefDeterm}{$\mathbf{y}, \mathbf{
%   \hat{y}}$}
%     \State $S_{tot} \gets \sum (y_i - \text{ave}(\mathbf{y}))$
%     % \State $S_{reg} = \sum (\hat{y}_i - \ave{\mathbf{y}})$
%     \State $S_{res}  \gets \sum (\hat{y}_i - y_i)$
%     \State $R^2 \gets 1 - (S_{res} / S_{tot})$  
%     \State \textbf{return} $R^2$
%   \EndFunction
        
%   \end{algorithmic}
  

  
%   \smallskip 
  
%   \begin{algorithmic}
%   \Function{LinearFit}{$\mathbf{x}, \mathbf{y}$}
%     \State $\mathbf{\tilde{x}} \gets $\Call{Interpolate}{$\mathbf{x}, \mathbf{y}$} 
%         \State  (Denote $\mathbf{x} = [x_1, \dots, x_n]$, $\mathbf{y} = [y(s_1), \dots, y(s_m)]$ and
%         \State interpolate over diagnostic times:   $\mathbf{\tilde{x}}=[x(s_1),\dots x(s_m)]$)
%     \State Find best fit $\mathbf{\hat{y}}_{\{a,b\}}$: $\min_{a,b} \norm{a\mathbf{\tilde{x}} + b - \mathbf{y}}_2^2$
%     % \State $R^2 = (\hat{y}_{\{a,b\}},y)$
%     \State $R^2 \gets $\Call{CoefDeterm}{$ \mathbf{y}, \mathbf{\hat{y}}_{\{a,b\}}$}
%     \State \textbf{return} $R^2, a, b$
%   \EndFunction
        
%   \end{algorithmic}
  
%     \smallskip
  
%   \begin{algorithmic}
%   \Function{MatchTraces}{$X, V, \mathbf{y}, \delta$}
%     \For{ $(j_s, j_e) \in V$ }
%         \State $\mathbf{x} \gets$ \Call{MakeIntegers}{$X, (j_s, j_e)$}
%         \State $ R^2, a, b \gets $ \Call{LinearFit}{$\mathbf{x}, \mathbf{y}$}
%         \If{$R^2 \geq \delta$} 
%             \State $M \gets M \cup \{(j_s,j_e, R^2, a, b)\}$ 
%         \EndIf
%     \EndFor
%     \State \textbf{return} $M$
%   \EndFunction
%   \end{algorithmic}
  
% \end{algorithm}
% Firstly, the goodness of fit for each model gives more than just a score of how well the model performs, but an indication of whether the token actually encodes the diagnostic signal
%Note that in order to get the true value measuring a physical signal, including units, we must apply the conversion for the matched diagnostic response, a formula accessible for these standardized DIDs \cite{obd2pids}.
% There are several important things to note about the matching algorithm. 
% Firstly, the goodness of fit for each model gives more than just a score of how well the model performs, but an indication of whether the token actually encodes the diagnostic signal. 
% In some cases it indicates that the CAN token is not an exact match, but does  encode a correlated signal, e.g., we have identified 1-byte tokens with high correlation to a continuously changing DID, presumably a binary indicator. 
% Hence $\delta$ can be tightened to isolate near-perfect encodings, or tuned down to discover multiple related signals to each DID. 
% We have have now reverse engineered complete signal definitions as described in Sec. \ref{sec:can-basics}: we extracted signals positions (start bit and length) in Sec. \ref{sec:cutprob}, endianessness in Sec. \ref{sec:endianess_opt}, signedness in Sec. \ref{sec:signed_class}, and the translation (label, unit, scale, offset) in Sec. \ref{sec:diag-matching}.


==> CAN-D IEEE/30-dataset.tex <==
 \section{Dataset}
\label{sec:dataset}
Because our goal is to build a vehicle-agnostic signal-extraction capability, we collected CAN data from 10 different vehicle makes and years ranging from 2010 to 2017 for training and evaluation. 
The details of defined signals for each log are described in Table \ref{tb:log_signal_stats}.
This dataset is far larger and more varied than any previous work. 
Notably, in order to test generalizability of the methods, no duplicate makes were included because different models of the same make (e.g., Toyota Camry and Corolla) have similar characteristics. 
%a wide variety of vehicles makes and years 
%Our full dataset for training and testing consists of 
%each collected from a different vehicle make, and 

% \subsection{Ground-Truth Data}
% \label{sec:ground_truth_data}



To obtain  data for our signal reverse engineering process (bit position, endianness, and signedness), we used DBCs acquired  from two sources. 
Log \#1 is from a vehicle that uses the J1939 standard \cite{J1979_201702}, a protocol for heavy trucks that provides signal definitions that are publicly available. We were therefore able to obtain absolute ground truth labels for the signals in this log. Because this log contains every type of signal (little endian, big endian, signed, unsigned) and we have absolute confidence in these labels, we consider this log to be the gold standard for testing. 

For logs \#2--10, we made use of CommaAI's OpenDBC project.\footnote{\url{https://github.com/commaai/opendbc}} 
% \cite{comma_opendbc}. 
This is an open, crowdsourced set of DBCs that was constructed by individuals using a CommaAI Panda device (an OBD-II plugin) along with the CommaAI Cabana interface to hand-label the data for their vehicle through trial, error, and visual inspection. 
OpenDBC includes DBCs for only a limited number of vehicles, and only a subset of IDs/signals for each vehicle is defined (see difference in IDs and Def. IDs in Table \ref{tb:log_signal_stats}). 
In particular, unobservable signals are often missing because these are created based on visual inspection. 

\begin{table}[t]
    \centering
    \caption{Statistics on 10 CAN logs, each collected from a vehicle of a different make.  For each log, we enumerate the following: nonconstant IDs (\textbf{IDs}), nonconstant IDs defined by CommaAI (\textbf{Def. IDs}), and each of the encodings of defined signals (big/little endian, signed/unsigned) resulting from ground truth labeling process (see Sec. \ref{sec:dataset}). Three logs contain a high percentage of little endian signals, and all but one contain signed signals.}
    \label{tb:log_signal_stats}
    \begin{threeparttable}
    \begin{tabular}{c r rrr rrr rrr r r}
    \toprule
    \textbf{Log} &  \textbf{IDs}\tnote{1} & \multicolumn{3}{c}{\textbf{Def. IDs}} & \multicolumn{3}{c}{\textbf{Unsigned, B.E.}} &  \multicolumn{3}{c}{\textbf{Signed}} &  \textbf{L.E.} &  \textbf{Total} \\
    \midrule
    \#1\tnote{2} &    54 &                 &17& &              &61& &       &3& &    25 &     89 \\
    \#2  &    66 &                          &14& &            & 143 & &      &21& &     0 &    164 \\
    \#3  &    35 &                          &7& &             & 50& &      &18& &     0 &     68 \\
    \#4  &    79 &                         &28& &             &181& &       &0& &     0 &    181 \\
    \#5  &    63 &                         &21& &             &111& &       &5& &     0 &    116 \\
    \#6  &    22 &                         &19& &              &72& &       &2& &    14 &     87 \\
    \#7  &    26 &                          &8& &              &53& &       &3& &     0 &     56 \\
    \#8  &    40 &                          &8& &              &98& &      &10& &     1 &    108 \\
    \#9  &    27 &                         &17& &              &56& &       &7& &    18 &     75 \\
    \#10  &    55 &                         &14& &             &136& &      &21& &     0 &    157 \\
    \bottomrule
    \end{tabular}
    \begin{tablenotes}
    \small
    \item[1] Nonconstant IDs: IDs with more than one nonconstant bit
    \item[2] Vehicle adheres to J1939 Standard protocol \cite{J1939_201308}, and signal definitions are derived from this open standard.
    \end{tablenotes}
    \end{threeparttable}
\end{table}


% The OpenDBC dataset also has a set of general DBCs for some manufactures, and customers can then leverage that signal definitions are often reused across models, years and trims, and using these as a starting point to then augment the signals that differ for that specific make/model/year. 

% We now describe our quality assurance and hand-labeling process.
% We selected vehicles to collect data from that had a closely matching CommaAI DBC (same manufacturer, similar model/year/trim). 
We collected data from vehicles that had a closely matching CommaAI DBC (same manufacturer, similar model/year/trim). 
Although CommaAI appears to do some measure of quality assurance on this data, because of the crowdsourced nature of the data, we must be mindful of the potential for mislabeled signals.
We performed quality control on this data using the following process. 
First, we partitioned each nonconstant ID trace into sequences of contiguous, nonconstant bits and label each as an unsigned, big endian signal. 
This provides a set of ``baseline'' signal definitions. 
Next, we parsed the data according to the DBC, trimming off any signal MSBs that were constant in our data because of extreme values not being reached, and redefined the signal to have the trimmed start bit and length. 
%We now consider the union of the signals in the Baseline and CommaAI DBCs, 

For IDs defined by CommaAI, we compared the baseline and trimmed CommaAI signal definitions.
If the definitions for the ID agree and pass a visual check,  we automatically added them to our ground truth DBC.
If they disagreed, we displayed the signal tokenization layout and signal time series' plots (see Fig. \ref{fig:qual_compare_paylods_signals}) side by side and identified the discrepancies.
If easily resolvable by experimentation and visual inspection (e.g., adding an obvious signal definition missing from CommaAI DBC, identifying an unsigned signal mislabeled as signed), we added the correct signal definitions to our DBC with minor errors fixed. 
If we were unable to resolve the discrepancy easily, we simply did not include the ID or signal in our ground truth DBC. 
For IDs that did not appear in the CommaAI DBC, we performed a similar process of visual inspection of the baseline plots, adding these definitions to our ground truth if easily resolved and discarding them if not. 

\begin{example}
For an example of this visual inspection process, consider Fig. \ref{fig:qual_compare_paylods_signals}(c), bytes 5 and 6. Suppose the trimmed CommaAI and baseline signal definitions yielded the top payload/signal plots (\textcolor{Maroon}{\textbf{maroon}} signal) and bottom payload/signal plots (\textcolor{Maroon}{\textbf{maroon}} \& \textcolor{Orange}{\textbf{orange}} signals), respectively. By inspection, we can clearly see that trimmed CommaAI definition (top) is correct (a two-byte little endian signal) because it results in a clear continuous  (\textcolor{Maroon}{\textbf{maroon}}) signal. Note that the baseline definition visualization is characteristic of a truncated signal's LSB (intermittently noisy/constant \textcolor{Orange}{\textbf{orange}}) and a signed signal (\textcolor{Maroon}{\textbf{maroon}} discontinuous near extreme values).
Thus, we would add the correct trimmed CommaAI definition. 
\end{example}

This process of visual inspection method is tedious and time consuming, but it is quite effective as  both legitimate signals and misclassified encodings (e.g., signed signals translated incorrectly as unsigned) %, or the Least Significant Byte of little endian signal) 
are usually recognizable from time series plots. 
In fact, our visual inspection process is quite similar to the CommaCabana interface used to create CommaAI DBCs. 
%Secondly, for two logs (\#4 and \#8)  we collected data from the exact model, trim, and year defined by the CommaAI DBC. 
% While non-comprehensive, all the signals defined by CommaAI appeared correct, and our process described above did not result in any modifications. 




% \begin{table}[t]
% \small
% \centering
% \caption{Statistics on seven CAN logs, each collected from a vehicle of a different make. \textbf{Top}: We list the time duration of each log, number of IDs seen over the course of the log (not including IDs with constant messages), and the total number of frames broadcast by these non-constant IDs. 
% \textbf{Middle}: We give the method by which we obtained the DBC for ground-truth labels (see Sec. \ref{sec:ground_truth_data} for details), and the number of non-constant IDs with message definitions provided by the DBC. 
% \textbf{Bottom}: We enumerate the number of each type of defined signal (signedness and endianness). }

% \label{tb:log_signal_stats}
% \begin{threeparttable}
% \begin{tabular}{lrrrrrrr}%{.48\textwidth}
% \toprule
% CAN Log &     1 &     2 &     3 &     4 &     5 &     6 &    7 \\
% \midrule
% %Vehicle Year             &  `15 &  `16 &  `17 &  `11 &  `17 &  `15 &  ? \\
% Length (min) &    38 &     7 &    12 &    29 &     9 &    14 &   16 \\
% IDs\tnote{1}            &    83 &    80 &    63 &    30 &    28 &    61 &   58 \\
% Frames ($\times1e6$)\tnote{1} &  6.4 &   .95 &  1.4 &  2.5 &   .49 &   .62 &  .67 \\
% \midrule
% DBC\tnote{2} &    C* &  C* &   C &    C* &    C &    C* &   J\\
% Defined IDs     &    39 &    72 &    37 &    11 &    26 &    51 &   36 \\
% \midrule
% Unsigned, B.E.        &   112 &   226 &   172 &    22 &    67 &   172 &   80 \\
% Signed           &    11 &     4 &     6 &     2 &     8 &    19 &    3 \\
% L.E.        &     0 &     0 &     0 &     1 &    18 &     0 &   17 \\
% Total            &   123 &   230 &   178 &    24 &    87 &   191 &  100 \\
% \bottomrule
% \end{tabular}
% \begin{tablenotes}
% \small
% \item[1] Only including non-constant IDs (IDs with non-constant messages), and frames sent by those IDs  \item[2] C = CommaAI OpenDBC\cite{comma_opendbc}, C* = CommaAI DBCs modified by quality assurance process,
% J = J1939 Standard protocol\cite{J1939_201206}
% %in heavy trucks that provides signal definitions (publicly available)
% \end{tablenotes}
% \end{threeparttable}
% \end{table}

% \begin{table}[t]
% \small
% \centering
% \caption{Statistics on seven CAN logs, each collected from a vehicle of a different make. \textbf{Top}: We list the time duration of each log, number of IDs seen over the course of the log (not including IDs with constant messages), and the total number of frames broadcast by these non-constant IDs. 
% \textbf{Middle}: We give the method by which we obtained the DBC for ground-truth labels (see Sec. \ref{sec:ground_truth_data} for details), and the number of non-constant IDs with message definitions provided by the DBC. 
% \textbf{Bottom}: We enumerate the number of each type of defined signal (signedness and endianness). }

% \label{tb:log_signal_stats}
% \begin{threeparttable}
      
% \begin{tabular}{lrrrrrrrrrr}
% \toprule
% {Log \#} &   1  &  2  &   3  &   4  &  5  &   6  &   7  &  8  &   9  &  10 \\
% \midrule
% Length   &    6 &   2 &    7 &   12 &   8 &   17 &   19 &   9 &   14 &  16 \\
% IDs           &   66 &  35 &   79 &   63 &  22 &   26 &   40 &  27 &   55 &  54 \\
% \midrule
% DBC            &    C &   C &    C &   C* &   C &    C &    C &  C* &    C &   J \\
% IDs*   &   55 &  20 &   61 &   23 &  21 &   19 &   28 &  20 &   45 &  33 \\
% \midrule
% \texttt{0+} &  143 &  50 &  181 &  111 &  72 &   53 &   98 &  56 &  136 &  61 \\
% \texttt{-}         &   21 &  18 &    0 &    5 &   2 &    3 &   10 &   7 &   21 &   3 \\
% \texttt{1}          &    0 &   0 &    0 &    0 &  14 &    0 &    1 &  18 &    0 &  25 \\
% Total          &  164 &  68 &  181 &  116 &  87 &   56 &  108 &  75 &  157 &  89 \\
% \bottomrule
% \end{tabular}

% \begin{tablenotes}
% \small
% \item[1] Only including non-constant IDs (IDs with non-constant messages), and frames sent by those IDs  \item[2] C = CommaAI OpenDBC\cite{comma_opendbc}, C* = CommaAI DBCs modified by quality assurance process,
% J = J1939 Standard protocol\cite{J1939_201206}
% %in heavy trucks that provides signal definitions (publicly available)
% \end{tablenotes}
% \end{threeparttable}
% \end{table}


==> CAN-D IEEE/40-evaluation.tex <==
\section{Evaluation}
\label{sec:eval}
Using the dataset described in Section \ref{sec:dataset}, we compared our algorithms, both with the heuristic\footnote{$\alpha_1 = .01, \alpha_2 = .5, \beta = .6$ (though irrelevant with binary Step 2 inputs),$ \gamma = .2, \delta = .4$.} and ML\footnote{Step 1 with tuned RF model found in Sec. \ref{sec:cutprob}, $\beta = .6, \gamma = .2, \delta = .4$.} for Step 1, against the following predecessors:  
TANG \cite{nolan2018unsupervised}\footnotemark, 
\footnotetext{TANG and ACTT incorrectly considered reverse bit ordering. We only consider forward bit ordering for these two methods.}
READ \cite{marchetti2019read},
ACTT \cite{verma2018actt}\footnotemark[\value{footnote}]\textsuperscript{,}\footnote{For the $R^2$ threshold, we used $0.4$.  For the 5/10 logs tested that contained no diagnostic packets; this method is equivalent to the baseline. %Therefore, results are actually even worse than reported. 
},
LibreCAN (Phase 0) \cite{Pese2019librecan}\footnote{
    The authors state that the optimal choice for parameter $T_{p0,2}$ (percent decrease of bit flip rates) was between $.01$ and $.02$ depending on the vehicle. The authors likely meant between $.1$ and $.2$, because a threshold of 1\% or 2\% would lead to (and we verified this)  a \textit{very} high false positive rate. 
    For the results reported,  $T_{p0,2} = .2$ was used, resulting in much higher F-scores. 
%Cue subtle dig at their claim that a single fixed param could reasonably be used for any dataset/vehicle. 
}. 
    %  Field Classification (maybe?) \cite{markovitz2017field}
See Section \ref{sec:related-works} for a description of each algorithm. Note that we did not test the algorithm proposed by Markowitz and Wool \cite{markovitz2017field} because it was tested by READ and shown to produce far inferior results. 
We also tested against a baseline method that simply uses constant bits as signal boundaries and assumes big endian, unsigned encodings. 
%cuts on the left of any constant bit; 
This represents accuracy scores obtained by simply identifying the obvious boundaries. 
% We include some notes on implementing the methods described in previous works, provide any choices we make for user set parameters, and include any details in which we deviated from the method described by the authors. 
% \fix{Method Implementation/setup/disclaimer section needs to be tightened}


% DISCLAIMER: Add any notes regarding adaptation and implementation of the other methods that may irritate any Italian or non-Italian researchers. 

In this section, we quantitatively compare the signal boundary classifiers (Step 1) proposed by each method (Section \ref{sec:eval-boundary-quant}, Table \ref{tb:compare} (top)), as well as the full tokenization and translation (Step 1--3) efforts of each (Section \ref{sec:eval-l1-error}, Table \ref{tb:compare} (bottom)). 
Recall that Step 2, Endianness Optimization, relies on boundary probabilities computed via Step 1 under both possible endiannesses and that Steps 1 and 2 together result in tokenization. 
Because the results of Step 2 are inherently tied to Step 1, we do not offer a stand-alone evaluation of our solution for Step 2. 
We also do not provide any comparative evaluation of Step 2 or 3 because no other methods propose algorithms for endianness optimization or signedness classification, although we did provide the classification metrics for our signedesss classifier (Step 3) in Section \ref{sec:signed_class}. 
% since the results of Step 2 are inherently tied to Step 1 (together these result in tokenization), we do not offer a standalone evaluation of our solution for Step 2. 
Moreover, we do not quantitatively evaluate the interpretation (Step 4) efforts by ACTT, LibreCAN, or CAN-D because, as pointed out by Pes\'{e} et al. \cite{Pese2019librecan}, ground truth interpretations are highly subjective and difficult to evaluate quantitatively.  
Instead, we offer a qualitative comparison of the full decoding efforts in Section \ref{sec:qual_results} and Fig. \ref{fig:qual_compare_paylods_signals}, which includes the supplemental interpretations given by CAN-D. We note that ACTT's interpretation is virtually identical to CAN-D's, and LibreCAN's requires an extra tool to obtain body-related labeled time series, so we did not attempt to perform their interpretation method.

Finally, we note that READ and LibreCAN make efforts to categorize signals, which is an added benefit of these methods over ours, but we do not evaluate the efficacy of their categorization algorithms.


==> CAN-D IEEE/41-quant_eval.tex <==

\subsection{Signal Boundary Classification Evaluation}
\label{sec:eval-boundary-quant}
We first quantitatively evaluated the signal boundary classification algorithms of each method using  three test sets that differ in the number of positive labels (detailed in Table \ref{tb:test_set_pos_labels}).
%, with 5784 negative labels for all sets. 

\begin{wraptable}[9]{r}{2.7cm}
 \fbox{%
   \begin{minipage}{\dimexpr2.7cm-2\fboxsep}
    \small
    \caption{Positive labels in each test set (5784 negative labels in all sets)}
    \label{tb:test_set_pos_labels}
        \begin{tabular}{l r r}
        \toprule
        {} &   {$n$} &  \% \\
        \midrule
        c  &   834 & 13\\
        f$-$ &   208&  3\\
        f$+$ &  1159 & 17 \\
        \end{tabular}
           \end{minipage}}
\end{wraptable} 
The condensed ``c'' set uses all positive labels (boundaries) in condensed traces (constant bits removed), thus increasing the number of nonobvious positive labels and decreasing class bias, resulting in the most robust evaluation set for testing and comparing the efficacy of signal boundary classification algorithms. 
In the full (noncondensed) ``f$+$'' set, all nonconstant samples are scored (including obvious examples of LSBs abutting constant bits/message ends). 
These full (noncondensed) f$+$ traces give a more accurate representation of the (very biased) distribution of labels and the most realistic setting for the positive and negative samples. 
This f$+$ set is the most representative and will yield the most realistic metrics for the total signals that could be extracted using a given method. 
Finally, in the full nonobvious set ``f$-$'', only nonobvious examples (those not abutting constant bits) are scored. This test set has very few positive labels (3\%), but unlike c, all are boundaries that delimit two adjacent signals in actual data, and unlike f$+$ will not result in score inflation from obvious boundaries not attributable to the algorithm being scored. 
The f$-$ set gives a balance of realism in use without the inflation of metrics from the obvious boundaries. 

To illustrate the differences in the three sets, suppose for the moment that bit 3 is the only constant bit observed in an ID's 64-bit data field; thus, bit 2 is necessarily the LSB of a signal, and bit 4 is the MSB of a signal. 
In the condensed testing set, c,  bit 3 is removed so bit 2 (LSB) and bit 4 (MSB) abut,  allowing  a positive example (i.e., a signal boundary that the algorithm will have to decide). Thus, c increases the ratio of positive examples in the data and allows more robust evaluation of whether the algorithm can identify signal boundaries. 
In this same case, the f$+$ set and the f$-$ set simply leave the constant bit (bit 3) in the dataset, allowing immediate and obvious identification of a signal boundary. 
The difference is that f$+$ indicates that this obvious signal boundary is counted during testing, whereas f$-$ indicates that it is ignored in testing because it is obvious (i.e., does not require inference based on neighboring bits). 
Thus, f$+$ scores indicate efficacy when used on real data, although the many obvious signal boundaries mask the performance of the classifiers. Sets c and f$-$ are included to provide this insight. 


\begin{table}[!b]
    \vspace{.2cm}
   \centering
    \begin{threeparttable}
\begin{tabular}{lccccccccc}
    & &  & \rotatebox{80}{\textbf{Baseline}} &  \rotatebox{80}{\textbf{TANG} \cite{nolan2018unsupervised}} &  \rotatebox{80}{\textbf{ACTT}\cite{verma2018actt}} & \rotatebox{80}{\textbf{READ} \cite{marchetti2019read}} &  \rotatebox{80}{\textbf{LibreCAN} \cite{Pese2019librecan} } & \rotatebox{80}{\textbf{CAN-D Heuristic}}& \rotatebox{80}{\textbf{CAN-D ML}}\\
\toprule
    \multirow{9}{*}{\rotatebox{90}{\textbf{Signal Boundary Classif.}}}
        &\multirow{3}{*}{\textbf{F}}
            &c     & 0.0 &  67.1 &   *      &  71.1 &      78.7 &            91.6 &     \textbf{93.5} \\
            &&f$-$ & 0.0 &  45.6 &  14.5    &  63.2 &      70.6 &            89.6 &     \textbf{91.2} \\
            &&f$+$ & 90.1&  84.9 &  89.6    &  94.4 &      94.2 &            98.1 &     \textbf{98.4} \\

    \cdashlinelr{2-10}
        &\multirow{3}{*}{\textbf{P}}
            &c     & 0.0   &  62.6     &    *    &  94.8 &      86.8 &            \textbf{97.2} &     96.4 \\
            &&f$-$ & 0.0   &  31.8     & 35.2    &  80.6 &      64.2 &            \textbf{89.9} &     87.6 \\
            &&f$+$ &\textbf{100.0} &  75.7 &  96.5     &  97.6 &      92.4 &            98.2 &     97.6 \\
    \cdashlinelr{2-10}
        &\multirow{3}{*}{\textbf{R}}
            &c     &   0.0 &  72.4 &   *        &  56.8 &      71.9 &            86.7 &     \textbf{90.8} \\
            &&f$-$ &   0.0 &  80.3 &    9.1   &  51.9 &      78.4 &            89.4 &     \textbf{95.2} \\
            &&f$+$ &   82.0&  96.5 &    83.7   &  91.4 &      96.1 &            98.1 &     \textbf{99.1} \\
\midrule \\
\midrule 
\multirow{11}{*}{\rotatebox{90}{\textbf{Mean $\ell^1$ Signal Error }}}
& \multirow{10}{*}{\rotatebox{90}{CAN  Log}}
    &\#1   &      18.9 &  30.0 & 18.9  &  20.9 &      25.4 &             4.0 &      \textbf{3.9} \\
    &&\#2     &      11.2 &  16.3 & 12.7  &   9.7 &      11.1 &             \textbf{0.7} &      1.9 \\
    &&\#3    &      20.9 &  25.6 & 20.9 &  19.8 &      20.5 &             \textbf{1.3} &      2.1 \\
    &&\#4    &       4.4 &  13.8 & 6.4  &   2.3 &       3.5 &             \textbf{1.3} &      1.7 \\
    &&\#5    &      11.9 &   8.9 & 11.9  &   8.8 &       3.7 &             3.3 &      \textbf{2.3} \\
    &&\#6    &      11.0 &  18.4 & 11.0  &  10.6 &       9.7 &             4.9 &      \textbf{3.4} \\
    &&\#7    &       6.1 &  16.4 & 7.9  &   5.5 &       7.6 &             \textbf{0.0} &      \textbf{0.0} \\
    &&\#8    &       9.4 &  16.7 & 9.4  &   7.9 &      10.2 &             \textbf{0.2} &      1.5 \\
    &&\#9    &      11.1 &  14.2 & 10.6  &  12.0 &      12.8 &             1.5 &      \textbf{1.2} \\
    &&\#10    &       9.8 &  14.1 & 11.3 &   7.9 &       9.9 &             \textbf{0.7} &      0.9 \\
    \cdashlinelr{2-9}
    &\multicolumn{2}{c}{Average} & 11.5 &  17.4 &  11.9 &  10.5 &      11.4 &  \textbf{1.8} &      1.9\\
\bottomrule
\end{tabular}
\caption{\textbf{Top:} Comparison of signal boundary classification results presented. \textbf{F} = F-score, \textbf{P} = precision, \textbf{R} = recall. 
We test each method using the three test scenarios, denoted in the third column and described in Sec. \ref{sec:eval-boundary-quant}.
% denoted in the third column:  c = `condensed' traces (obvious boundaries removed, best for testing signal boundary prediction), f$-$ =`full' traces (scoring only non-obvious boundaries, removes score inflation by obvious boundaries), and  f$+$ = `full' traces scoring all positive labels (unmodified CAN data, most representative for use). 
``Baseline'' identifies only obvious signal boundaries only at constant bits, which trivially has perfect precision.  
CAN-D ML achieves the highest F-score and recall, while the heuristic exhibits the best precision for all sets.  
Both exhibit over $\smalltilde$10\% improvement in recall over all previous methods in the two  difficult test sets (c, f$-$).
We do not evaluate ACTT under scenario (c); it relies heavily on constant bits to shrink the search space. 
\textbf{Bottom:} Mean $\ell^1$ error of translated signal values (Eq. \ref{eq:log_error}) reported for each CAN log, \#1--\#10 (described in Table \ref{tb:log_signal_stats}). 
CAN-D has lowest error on every log (often by far), exhibiting more than five times lower error on average, and almost five times times lower error on the ``gold-standard'' log \#1.
Averaged across all CAN logs, CAN-D is the only algorithm to substantially beat the baseline,
achieving perfect translation in log \#7.
% In fact, all previous methods are less accurate than Baseline on 3/7 logs, and are comparable to Baseline on average.
The most substantial decrease in error is on logs that have a high percentage of little endian (e.g., \#1, \#9) or signed (e.g., \#2, \#3) signals, demonstrating the efficacy of Steps 2 and 3.
Even on \#4, the lone log without little endian or signed signals, CAN-D exhibits at least $\smalltilde$ 50\% decrease in error from other methods.
Finally, note that while CAN-D ML has slightly higher average error than CAN-D heuristic (due mostly to worse precision in Step 1), it has lower error for all logs containing little endian signals (\#1, \#6, \#9), perhaps illustrating that the endianness optimization (Step 2) benefits from the probability inputs offered by the ML in Step 1. 
}
\label{tb:compare}
\end{threeparttable} 
\end{table} 



% \subsubsection{Datasets for Training and Tuning our Supervised Classifier}
% \label{sec:train-tune-sets}
% % To construct inputs to the boundary classification  (Sec. \ref{sec:cutprob}),
% % we preprocess our data to battle class bias in training and testing. %into three different test sets. 
% Recall from Sec. \ref{sec:cutprob}, we train our supervised boundary classification models on ``condensed'' ID traces (with constant bits removed). The motivation for %using these condensed traces in training is multifold: 
% this is threefold:
% (1) Based on assumption (\textbf{A0}) (see Sec. \ref{sec:problem}), observed constant bits necessarily delimit signals, so a simple rule suffices to identify these obvious signal boundaries.
% (2) Our features encode neighboring bits' values and flips, so when nearby bits are constant features are either trivial or undefined. 
% Removing the non-constant bits prior to feature building yields a better feature set. 
% (3) Classes are highly biased towards the negative class\textemdash most bits are not an LSB (not on a signal boundary). 
% By removing constant bits, we artificially increase the number of non-obvious signal boundaries and decrease class bias particularly for the non-obvious examples for which a classifier is needed.  
% % When training a model, removing these bits prior to feature building yields a better feature set, allowing the classifier to learn on more examples of boundaries between two adjacent signals, which are precisely the non-obvious examples for which a classifier is needed. 
% This is the ``c'' set  described in Sec. \ref{sec:eval-boundary-quant}.


% When tuning the model, we only score examples that were non-obvious---not abutting a constant bit in the ``full'' non-condensed trace---since we ultimately wish to apply the model to full 64-bit traces and want to optimize performance for this scenario. 
% This set is the  ``f$-$'' set described in Sec. \ref{sec:eval-boundary-quant}. 
% % In testing on this condensed data, we increase the number of positive labels on which we can evaluate a signal boundary identification algorithm, in particular, the non-obvious boundaries. 
% % In testing, condensing the data increases the number of non-obvious labels and decreases class bias, improving the evaluation set.
% % This condensed dataset is the best test set for the efficacy of signal boundary prediction algorithms. 


The classification F-score, precision, and recall for each scenario are reported in Table \ref{tb:compare} (top). Recall that because little endian signals are split on the byte boundary into two big endian signals for labeling, we test only the efficacy of the signal boundary classification methods without taking endianness into account, 
thus not penalizing other algorithms for the limiting assumption of big endianness. Also note that because CAN-D is supervised, reported metrics are from aggregating results from LOOCV per log.

\subsection{Signal Error Evaluation}
\label{sec:eval-l1-error}
Second, we compare the full tokenization and translation efforts of each method, computing the $\ell^1$ error between the translated signals and their corresponding ground truth signals. 
Results are shown in Table \ref{tb:compare} (bottom).  
The motivation for this evaluation is that ultimately, the goal of all of these methods to extract time series that can be used as actual real-time measurements from systems in the car. 
Therefore,  the most important metric for measuring the efficacy of these methods is not how many bits overlap or the number of boundaries correctly classified (as described above), but the difference between the values of the extracted signal's time series and the true signal's time series. 
All previous methods assume big endian, unsigned signals; consequently, once signal boundaries are assigned, the translated signal values are completely determined, and this is what is used for this second evaluation. For CAN-D, Steps 2--3, Endianness Optimization and Signedness Classification, provide the remaining tokenization and translation information. 

We compute the score for each log as follows. 
Let $S$ denote the set of normalized true signals and $\hat{S}$ the set of normalized predicted signals (all taking values in [0,1])  for a CAN log. 
Let $\eta:S\to\hat{S}$ so that for each true signal, $s$, $\eta(s)$ is the predicted signal that contains the MSB of $s$. 
Any predicted signals that are left unmatched ($\forall \hat{s}\in\hat{S}\backslash \eta(S)$) are paired with the zero vector $\vec{0}$. 
Take the normalized $\ell^1$ difference between each signal pair, resulting in a signal error between 0 and 1. 
The \textit{mean signal error for the log} is defined as
\begin{equation}
    \label{eq:log_error}
       \sum_{s\in S} \|s-\eta(s)\|_1 + \sum_{\hat{s}\in \hat{S}\backslash\eta(S)} \|\hat{s}\|_1 \; , 
    %  \sum_{s\in S} \left(  \sum_{t = 1}^{n_s} \frac{|s(t) - \eta(s)(t)|}{n_s} \right) \sum_{\hat{s}\in \hat{S}\backslash\eta(S)} \left(  \sum_{t = 1}^{n_{\hat{s}}} \frac{|\hat{s}(t)|}{n_{\hat{s}}}\right)
\end{equation}
where $\|s\|_1:= \sum_{t = 1}^{n_{id}} |s(t)|/n_{id}.$
% Note that using this scoring, there will be one summand per ground-truth signal, and a summand for each extra signal (penalizing spurious signals).
 %oh hai!



==> CAN-D IEEE/42-qualitative-results.tex <==
\subsection{Qualitative Results}
\label{sec:qual_results}
Fig. \ref{fig:qual_compare_paylods_signals} depicts three examples of messages decoded by CAN-D (identical decodings for the ML and heuristic signal boundary classification) and by the most accurate competing methods (READ and LibreCAN, which both produce the same signal boundary predictions for these examples)  with detailed descriptions and discussion. 
These examples illustrate a message with 
signed and unsigned signals (top), 
little endian unsigned signals (bottom left) 
and little endian (signed and unsigned) signals (bottom right). 
CAN-D correctly tokenizes and translates all examples depicted and overall furnishes interpretable time series. 
Where available, CAN-D's physical interpretation  (Step 4, Section \ref{sec:diag-matching})  is provided in annotations above signals, showing $R^2$ value to gauge goodness-of-match. 
Overall, mistokenization and mistranslation by other methods resulted in rampant discontinuities and dramatic error in most time series, exhibiting the necessity of correctly identifying each signal's endianness and signedness. 

We also attempted to find common attributes of the incorrectly classified signals by CAN-D and found that two key characteristics that lead to higher signal error. 
First, discontinuous signals or discrete signals are often incorrectly split into multiple signals. 
Most commonly, this seems to occur for CAN signals that are mapped to enumerated choices known as ``enumeration value types'' \cite{vector_candb_docs} (e.g., a gear shift signal with the mapping $\{2:\texttt{P}, 4: \texttt{R}, 8 : \texttt{D}, 16: \texttt{L}\}$). Secondly, short (1--3 bit) abutting signals that move together are sometimes incorrectly joined together because of the fact that the bit flips of adjacent MSBs and LSBs of these signals are highly dependent. Importantly, other methods appear to have similar shortcomings. 
% Interestingly, the \textcolor{MidnightBlue}{\textbf{navy}} signal at bit 4, matched to DID `Accelerator pedal position D' with $R^2 = .53$. This is likely a binary indicator of acceleration; thus, we have interpreted a signal that is not a diagnostic. 
% extracted interpretation information for a signal related to a diagnostic, 

% The bottom left plots show a message with four speed-related, little endian signals that are (necessarily) mistokenized  by other methods.
% %due to their inablilty to handle little endian tokens. 
% % TANG yields a similar translation to READ and LibreCAN but chops off bits 7 and 39 into 1-bit signals.
% The competing methods wrap the three most significant bits of each correct signal incorrectly at the byte boundary, attributing them to the wrong signal.
% Yet, for the \textcolor{cyan}{\textbf{light blue}}, \textcolor{green}{\textbf{green}}, and  \textcolor{Orange}{\textbf{orange}} signals the plots appear nearly correct as all signals are close in value, and quantitative signal error evaluation above would have yielded near perfect results.

% The bottom right plots show results of a message with four little endian steering-related signals of varying signedness.
% Competing methods incorrectly identify tokenize and translate all signals, and the results are noisy. 
% Notice the scale of the translated time series for the top \textcolor{MidnightBlue}{\textbf{navy}} signal.
% The big endian assumption of the other methods mis-attributes the two MSBs, resulting in correct values when the top two MSBs are zero (values under $2^8 = 256$), but otherwise with error of at least $2^8$.
% This is noticeable when comparing to the CAN-D (correct) translation for $t \in [0,50].$ 




% \begin{figure*}[t]
%     \centering
%         \includegraphics[width=.12\textwidth]{figs/wheelspeed_payload_other.png}%\hspace{-.3cm}
%       \includegraphics[width=.20\textwidth]{figs/wheelspeed_signals_other.png}%\vspace{-.3cm}
%         \includegraphics[width=.12\textwidth]{figs/engine_pedal_payload_actt2.png}
%         \includegraphics[width=.20\textwidth]{figs/engine_pedal_signals_other.png}
%         \includegraphics[width=.12\textwidth]{figs/steering_payload_other.png}
%         \includegraphics[width=.20\textwidth]{figs/steering_signals_other.png}
%     \\
        
%         \includegraphics[width=.12\textwidth]{figs/wheelspeed_payload_actt2.png}
%         \includegraphics[width=.20\textwidth]{figs/wheelspeed_signals_actt2.png}
%         \includegraphics[width=.12\textwidth]{figs/engine_pedal_matching_signals_actt_zoom.png}
%         \includegraphics[width=.20\textwidth]{figs/engine_pedal_signals_actt2.png}
%         \includegraphics[width=.12\textwidth]{figs/steering_payload_actt2.png}
%         \includegraphics[width=.20\textwidth]{figs/steering_signals_actt2.png}
        
%         \label{fig:qual_compare_paylods_signals}
%         \caption{Tokenization of three payloads by READ, LibreCAN and TANG* in top row, and corresponding tokenizations and translations of the same payloads by CAN-D in the bottom row. Note that when supplemental labels are provided by the translation step of ACTT, the name and units of the matching diagnostic is provided, as well as the $R^2$ value between the signal and the diagnostic. Left: Tokenization of payload containing four wheelspeeds encoded as Little Endian Signals: Top: Incorrect Tokenization of other methods due to the incorrect handling of little endian signals. Bottom: Correct Tokenization and Translation by CAN-D. Middle: Tokenization of a payload containing signed and unsigned engine and pedal related signals. The tokenization is identical for all methods, but the first (green) and second (light blue) signed signals are converted into values incorrectly by the other methods (top), resulting in sharp discontinuities where the signal values change sign. Note that the translation provided by ACTT2.0 (bottom) would not have been feasible without correctly classifying these signed signals. We illustrate the diagnostic matching of CAN-D to the right of the signals plots, where the matched diagnostics are plotted in black, and the signals values at the interpolated diagnostic timepoints are plotted in color. Right: payload containing four steering related little endian signed signals that are tokenized incorrectly by the other methods (top) and correctly by CAN-D (bottom). Note that in this case, we do not find any matching diagnostics in the translation step of CAN-D, but since these labels are supplemental, the tokenization still succeeds (as opposed to [Redacted citation]).  *TANG differs slightly in all of these tokenizations in that it sometimes splits off the least significant bits into 1-bit signals.}
        
% \end{figure*}




==> CAN-D IEEE/45-big-figs.tex <==
\begin{figure*}
        \vspace{-.8cm}
    \caption{Tokenization and translation of three messages by CAN-D and top competing methods, READ \&  LibreCAN.
    When interpretation is provided by CAN-D, the label and units of the matched diagnostic are shown with the $R^2$ value, and the values are scaled appropriately. 
    %  In the top figure we get the same boundary and endianness results in all methods, so the tokenization for all methods is shown with single signal layout plot. 
    %  However, in the bottom two examples, we have different tokenizations, signal layouts for ACTT are shown on the left, and the layouts for the others are shown on the right. 
    %  *TANG differs slightly in all of these tokenizations from READ \& LibreCAN in that it sometimes splits off the least significant bits into 1-bit signals.
     }
    \hrule
    \centering
        \begin{subfigure}[c]{\textwidth}%
        \includegraphics[width=.21\textwidth]{figs/engine_pedal_payload_cand.pdf}%
        \includegraphics[width=.38\textwidth]{figs/engine_pedal_signals_cand.pdf}%
        \includegraphics[width=.39\textwidth]{figs/engine_pedal_signals_other.pdf}%
        \vspace{-.1cm}%
        \subcaption{Message containing signed and unsigned engine- and pedal-related signals. \textbf{Left}: Signal boundaries and endianness are correctly identified by all methods. \textbf{Middle}: All signals are correctly translated and have physical interpretations by CAN-D. Highly correlated matches found for \textcolor{green}{\textbf{green}}, \textcolor{Cerulean}{\textbf{blue}}, and \textcolor{Maroon}{\textbf{maroon}} signals. The \textcolor{Blue}{\textbf{navy}} signal at bit 4, matched to DID `Accelerator pedal position D' with low correlation ($R^2 = .53$), is likely an accelerator indicator. As this is not an available DID, CAN-D has unearthed information that could not be simply queried.% %using UDS. 
        \textbf{Right}: Other methods incorrectly translate \textcolor{green}{\textbf{green}} and \textcolor{Cerulean}{\textbf{blue}} signals as unsigned, resulting in sharp discontinuities where the signals change sign.%
        %Note that the translation provided by ACTT2.0 (bottom) would not have been feasible without correctly classifying these signed signals. 
        }%
    \end{subfigure}%
    \vspace{-.15cm}
    \hrule%
    \begin{subfigure}[c]{0.485\textwidth}%
        \includegraphics[width=.99\textwidth]{figs/wheelspeed_signals_cand.pdf}
        \raggedleft{\rule[.05mm]{4.4cm}{.01cm}} \\
        \includegraphics[width=.45\textwidth]{figs/wheelspeed_payload_cand.pdf}
        \vspace{-.4cm}
        \hspace{.2cm}
        \rule[-2mm]{.005cm}{4cm}
         \hspace{.2cm}
        \includegraphics[width=.45\textwidth]{figs/wheelspeed_payload_other.pdf} \\
        \raggedright{\rule[-2mm]{4.4cm}{.01cm}}
        \includegraphics[width=.99\textwidth]{figs/wheelspeed_signals_other.pdf}
        \vspace{-.45cm}
        \subcaption{Message containing four wheel speeds encoded as little endian signals. \textbf{Top}: Correct tokenization and translation by CAN-D and match to ``Vehicle Speed'' DID with $R^2 = 1$. \textbf{Bottom}: Mistokenized as five big endian signals by other methods with MSBs (bits 13--15, 29--31, and 45--47) attributed to the wrong signals. Because all encode speed, \textcolor{Cerulean}{\textbf{blue}}, \textcolor{green}{\textbf{green}}, and  \textcolor{Orange}{\textbf{orange}} signals appear correct, save some minor discontinuities. 
        %Hence, quantitative signal error evaluation would yield near perfect results. 
        However, these signals encode the wheel speeds and are often used by Electronic Stability Control to stimulate anti-lock braking and traction control pending discrepancies in wheel speeds; mixing the MSBs of wheel speeds may go unnoticed in normal conditions but could prove consequential in adverse driving conditions!
        }
    \end{subfigure}
    \hspace{.3cm}
    \begin{subfigure}[c]{0.485\textwidth}
        \includegraphics[width=\textwidth]{figs/steering_signals_cand.pdf}
        \raggedleft{\rule[.05mm]{4.4cm}{.01cm}} \\
        \includegraphics[width=.45\textwidth]{figs/steering_payload_cand.pdf}
         \vspace{-.4cm}
        \hspace{.2cm}
        \rule[-2mm]{.005cm}{4cm}
         \hspace{.2cm}
        \includegraphics[width=.45\textwidth]{figs/steering_payload_other.pdf} \\
         \raggedright{\rule[-2mm]{4.4cm}{.01cm}}
        % \vspace{-.1cm}
        \includegraphics[width=.99\textwidth]{figs/steering_signals_other.pdf}
        \vspace{-.45cm}
        \subcaption{Message containing four steering-related, little endian signals, three of which are signed. \textbf{Top}: Correct tokenization and translation by CAN-D (no interpretation). \textbf{Bottom}: Incorrect tokenization and translation by other methods. 
        Assuming big endian signals, they are forced to cut on most byte boundaries, resulting in truncated, noisy \textcolor{SeaGreen}{\textbf{teal}}, \textcolor{SpringGreen}{\textbf{lime}}, \textcolor{Orange}{\textbf{orange}}, and \textcolor{Maroon}{\textbf{maroon}} signals. 
        The \textcolor{Blue}{\textbf{navy}} signal does not appear noisy but is noticeably incorrect when comparing the scale and the values for $t \in [0,50]$ to the correct CAN-D translation. 
        The two MSBs are misattributed to the next signal, resulting in errors of at least $2^8$ when the MSB(s) are nonzero.
        }
    \end{subfigure}
     \label{fig:qual_compare_paylods_signals}
\end{figure*}




==> CAN-D IEEE/50-implementation.tex <==
\section{Prototype OBD-II Plugin}
The CAN-D prototype device is a vehicle-agnostic, OBD-II plugin  that collects CAN data from the vehicle and runs the entire CAN-D pipeline depicted in Fig. \ref{fig:pipeline}. 
%(This of course depends on accessibility of ambient CAN data via OBD-II.) 
The prototype (shown in  Fig. \ref{fig:hw-pic}) is built using Linux-based, single-board computers. 
\label{sec:hw} 
\vspace{-.1cm}
 \begin{wrapfigure}[10]{r}{.25\textwidth}
    \centering
    \includegraphics[scale = .04]{figs/rpi_prototype_2.jpg}
    \caption{Prototype CAN-D device using a Raspberry Pi and CANBerry Dual 2.1 boards.}
    \label{fig:hw-pic}
\end{wrapfigure}
Specifically, we use a Raspberry Pi 3B+ with Raspbian Buster in conjunction with an Industrial Berry's  CANBerry Dual 2.1\footnote{\url{http://www.industrialberry.com/canberrydual-v2-1/}}.
The Raspberry Pi 3B+ offers 1 GB of RAM and a 1.4 GHz ARMv8 processor. 
The device is powered either from battery or using on-board power from a vehicle's 12-volt system.
%, and schematic is shown in Fig. \ref{fig:rpi_scheme} in \hyperref[sec:appendix]{Appendix}. 

% To use CAN-D 2.0, the supervised model for learning signal boundaries (see Step 1 of Fig \ref{fig:pipeline} and Sec. \ref{sec:cutprob}) would be trained offline in advance (once). 
% Next, upon plugging the device into the OBD-II port, it automatically determines the supported (responsive) DIDs, and logs CAN traffic log while iteratively requesting each supported DID. 
% At this point the driver would ideally exercise as much of the vehicle's functionality as possible. 
% Once the CAN log is captured, the algorithmic pipeline processes the log and builds a \texttt{.dbc} file giving the signal definitions (learned tokenization, translation, and interpretation) for each ID. 
% This process of collecting CAN data and running the algorithmic pipeline to produce a .dbc file will occur once per vehicle.  
% Finally, CAN-D 2.0 uses the Python cantools module \cite{cantools} and the produced \texttt{.dbc} file to decode CAN data in real-time on future drives. 


One challenge of building a vehicle-agnostic prototype is that the bitrate for the CAN is unknown and variable per  vehicle, and improper bitrate selection can cause adverse vehicle function.
To solve this issue, the device iterates through common bitrates, identifying the bitrate that results in only expected packets. % (which would indicate an improper bitrate).
%(e.g. extended IDs on passenger vehicles, remote data frames, error frames, no packets) to detect improper settings, thus determining the correct bitrate that yields only the expected packets. 
This allows our prototype to be compatible with most CANs regardless of bitrate.

Another complication is that automobiles typically have multiple CAN buses, and often more than one is available from the OBD-II interface. 
The prototype analyzes two unique networks by allocating a dedicated CAN controller for each using CANBerry Dual 2.1. 
Once connected, it automatically determines each network bitrate and identifies the VIN using the Unified Diagnostic Services query--response protocol (see Sec. \ref{sec:can-basics}), and begins logging data. 
%which is then used along with date and time to name the log file. 
%LEDs on the device indicate function and no user input is required. 
A switch on the prototype can be used to augment the network traffic with the other available diagnostic queries.  
The CAN traffic is collected using SocketCAN CAN-Utils\footnote{\url{https://github.com/linux-can/can-utils}}, logged to an ASCII-encoded text CAN log file, and %(see Fig. \ref{fig:canlog}) 
named using the  VIN (automatically identified via a DID query) and timestamp. 
Flashing LEDs on the device indicate the progress throughout this collection process. 
The device then runs this CAN log through the CAN-D pipeline, outputting a DBC, which can then be used for real-time decoding and visualization of signals on the device. 


%Challenges:\begin{itemize}
 %   \item Each CAN has a predefined (and usually unknown) bitrate %that must be identified to access the network.
 %  Improper implementation of CAN devices can cause unintended vehicle behavior* 
%The prototype must work on any CAN with limited or no user interaction.
  %  \item The device should analyze multiple CANs which may be accessed through the On-Board Diagnostic Interface (OBD-II).
%te and time must be recorded in order to properly organize data.
%\end{itemize}

%\begin{itemize}
 %   \item CAN-D Prototype Device configures itself to the correct network speed by stepping through common bitrates and identifying unusual message types (e.g., existence of extended IDs on passenger vehicles, remote data frames, error frames, and missing messages).
%Device automatically catalogs VIN and saves data per-vehicle based on unique VIN and date-time combination using a real-time clock.
%LED lights indicate function to user. 
%Raw CAN data  automatically logged with or without diagnostic queries.
 %   \item Multiple CAN controllers are used in order to analyze data from numerous networks on the same diagnostic port.
%\end{itemize}



% \missingfigure{Schematic}6


Using our heuristic signal boundary classifier (Step 1), we benchmarked the device running the CAN-D pipeline.   
We collected CAN traffic augmented with diagnostic data from a passenger vehicle for 70 s, logging $\smalltilde$170K frames. 
Running the pipeline on this log averaged 129 s--55 s for preprocessing, 14 s for tokenization and translation (Steps 1--3), 50 s for interpretation (Step 4), and 10 s for writing to DBC, over six runs with negligible variance.   
As implementation was focused on algorithmic research, efficiency was not a main goal and could be significantly improved. 
This proves the pipeline is viable for use in a portable, lightweight, edge computing device. 

Finally, we note a limitation with respect to the prototype. As stated previously, vehicles not required to follow the diagnostic standards (e.g., nonemissions producing vehicles) may not be queryable, and thus getting labeled diagnostic ground truth signals for Step 4 would not be possible. On the other hand, some vehicles (particularly newer models) have segmented CANs, allowing diagnostic queries to be sent/received at the OBD-II port but not allowing visibility to ambient CAN traffic. Thus, this prototype would be unable to collect the raw CAN data via this port. One possible workaround for these vehicles would be to bypass the gateway at the OBD-II connector and directly access the targeted network's CAN wires. 

% we used our heuristic for the signal boundary classifier (Step 1). 
% While training the supervised signal boundary classifier (step 1) can occur on a traditional compute environment, the prototype can also be used for this one-time training. 
% To benchmark the performance of this prototype, we train the classifier based on X minutes of log data, which takes  $\smalltilde3$m.

% Performance tuning our implementation has not been performed, but promises greater efficiency. 
% \add{something about how we didnt make an effort to be computationally efficient}






 




==> CAN-D IEEE/60-conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}
We considered the problem of developing a vehicle-agnostic method for extracting the hidden signals in automotive CAN data and present a comprehensive survey of this area. 
We presented CAN-D, a four-step, modular pipeline using a combination of ML, a novel optimization process, and heuristics  to identify and correctly translate signals in CAN data to their numerical time series. 
In particular, CAN-D is designed to extract big and little endian signals as well as signed and unsigned signals.  
Although this greatly enhances the complexity of the problem, these are necessary accommodations as specified by standard signal definitions. 
As our results show,  when endianness and signedness are ignored, the resulting translations are incorrect and overly noisy.  
In evaluation on 10 diverse vehicles' data, we compared CAN-D to the four state-of-the-art methods, providing a comparative study of previous methods on a more comprehensive dataset than ever previously used. 
We achieved less than 20\% of the average error of other methods and established that CAN-D is the only method that can handle any standard CAN signal.
Finally, we presented a lightweight hardware implementation for using CAN-D in situ via an OBD-II connection to first learn a vehicle's signals, and in future drives convert raw CAN data
% once-hidden CAN signals 
to multivariate time series in real time. 
Because CAN signals provide a rich source of real-time data that is currently unrealized, we hope this contribution will facilitate many vehicle technology developments.%CAN vulnerability and security research, among other vehicle technology developments. 

%able to handle both endiannesses and signednesses. 

% Our results give a comparative study evaluating the four state-of-the-art methods against CAN-D. 

% We extract complete signal definitions as defined at the outset of the problem: we identified signals positions (start bit and length) in Sec. \ref{sec:cutprob}, endianessness in Sec. \ref{sec:endianess_opt}, signedness in Sec. \ref{sec:signed_class}, and the translation (label, unit, scale, offset) in Sec. \ref{sec:diag-matching}.

% We broaden the scope of the problem introduced by previous works, and removing the overly limiting assumptions that limit the efficacy of these methods, namely that these methods do not consider the full range of possible signal encodings 
% big endian byte ordering and only unsigned bit encodings. 

% We implement all of the methods, develop a set of metrics, and compare all of the methods on a large representative set of CAN data spanning many makes, models, and years. We demonstrate that our method is superior not only on the signals that violate the limited assumptions made by previous methods, but on unsigned big endian signals as well. We additionally provide a qualitative evaluation which visually illustrates the superiority of CAN-D. 


% This reduces the problem of signal extraction to simply identifying signal boundaries (equiv., start bit, length), an oversimplification that  prevents correctly decoding signal's bits into their tokenized numerical (and ideally translated) values---the end goal of solving the signal extraction problem. 
% Algorithmically accommodating signals that may wrap across byte boundaries to the next (big endian) or previous (little endian) byte greatly enhances the complexity of the signal extraction problem. 
% Furthermore exacerbating the situation is the presence of unsigned (base 2) and signed (2's complement) bit encodings (which defines how a given bit string is converted to an integer). 
% Finally, provided signals of both endianess and encoding schemes can be identified (and therefore signals can be decoded into their numerical values), mapping a signal's decoded time-series to the actual physical meaning in the car is desired. 


% Future work: (in ordre of importance)
% arrow a mature buck, 
% signal categorization, 
% integrate body-related signal translation process (e.g., see \cite{Pese2019librecan}), user study, 
% solve cyber security, mail copy to Pese and Mirco w/ a love note non quid pro quo for dirt on Hunter Biden. 
% $$ACTT \geq \infty > LibreOffice > READ > Air Force > Isreali Crap$$

% \add{putting this here b/c not sure if/where we need it:}


==> CAN-D IEEE/98-acknowledgements.tex <==

\section*{Acknowledgments}
Special thanks to Bill Kay for his helpful comments. Research was sponsored by the Laboratory Directed Research and Development Program of Oak Ridge National Laboratory, managed by UT-Battelle LLC, for the US Department of Energy (DOE) and by the DOE, Office of Science, Office of Workforce Development for Teachers and Scientists (WDTS) under the Scientific Undergraduate Laboratory Internship program. 


==> CAN-D IEEE/99-biographies.tex <==
\vskip -2\baselineskip plus -1fil

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bio_pics/miki.jpg}}]{Miki E. Verma} recieved a B.S. in Applied and Computational Math Sciences from the University of Washington in 2018 and is currently pursuing an M.S. in Symbolic Systems at Stanford University. Miki joined Oak Ridge National Laboratory as an intern in 2018, and is currently a research data scientist in the Cyber Resilience and Intelligence Division, where she works on applications in a variety of cybersecurity domains including vehicle and network security, and security operations. 
\end{IEEEbiography}

\vskip -2\baselineskip plus -1fil

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bio_pics/bobby_profesh.jpg}}]{Robert A. (Bobby) Bridges}  received  the B.S. in 2005 from Creighton University and a Ph.D.  in 2012 from Purdue University, both in Mathematics. Bobby joined Oak Ridge National Laboratory  as a postdoc in 2012, was promoted to Associate Researcher in 2013 then Staff Researcher in 2017, and now serves as the (Acting) Cybersecurity Research Group Leader. Bobby's provides applied mathematics and data science support to a diverse team focusing on network and vehicle security. 
\end{IEEEbiography}

\vskip -2\baselineskip plus -1fil

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bio_pics/jordan.png}}]{Jordan J. Sosnowski} received a B.S. in Software Engineering and M.S. in Cybersecurity Engineering from Auburn University in 2019 and 2021, respectfully. Jordan joined Oak Ridge National Laboratory as a summer intern in 2019 to research controller area networks. He is currently an incident responder at a department of energy national laboratory, where his focus is on malware analysis and reverse engineering.
\end{IEEEbiography}

\vskip -2\baselineskip plus -1fil

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bio_pics/sam.jpg}}]{Samuel C. Hollifield} is currently pursuing a B.S. degree in computer engineering from Tennessee Technological University, Cookeville, TN.

In 2018, he joined the Oak Ridge National Laboratory (ORNL) as an intern, exploring the security of electronic control units used in modern automobiles. He is currently a cyber security research associate in the Cyber Resilience and Intelligence Division at ORNL where he works primarily on network and application cybersecurity for automotives and similar embedded systems. Mr. Hollifield is a member of the Society of Automotive Engineers (SAE). 
\end{IEEEbiography}

\vskip -2\baselineskip plus -1fil

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bio_pics/mike.jpg}}]{Michael D. Iannacone} 
received a B.S. in computer engineering from 
Rochester Institute of Technology in 2008 and a M.S. in 
information security from Georgia Institute of Technology in 2013.

From 2007 to 2008, he was a Research Assistant with RIT's Lab for Wireless Networking and Security, modeling wireless ad-hoc networks.
From 2009 to 2011, he was a Research Assistant at the Georgia Tech Information Security Center (GTISC) research lab, studying cellular device security.
Since 2011, he has been a researcher with Oak Ridge National Laboratory, currently in the Cyber Resilience and Intelligence Division. His work has focused on network intrusion detection and anomaly detection, and securing embedded devices, vehicles, and vehicle infrastructure.

\end{IEEEbiography}



% \begin{IEEEbiography}{Michael Shell}
% Biography text here.
% \end{IEEEbiography}

% % if you will not have a photo at all:
% \begin{IEEEbiographynophoto}{John Doe}
% Biography text here.
% \end{IEEEbiographynophoto}

% % insert where needed to balance the two columns on the last page with
% % biographies
% %\newpage

% \begin{IEEEbiographynophoto}{Jane Doe}
% Biography text here.
% \end{IEEEbiographynophoto}

% % You can push biographies down or up by placing
% % a \vfill before or after them. The appropriate
% % use of \vfill depends on what kind of text is
% % on the last page and whether or not the columns
% % are being equalized.

% %\vfill

% % Can be used to pull up biographies so that the bottom of the last one
% % is flush with the other column.
% %\enlargethispage{-5in}



% % that's all folks

==> CAN-D IEEE/OLD-ml-eval.tex <==
\subsection{Evaluate Classifiers for Step 1}
\label{sec:eval-step1}
% \subsubsection{Step 1 Evaluation}
% \label{sec:eval-step1}

\textit{Cut prob ML model evaluation, tables, conclusions. Ultimately we chose RF with 100 estimators and these features for our pipeline. }

 \add{Bobby: try to rewrite this nicer, shorter. plan to keep the Table 2, and depending on coding progress, we'll reference to Appendix for feature selection} 
 
% We collected CAN data on six vehicles dated 2013, 2015, 2016 and 2017 of six different makes and using both combustion engine and hybrid vehicles. 
% Data was captured from these vehicles using a Kvaser Leaf Lite VS (www.kvaser.com) providing CAN-to-USB translation to a Linux OS laptop using SocketCan Software (https://elinux.org/Can-utils). 
After capturing and aggregating the data we performed a leave-one-AID-out cross validation across multiple classifiers.
Note that each vehicle is a separate model and trim and that if there were multiple captures from the same vehicles they would be trained together, as testing with a vehicle that we had trained on would give metrics that are not credible. 
Leave-one-AID-out has us training on all the AIDs but one and testing on leftover AID, this process is repeated until each AID is the validation set. 
% The per AID confusion matrix is micro-averaged and reported in Table \ref{tb:aid}.

For our classifiers we used the Python library SciKit \cite{scikit-learn}. 
The general classifiers used were: logistical regression, support-vector machine classifier, decision trees, and random forest. 
We tested two different logistical regression classifiers.
% Both used a max iteration of 10,000 and a constant random state. 
However, one had balanced class weights, the other had no class weights the rest of the parameters were set to default. 
Eight support-vector machine classifiers were tested with either balanced class weight or no class weights, constant random states, and each with a different kernel: radial basis function, linear, polynomial (power of 3), sigmoid. 
Only one decision tree classifier was tested.% and it was configured with a constant random state. 
Four random forest classifiers were included. 
One had 10 estimates with balanced class weights, another with 10 estimators with no balancing, another with 100 estimators with balanced class weights, and another with 100 estimators with no weights. 
Micro-average results from running leave-one-AID-out are listed in Table \ref{tb:aid}.
\begin{table}[ht]
    \centering
    \begin{threeparttable}[b]
        \caption{Micro Average Results of Leave-One-Out by AID}
        \label{tb:aid}
        
        \begin{tabular*}{0.45\textwidth}{llll}
            \toprule
            \textbf{Classifier} & \textbf{F-Score} & \textbf{Precision} & \textbf{Recall} \\ \midrule
            
            Log Reg OVR & 90.2 & 94.2 & 86.6 \\
            Log Reg OVR (bal.) & 86.9 & 82.5 & 91.8 \\
            
            SVC linear & 91.0 & 94.2 & 88.0 \\
            SVC linear (bal.) & 87.5 & 84.3 & 90.9 \\
            SVC poly & 65.3 & \textbf{96.5} & 49.4 \\
            SVC poly (bal.) & 75.7 & 62.8 & \textbf{95.2} \\
            SVC RBF & 91.3 & 95.9 & 87.2 \\
            SVC RBF (bal.) & 90.2 & 87.4 & 93.2 \\
            SVC sigmoid & 60.5 & 62.7& 58.4 \\
            SVC sigmoid (bal.) & 52.6 & 40.4 & 75.4 \\
            
            Decision tree & 89.1 & 89.1 & 89.1 \\
            
            RF - 10 Est. & 92.2 & 94.0 & 90.5 \\
            RF (bal.) - 10 Est. & 91.7 & 94.2 & 89.3 \\
            RF - 100 Est. & \textbf{92.8} & 94.2 & 91.5 \\
            RF (bal.) - 100 Est. & 92.1 & 93.7 & 90.5 \\
            \bottomrule
        \end{tabular*}
        
    \end{threeparttable}
\end{table}


Note, our precision is normally higher than our recall. 
This fact is to be expected since we have biased classes, specifically, a larger amount of instances in our training data where there should not be a cut compared to there being a cut. 
Across the six cars' data we have 3,868 instances of when the bit should not cut to the `right' and 944 instances where the bit should be cut to the `right'; therefore, the base-rate of the data is approximately 4:1.
Because of this imbalance in our class representation we have a biased class issue. 
We attempted to combat this issue by balancing the class weights. 
Balancing class weights allow classes that are disproportionately represented to be better represented. 
However, as one can see in Table \ref{tb:aid} using balancing techniques did not increase our overall F-Score.

An additional attempt to increase our metrics was feature selection. The general idea is to eliminate spurious features, that is features that lower classification abilities. 
We used feature selection algorithms false discovery rate and mutual info  on a random forest classifier.
False discovery rate and mutual info feature selection are provided by Scikit Learn \cite{scikit-learn}. 
In the end feature selection did not have a meaningful impact, metrics did not increase with only select features included. 
Interestingly, near optimal classification metrics are obtained with ultimately few features.
Overall, we exhibited a train classifier that can achieve over 92\% F-Score in tokenzing signals from can data captures. 
The results of this can be seen in Table \ref{tb:selection}. 



The Top 10 Features across all five of the vehicles with False Discovery Rate can be seen in Table \ref{tb:top_fdr} and the top for Mutual Class can be seen in Table \ref{tb:top_mutual}.


% \subsubsection{Step 3 Evaluation}
% \label{sec:eval-step3}
% \textit{Signedness classification model evaluation, tables, conclusions. Ultimately, we chose to use the heuristics in our pipeline rather than any learned model.}

% Here we followed the same setup as Section \ref{sec:eval-step1}.
% Additionally we tested two rule-based algorithms against our machine learning classifiers.
% The Benford Rule and Flip-Based Rule defined in Algorithm \ref{rules}. 
% The parameter $X$ used in Algorithm \ref{rules} is the total feature array discussed in Section \ref{sec:cutprob}

% \smallskip
% \begin{algorithm}[h]
%   \caption{Rules}\label{rules}
%   \label{alg:1} 
%   \begin{algorithmic}
%   \Function{BenfordRule}{$X$}
%     \State $\hat{y} \gets \emptyset$
%     \For{$i$ in $\text{len}(X)$}
%         \If{$(X_{i3} + X_{i2} < .1 )$ \& $(X_{i4} > X_{i3})$}
%             \State $\hat{y}_i \gets \text{True}$
%         \Else
%             \State $\hat{y}_i \gets \text{False}$
%         \EndIf
%     \EndFor
%     \State \textbf{return} $\hat{y}$
%     \EndFunction


%     \smallskip


%   \Function{FlipRule}{$X \text{, flips}$}
%     \State $\hat{y} \gets \emptyset$
%     \For{$i$ in $\text{len}(X)$}
%         \If{$(X_{i3} + X_{i2} = 0$}
%             \State $\hat{y}_i \gets \text{True}$
%         \ElsIf{$\text{flips}_{i} = 0$}
%             \State $\hat{y}_i \gets \text{False}$
%         \ElsIf{$X_{i3} + X_{i2} < .1$}
%             \State $\hat{y}_i \gets \text{True}$
%         \Else
%             \State $\hat{y}_i \gets \text{False}$
%         \EndIf
%     \EndFor
%     \State \textbf{return} $\hat{y}$
%     \EndFunction
%   \end{algorithmic}
% \end{algorithm}

% Note the rule-based algorithms do not actually use the training data. 
% Instead, each will simply apply their heuristic to label the test data.
% Micro Average Results from running leave-one-AID-out are listed in table \ref{tb:signal}



% \begin{table*}[h]
%     \centering
%     \begin{threeparttable}[b]
%         \caption{Micro Average Results of Leave-One-Out Grouped by AID}
%         \label{tb:signal}
        
%         \begin{tabular*}{.45\textwidth}{l l l l}
%             \toprule
%             \textbf{Classifier} & \textbf{F-Score} & \textbf{Precision} & \textbf{Recall} \\ \midrule
%                 Log Reg OVR & 23.5 & 75.0 & 13.9 \\
%                 Log Reg OVR (bal.) & 66.1 & 49.4 & \textbf{100.0} \\
%                 SVC Linear & 69.8 & 72.5 & 67.4 \\
%                 SVC Linear (bal.) & 71.0 & 55.1 & \textbf{100.0} \\
%                 SVC Poly & 72.2 & 89.6 & 60.4\\ 
%                 SVC Poly (bal.) & 65.6 & 49.4 & 97.6 \\ 
%                 SVC RBF & 0.0 & 0.0 & 0.0\\
%                 SVC RBF (bal.) & 64.6 & 47.7 & \textbf{100.0}\\
%                 SVC Sigmoid & 15.1 & 16.6 & 13.9 \\
%                 SVC Sigmoid (bal.) & 18.2 & 11.2 & 48.8 \\
%                 Decision Tree & 87.6 & 84.7 & 90.7\\
%                 RF - 10 Est. & 90.0 & 97.3 & 83.7 \\
%                 RF (bal.) - 10 Est. & 94.1 & 95.2 & 93.0 \\
%                 RF - 100 Est. & 92.8 & 95.1 & 90.7 \\
%                 RF (bal.) - 100 Est. & 92.8 & 95.1 & 90.7 \\
%                 Benford Rule & 95.4 & 93.3 & 97.6 \\
%                 Zero Flip Rule & \textbf{97.6} & \textbf{97.6} & 97.6 \\
%             \bottomrule
%         \end{tabular*}
        
%     \end{threeparttable}
% \end{table*}


% From these results one can see how the rule-based algorithms performed far better than any classifier. 
% However with this specific dataset we only have 408 signals to test on but with tokenization we have 4812 bits to test on.
% With more data the chance of a classifier performing better than the rule will hopefully increase.
% Additionally we believe we can use machine learning to determine the threshold used during the rule based algorithms. 
% For our tests we set it to 0.1, but that was an arbitrary decision that, we believe, can be improved with machine learning. 


==> CAN-D IEEE/cutprob.tex <==
\subsection{Learn Signal Boundary Probabilities}
\label{sec:cutprob}



% \begin{figure*}{\linewidth} 
% \begin{minipage}{.31\textwidth}
% % \begin{table}[!h]
% % \small
% %     \centering
%     \begin{threeparttable}
%         \caption{Local Features ($t$ and $t'$ denote subsequent timestamps)}
%         \label{tb:features}
%         \begin{tabular}{l}
%             \toprule
%             \textbf{Bit Values } \\
%             \midrule
%             $P(B_i = 0)$\\
%             $P(B_i = 0 \mid B_{i+1} = 0)$\\
%             $P(B_{i+1} = 0 \mid  B_i = 0)$ \\
%             $P(B_i = 1 \mid  B_{i+1} = 1)$\\
%             $P(B_{i+1} = 1 \mid  B_i = 1)$\\
%             \midrule
%             \textbf{Bit Flips } \\
%             \midrule
%             $P(B_i(t) \neq B_i(t'))$\\
%             $P(B_i(t) \neq B_i(t') \mid B_{i+1}(t) \neq B_{i+1}(t'))$\\
%             $P(B_{i+1}(t) \neq B_{i+1}(t') \mid B_i(t) \neq B_i(t') )$\\
%             $P(B_i(t) = B_i(t') \mid B_{i+1}(t) = B_{i+1}(t'))$\\
%             $P(B_{i+1}(t) = B_{i+1}(t') \mid B_i(t) = B_i(t'))$\\
%             \midrule
%             \textbf{Benford}  \\
%             \midrule
%             $P(B_i, B_{i+1} = 0, 0)$\\
%             $P(B_i, B_{i+1} = 1, 0)$  \\
%             $P(B_i, B_{i+1} = 0, 1)$  \\
%             $P(B_i, B_{i+1} = 1, 1)$ \\
%             \midrule
%             \textbf{Entropy}\\
%             $H(B_i)$\\
%             $H(B_i, B_{i+1})$\\
%             $H(B_i\dots B_{i+3})$ \\
%             \bottomrule
%         \end{tabular}
%      \end{threeparttable}
% %  \end{table}
%  \end{minipage}\quad
% \begin{minipage}{.67\textwidth}
%     \begin{figure*} 
%     \includegraphics[width=\linewidth]{figs/feature_generation_diagram.pdf}
%     \caption{(\textbf{Top}:) Process for creating a feature array from a ID trace. (\textbf{Bottom}:)  Subprocess for creating a feature vector for each bit gap.}
%     \label{fig:feature_gen}
%     \end{figure*}
% \end{minipage}%
% \end{figure*} 
 
 
% \begin{figure*}[H]
%     % \vspace{-1.2cm}
%   \centering
% \begin{minipage}{0.3\textwidth}
% \begin{table}[ht]
% \small
%     \centering
%     \begin{threeparttable}
%         \caption{Local Features ($t$ and $t'$ denote subsequent timestamps)}
%         \label{tb:features}
%         \begin{tabular*}{}{l}
%             %\addtolength{\tabcolsep}{-2pt}
%             \toprule
%             \textbf{Bit Values } \\
%             \midrule
%             $P(B_i = 0)$\\
%             $P(B_i = 0 \mid B_{i+1} = 0)$\\
%             $P(B_{i+1} = 0 \mid  B_i = 0)$ \\
%             $P(B_i = 1 \mid  B_{i+1} = 1)$\\
%             $P(B_{i+1} = 1 \mid  B_i = 1)$\\
%             \midrule
%             \textbf{Bit Flips } \\
%             $P(B_i(t) \neq B_i(t'))$\\
%             $P(B_i(t) \neq B_i(t') \mid B_{i+1}(t) \neq B_{i+1}(t'))$\\
%             $P(B_{i+1}(t) \neq B_{i+1}(t') \mid B_i(t) \neq B_i(t') )$\\
%             $P(B_i(t) = B_i(t') \mid B_{i+1}(t) = B_{i+1}(t'))$\\
%             $P(B_{i+1}(t) = B_{i+1}(t') \mid B_i(t) = B_i(t'))$\\
%             \midrule
%             \textbf{Benford}  \\
%             \midrule
%             $P(B_i, B_{i+1} = 0, 0)$\\
%             $P(B_i, B_{i+1} = 1, 0)$  \\
%             $P(B_i, B_{i+1} = 0, 1)$  \\
%             $P(B_i, B_{i+1} = 1, 1)$ \\
%             \midrule
%             \textbf{Entropy}
%             $H(B_i)$\\
%             $H(B_i, B_{i+1})$\\
%             $H(B_i\dots B_{i+3})$ \\
%             \bottomrule
%         \end{tabular*}
%     \end{threeparttable}
% \end{table}
% \end{minipage}%
%   \includegraphics[width=.7\linewidth]{figs/feature_generation_diagram.pdf}
%   \caption{(\textbf{Top}:) Process for creating a feature array from a ID trace. (\textbf{Bottom}:)  Subprocess for creating a feature vector for each bit gap.}
%   \label{fig:feature_gen}
% %   \vspace{-.7cm}
% \end{figure*}

% \begin{figure*}[h]
%   \centering
%   \includegraphics[width=\linewidth]{figs/feature_generation_diagram.pdf}
%   \caption{Top: Process for creating a feature array for each capture, which calls the 'Bit Feature Generation' subprocess; Bottom: Subprocess for creating a feature vector for each bit}
%   \label{fig:feature_gen}
%   \vspace{-.75cm}
% \end{figure*}

For each ID, the 64-bit message has 63 ``bit gaps'' indexed $(i,i+1)$ for $i = 0, \dots, 62$, and bits $i$ and $i+1$ are either contained in the same signal or span two signals. 
Previous works have focused on identifying signal boundaries using hand-crafted heuristics that leverage only two main features computed from an ID trace: each bit's flip probability and the range of values a candidate signal realizes.
%\textemdash and depended on the overly simplifying assumption that all signals are big endian and unsigned. 
The first step of CAN-D is to build a robust set of features for each gap and leverage well established statistical machinery from supervised machine learning to determine signal boundaries from the many features.  
This subsection describes the features and machine learning research used for this task and is represented in the top row of Fig. \ref{fig:pipeline}. 
In Sec. \ref{sec:eval} we evaluate our binary classification for signal boundary identification against the previous state-of-the-art methods. 
Finally, note that while we frame this as a binary classification problem, labelling each gap as signal boundary or not, the output needed for the second step of the CAN-D pipeline is not binary, but the estimated probability of a boundary at each gap. 


\textbf{Preprocessing}: 
Refer to Fig. \ref{fig:feature_gen}, which depicts the entire feature generation process for each ID trace (top) and then for each gap within the ID trace (bottom).
To build features from an ID trace,  we  first remove the constant bits. 
Sec. \ref{sec:test_data_types}, which discusses the many reasons for this. 
% as: (1) constant bits necessitate an adjacent signal boundary that need not be learned, 
% (2)  many features, which depend on nearby bit values and flips, are not defined for gaps adjacent to constant bits, and 
% (3) this counteracts the bias class problem, giving more adjacent signals to learn from in training. 
Denote the condensed ID trace $B^{\prime id} \in \{0,1\}^{n_{id}\times{m_{id}}}$ where $m_{id}$ is the number of non-constant bits for a given arbitration ID $id$. 
For each remaining $m_{id}-1$ bit gaps, we generate a set of 85 features: 17 features are ``local'' to the gap, examining only bits $i$ and $i+1$,
%and the bit directly to the left of the gap $(i, i+1)$ under inspection,
and the rest are from values of ``neighboring bits'' (e.g. bit $i-1$, bit $i+2$, etc.).

\begin{table}[b]
\small
    \centering
    \begin{threeparttable}[b]
        \caption{Local Features ($t$ and $t'$ denote subsequent timestamps)}
        \label{tb:features}
        \begin{tabular*}{.48\textwidth}{ll}
            %\addtolength{\tabcolsep}{-2pt}
            \toprule
            \textbf{Bit-Value }  & \textbf{Bit-Flip } \\
            \midrule
            $P(B_i = 0)$ & $P(B_i(t) \neq B_i(t'))$\\
            $P(B_i = 0 \mid B_{i+1} = 0)$ & $P(B_i(t) \neq B_i(t') \mid B_{i+1}(t) \neq B_{i+1}(t'))$\\

            $P(B_{i+1} = 0 \mid  B_i = 0)$ & $P(B_{i+1}(t) \neq B_{i+1}(t') \mid B_i(t) \neq B_i(t') )$\\
            $P(B_i = 1 \mid  B_{i+1} = 1)$ & $P(B_i(t) = B_i(t') \mid B_{i+1}(t) = B_{i+1}(t'))$\\
            $P(B_{i+1} = 1 \mid  B_i = 1)$ & $P(B_{i+1}(t) = B_{i+1}(t') \mid B_i(t) = B_i(t'))$\\
            \midrule
            \textbf{Benford}  & \textbf{Entropy} \\
            \midrule
            $P(B_i, B_{i+1} = 0, 0)$ &  $H(B_i)$ \\
            $P(B_i, B_{i+1} = 1, 0)$ &  $H(B_i, B_{i+1})$ \\
            $P(B_i, B_{i+1} = 0, 1)$ &  $H(B_i\dots B_{i+3})$ \\
            $P(B_i, B_{i+1} = 1, 1)$ &  \\
            \bottomrule
        \end{tabular*}
        
    \end{threeparttable}
\end{table}




\textbf{Local Features}:  We first generate the 17 local features for bits $i$ and $i+1$  (see Fig. \ref{fig:feature_gen} Bottom Left), which are denoted $v^{id}_i \in \mathbb{R}^{17}$. 
These local features belong to four categories and are listed in Table \ref{tb:features}.
% These encoding information about the bit $i$, the bit directly to the left of the gap $(i, i+1) $ under inspection.
\textit{Bit-Value}: The first bit-value feature, $P(B_i = 0)$, is motivated by the fact that the distribution of values differs significantly between the most and least significant bits of a signal; e.g., for LSBs $P(B_i = 0) \approx 0.5$ since LSBs frequently alternate values (for both signed and unsigned encodings). 
% only extreme (and therefore likely more unusual) signal values will take on value of 1, whereas LSBs flip more often. 
The next four bit-value features, are conditional bit-value probabilities (e.g. $P(B_{i+1} = 0 \mid  B_i = 0)$). 
These are expected to differ significantly for adjacent bits contained in the same signal vs. those that are part of separate signals, as the former are dependent while the latter are likely independent.  
% ; most notably, if bit $i$ is the LSB of one signal, and bit $i+1$ is the MSB of the adjacent signal, then $P(B_{i+1} = 0 \mid  B_i = 0) \approx 0$ since $P(B_{i+1} = 0) \approx 0$ and $P(B_{i} = 0) \approx .5$ for continuous signals. 
\textit{Bit-Flip}: We compute five analogous features, now for the probability that a bit ``flips'', i.e., alternates value in subsequent messages. 
The main intuition is that LSBs generally alternate values much more often than an adjacent signal's MSB; hence, the bit-flip features should provide good indicators for boundaries. 
Note that this is the feature that previous works build heuristics upon. 
\textit{Benford}: These features are based upon Benford's Law \cite{benfords}, 
%also known as the law of anomalous numbers. Benford's Law is 
an observation regarding the frequency distribution of leading digits $d$ of a base $b$ number, $P(d)=\log_{b} \left(1+\tfrac{1}{d}\right).$ %\log_b(d+1)-\log_b(d)
In base $b=10$, it states that $d=1$ appears as the significant digit $\smalltilde 30\%$ of the time, while $d=9$ appears as the leading significant digit less than $\smalltilde 5\%$.
While the law is trivial for base $b=2$, as an MSB is necessarily 1, we harness the intuition that the significant digits have a distinct distribution and include the distribution of 
%the gap's adjacent pair of bits 
the pair of bits $i$ and $i+1$ as local features. 
\textit{Entropy}: For the final three local features, we consider the entropy of bits $[i,\dots, i+j]$ for  $j \in \{0, 1, 3\}$. 
% The idea behind these features is to capture the amount of uncertainty in a short sequence of bits. 
We expect that sequences of bits that are part of the same physical signal will have very low entropy; whereas, sequences that contain bits from multiple signals will have higher entropy. 
% \add{One more sentence of explanation on entropy feature, why we expect this, and perhaps something about the entropy of checksums which violate the continuity assumpiton that all of the other features are based upon?}


\textbf{Neighboring bits' features}:  
We then forward/backward to neighboring bits (see Fig. \ref{fig:feature_gen} Bottom Right) and compute the same features for gaps $(i-1, i)$ and $(i+1, i+2)$;  thus, we add 34 more features by adding $v^{id}_{i-1}$ and $v^{id}_{i+1}$ to our feature set.  
In initial testing we experimented with adding more look forward/backward features and found that 1 in each direction was sufficient.
Finally, we another 34 difference features $v^{id}_{i}-v^{id}_{i-1}$ and $v^{id}_{i+1}-v^{id}_{i}$, yielding an 85-length feature vector for gap $(i, i+1)$. 

\textbf{Targets}: 
From a known DBC and a matching CAN log, we create a binary vector for each ID $y^{id}\in \{0,1\}^{m_{id}-1}$ giving the labels for training/testing. 
This is straightforward for big endian signals, yet, little endian signals have adjacent bits with non-adjacent indices at byte boundaries (see Eq. \ref{eq:bit-orderings}). 
%% Moved to next section: % Using the example of Sec. \ref{sec:can-basics} for illustration, if the first two bytes are a little endian signal we have neighboring indices $8\rightarrow 0$.  
% Our features require information from neighboring bits, but must be extracted from ID traces before endianness is known; yet endianness determines bit orders at byte boundaries (Eq. \ref{eq:bit-orderings}) . 
% Since big/little endian entail different bit orderings
%at byte boundaries; consequently, during feature generation 
% we do not know which bits to consider as  neighbors. 
% non-adjacent bits are within-signal neighbors. % cannot during feature generation know which signals are little or big endian.  
For training and testing the  model we split little endian signals on byte boundaries. 
For signal extraction, this is reconciled in CAN-D's step 2 (Sec. \ref{sec:endianess_opt}), which considers bit orderings of both endianness
%options at each byte when using this machine learning model as part of 
and uses an optimization process that accommodates extraction of full little endian signals.  
% When evaluating signal boundary identification, this means previous methods are not penalized for assuming that all signals are big endian.  



\textbf{Classifier}: 
We experimented with several classifiers and parameters including Decision Trees, Random Forests, Support Vector Classifiers, and Logistic Regression using Python's SciKit library.
% \cite{scikit-learn}. 
We also experimented with using balanced class weights, since we have high bias  towards the negative class (non-boundary gaps). 
See Sec. \ref{sec:dataset} for a description of data used. 
To examine the accuracy of the classifiers, we used Leave One (ID) Out Cross Validation (LOOCV), removing each ID from training and using it for testing, then microaveraging results. 
We found that Random Forest Regression with 100 Estimators and balanced class weights yielded the best results, with micro-averaged 94\% precision and 91.5\% recall for an F-Score of 93\%. 
Table \ref{tb:boundary_classifier_results} in \hyperref[sec:appendix]{Appendix} itemizes results for all the classifiers tested. 



The next step of our algorithm requires the inputs to be probabilities rather than binary labels, so for step 2 we use the classifier's un-thresholded output, a number in [0,1] interpreted as the probability of a cut at  gap $(i, i+1)$. 


% Following training, the model can then be exported to predict signal boundaries on a new dataset, which would be done online. 
% This process is shown in the white section of the first panel of Fig. \ref{fig:pipeline}. 

% After training, we let $f^{id}(i) \in [0,1]$ denote the output of the model, 
% which is the probability of a cut between bits $i$ and $i+1$ for ID $id$ in a given log. 



% \subsection{Tokenization Prediction}
% We use a trained classifier and a feature vector from unlabeled candata $X'$ into targets $y'$.
% % We describe the necessary steps to apply our trained model assuming one has a CAN data capture from a vehicle that they would like to tokenize. 
% Following the same process of aggregating the capture into ID traces, one can then generate a feature array based on the ID traces. 
% Once the feature array is generated it is fed to the trained classifier, and a prediction array is returned for each ID which can be defined as $P \in [0,1]^{b}$ with $b$ being the number of non-constant bits of the specific ID trace. 


% \begin{figure}[ht]
%     \includegraphics[width=.5\textwidth]{figs/bit_cut_feature_extraction_and_labeling_process.pdf}
%     \caption{As supervised binary classification is used for learning signal boundaries, the diagram depicts (\textbf{top}:)  how a CAN log is transformed into a feature vector array and (\textbf{bottom}:) how the corresponding DBC is transformed into a binary array of labels of the signal boundaries. 
%     \fix{in figure, change "bit cut" to "signal boundary" }
%     \fix{change figure headers to say signal boundary, remove ks, and use word log instead of capture} 
%     \fix{transpose figures, so that processes move from top to bottom, put side by side, and move next to \ref{fig:feature_gen}}}
%     \label{fig:feature_extraction_labeling}
% \end{figure}



% The tokenization pipeline consists of four main components: (1) data pre-processing, (2) feature and target generation, (3) model training, (4) tokenization prediction.


% Based on Assumption 4, we consider constant bits to necessarily delimit signals, and thus any 

% It is imperative that we capture CAN data that encompasses all of the vehicles functionalities so that all the bits are being exercised in their defined signals. 
% If not, some signals' most significant bits may not change and seem to appear constant, and get discarded mistakenly. 

% Therefore any valid signal must contain any contiguous set of bits that does not contain constant bits. 
% After grouping and filtering the ID traces, features can be calculated for each bit per trace. 

% and build $X \in {id} \in \mathbb{R}^{85}$. This entire Feature Generation process is depicted in  Fig. \ref{fig:feature_gen} (top). 
% The subprocess for generating these feature for each bit is described in the following sections \ref{sec:base_features}-\ref{sec:non_base_features}, and is depicted in Fig. \ref{fig:feature_gen} (bottom). 


%  are part of the same signal or separate signals based on characteristics of a bit's value, how its value changes over time, and how these characteristics relate to those of the surrounding bits. 
% Formally, we define a set of features $X_i$ for bit $i$, and try to predict $y_i \in \{0,1\}$ where $y_i = 0$ denotes that bits $i$ and $i+1$ are part of the same signal, and $y_i=1$ denotes that there is a signal boundary between bits $i$ and $i+1$.
% We build this set of features and ground truth labels, and train a classification model offline. 
% This is shown in the top left gray portion of Fig. \ref{fig:pipeline}. This consists of two main components, "Signal Boundary Feature Extraction Process" and "Signal Boundary Labeling Process", which are illustrated in Fig. \ref{fig:feature_extraction_labeling}, and explained in \ref{sec:bit_cut_feature_extraction}-\ref{sec:non_base_features} and \ref{sec:bit_cut_labeling} respectively. 

% \subsubsection{Signal Boundary Feature Extraction}
% \label{sec:bit_cut_feature_extraction}


% To build features, we first separate the sequence of data fields in a log by ID, building a set of \textit{ID traces}. 
% We define an ID \textit{trace} $B^{id} \in \{0,1\}^{n_{id}\times64}$ to be the set of $n_{id}$ 64-bit messages sent on a particular arbitration $id$ over the course of a CAN log.


% We denote the $i$\textsuperscript{th} bit of the message sent at time $t$ as $B^{id}_i(t)$, where $i \in [0,...63]$ and bits are numbered in order of transmission on the bus (normal, not sawtooth numbering). 
%Note that, a message can have fewer than 8 bytes of data, so we pad any shorter messages with zeros. 
% We then remove all of the constant bits from each ID trace, we are left with \textit{non-constant ID trace} $B^{\prime id} \in \{0,1\}^{n_{id}\times{m_{id}}}$ where $m_{id}$ is the number of non-constant bits for a given arbitration ID $id$. 
%The reason why we use the non-constant traces $B^{\prime id}$ is because our features depend on how bit values change, and based on Assumption 4, we consider constant bits to necessarily delimit signals. 
%\add{Furthermore, because the most significant bits of signals are unchanging when extreme values are not reached, constant bits will naturally delimit signals. We smash signals together to make for better training data. Explain further in \ref{sec:eval-step1}}

% $for each bit $i$ in the nonconstant trace $B^{\prime id}$ for ID $id$. These base features, which are listed in Table \ref{tb:features} fall into four feature categories: bit value probabilities, bit flip probabilities, Benford state probabilities, and entropy. 

% \add{Note that many of these features are combinations of one another; we plan to do feature selection, and put in some redundancies in order to determine which features were the most important}

% This subsection describe how we convert the arrays of parsed candata into a feature array $X$ and DBCs into a target vector $y$.
% After grouping and filtering the can data into ID traces, features can be calculated for each bit position $j = 0, \ldots 63$ per trace; that is for each trace, for each $j = 0, \ldots 63$ we will compute a feature vector.
% Overall we compute 100 features, the first twenty are base features which are listed in Table \ref{tb:features}. 
% \medskip


% \textit{\underline{Bit Value Probabilities}} \\
% We compute 5 features relating to the probability of a bits value, and the conditional probability of its value given the value of the bit to its right (also condition in opposite direction). 
% bits that are towards the right end of a signal (least significant) than for bits that are towards the left end (most significant). 
 
%$P(B_i = 0) \approx .5$ for the least significant bit of a continuous signal as it will flip between 0 and 1 every time the value of the signal is incremented or decremented by 1. Similarly, for the most significant bit,  $P(B_i = 0) \approx 1$ since only extreme (and therefore likely more unusual) signal values will take on value of 1. 

% For example, if bits $i$ and $i+1$ are part of the same signal $P(B_{i+1} = 0 \mid  B_i = 0) \approx .5$ because each bit will take on value 0 roughly half the time that the next less significant bit will. However, if this is unlikely to be true if they are from different signals, most notable if bit $i$ is the lsb of one signal, and bit $i+1$ is the msb of the adjacent signal, then $P(B_{i+1} = 0 \mid  B_i = 0) \approx 0$ since $P(B_{i+1} = 0) \approx 0$ and $P(B_{i} = 0) \approx .5$. 

% \medskip
% \textit{\underline{Bit Flip Probabilities}} \\


% Similarly to the bit value features, we compute 5 bit flip probability features which are based on the probability of a bits value flipping between two successive messages, as well as the probability of a bits value flipping conditioned on whether the bit to its right flips. The motivations are similar to those of the bit value features: the non-conditional probability feature, $P(B_i(t) \neq B_i(t+1))$, serves as an indicator of the significance of a bit within a signal (we expect lsbs to flip almost every time, and msbs to flip very rarely), and the conditional probability features distinguish adjacent bits that fall on opposite sides of a signal boundary (e.g. we expect a bit to flip every 
% time a bit to its right flips if they are part of the same signal, but very rarely if they are not).

% \medskip

% While there is a specific formula for calculating whether the leading digit of a set of numbers in an arbitrary base satisfies Benford's law for, the case for base 2 is trivial, and we instead simply adopt the general idea \textemdash large leading significant digits occur much less frequency than small ones. 
% In our features, we consider the probability distribution of each pair of adjacent bits, with the motivation that the two most significant bits of a signal will have a different probability distribution than less significant pairs.  

% \medskip

% \textit{\underline{Entropy}} \\


%After generating this base features list, we will then generate features that allow the consideration of the base features for bits further along or behind in the message, that is,
% Without these look forward/backward features a cut may not be realized since we are attempting to predict whether to cut between bits $i$ and $i+1$, and a strong feature may be related to the characteristics of bit $i-1$.

% we compute the differences between the base features of the current bit $i$ and the corresponding feature to the left, $i-1$, and to the right, $i+1$. We then add these 34 \textit{difference features} $\delta(v^{id}_{i-1}, v^{id}_{i})$, $\delta(v^{id}_{i}, v^{id}_{i+1})$ to our feature set. 





% \subsubsection{Signal Boundary Labeling}
% \label{sec:bit_cut_labeling}

% % For training and validation one must have DBCs for the captures to provide labels. 
% For a given log, we obtain the ground truth labels for cuts,$y$, from a DBC for that vehicle (see Fig.\ref{fig:feature_extraction_labeling} (bottom)). We extract the message definitions for each of the IDs, and then create a label vector 
% $y \in \{0,1\}^{m_{id}}$, where each element $y_i$ denotes whether or not the gap to the right of bit $i$ is a signal boundary. Note that this vector of length $m_{id}$, because we do not include bits that are constant in a log, even if they are defined in the DBC. 


% For training a machine learning classifier, a sufficient amount of labeled data is necessary to get valid results. 
% Therefore, the algorithm will need to allow multiple CAN captures from different vehicles to be fed into the feature generation. 
% Note that each capture's features are generated in isolation; they are not merged until each feature set is calculated per ID. 
% Merging the information beforehand would skew results as different captures would be taken at different times and some cars have the same IDs which would artificially inflate each ID trace. 

% This process of generating a feature array will be performed on each ID trace for capture.
% When finished there will be a feature array $f \in \mathbb{R}^{m\times100}$ where $m$ is the total number of non-constant bits across all the ID's in the captures.
% It is important that if we have multiple captures from one vehicle those captures should be merged before feature generation into one larger capture.
% Note, an ($n+1$-bit) message has $n$ gaps between adjacent bits that will be labeled as a ``cut'' meaning where a signal starts/ends.  

% \subsubsection{Predicting Boundary Probabilities}

% Armed with these features and labels, we seek to train a supervised algorithm to accurately predict the cuts for a new data log. For training successful vehicle-agnostic classifier, we require  sufficient amount of labeled data from a variety of vehicle makes and years. In order to train a model, we aggregate each of the feature arrays $X$ and and label vectors $y$, which we then use to train a classifier.



% After loading all the captures, a \textit{full feature array} containing multiple vehicles' captures can be generated. 
% This array can be defined as $X \in \mathbb{R}^{M\times100}$ where $M$ is the total number of non-constant bits across all captures. 
% $X$ is the concatenation of the feature arrays, $X^{id, k}$ for each ID and data capture. 
% A \textit{full target array} containing multiple vehicles' captures is also generated, this array can be defined as $y \in \{0,1\}^M$.
% $y$ is the concatenation of the target array, $t$ from each vehicle.




% \begin{table*}[h]
%     \centering
%     \begin{threeparttable}[b]
%         \caption{Base Features}
%         \label{tb:features}
%         \begin{tabular}{c c c c}
%             \toprule
%             \textbf{Bit Value Prob}  & \textbf{Bit Flip Prob} & \textbf{Benford State Prob}  & \textbf{Entropy}\\
%             \midrule
%             $P(B_i = 0)$ & $P(B_i(t) \neq B_i(t+1))$ &  $P(B_i, B_{i+1} = 0, 0$) &  $H(B_i)$ \\
%             $P(B_i = 0 \mid B_{i+1} = 0)$ & $P(B_i(t) \neq B_i(t+1) \mid B_{i+1}(t) \neq B_{i+1}(t+1))$ & $P(B_i, B_{i+1} = 1, 0$) &  $H(B_i, B_{i+1})$ \\
%             $P(B_{i+1} = 0 \mid  B_i = 0)$ & $P(B_{i+1}(t) \neq B_{i+1}(t+1) \mid B_i(t) \neq B_i(t+1))$ &   $P(B_i, B_{i+1} = 0, 1$) &  $H(B_i\dots B_{i+3})$ \\
%             $P(B_i = 1 \mid  B_{i+1} = 1)$ & $P(B_i(t) = B_i(t+1))$  &  $P(B_i, B_{i+1} = 1, 1$) &  \\
%             $P(B_{i+1} = 1 \mid  B_i = 1)$ & $P(B_i(t) \neq B_i(t+1) \mid B_{i+1}(t) = B_{i+1}(t+1))$ &&\\
%              & $P(B_i(t) = B_i(t+1) \mid B_{i+1}(t) \neq B_{i+1}(t+1))$&&\\
%              & $B_{i+1}(t) \neq B_{i+1}(t+1) \mid P(B_i(t) \neq B_i(t+1))$&&\\
%             \bottomrule
%         \end{tabular}
        
%     \end{threeparttable}
% \end{table*}

% \begin{table*}[ht]
%     \centering
%     \begin{threeparttable}[b]
%         \caption{Base Features}
%         % \label{tb:features}
%         \begin{tabular}{c c c c}
%             \toprule
%             \textbf{Bit Flip Probability}  & \textbf{Count Probability} & \textbf{Entropy} & \textbf{Benford State Probability}  \\ 
%             \midrule
%           $P(b_i\, \text{ flips})$  & $P(b_i = 1\, |\, b_{i+1} = 1)$ & $H(b_{i} \ldots b_{i+7})$ & $P(b_{i},b_{i+1} = 0,0)$\\ 
%             $P(b_i\, \text{ flips}\, |\, b_{i+1}\, \text{ flips})$  & $P(b_{i+1} = 1\, |\, b_i = 1)$ & $H(b_{i} \ldots b_{i+3})$ & $P(b_{i},b_{i+1} = 0,1)$\\
%             $P(b_{i+1}\, \text{ flips}\, |\, b_i\, \text{ flips})$  & $P(b_i = 0)$ & $H(b_{i}, b_{i+1})$ & $P(b_{i},b_{i+1} = 1,0)$  \\
%             $P(b_i\, \neg\, \text{ flips})$ &  $P(b_i = 0\, |\, b_{i+1} = 0)$ & $H(b_{i})$ & $P(b_{i},b_{i+1} = 1,1)$ \\
%             $P(b_i\, \text{ flips}\, |\, b_{i+1}\, \neg \,\text{flips})$ & $P(b_{i+1} = 0\, |\, b_{i} = 0)$  \\
%             $P(b_i\, \neg \,\text{ flips}\, |\, b_{i+1}\, \text{flips})$ &   \\
%             $P(b_{i+1}\, \neg \,\text{ flips}\, |\, b_i\, \neg\, \text{ flips})$ & \\ \bottomrule
%         \end{tabular}
        
%     \end{threeparttable}
% \end{table*}



% From a known DBC and a matching CAN log, we create a binary vector for each ID $y^{id}\in \{0,1\}^{m_{id}-1}$ giving the labels for training/testing. 
% While this is straightforward for big endian signals, note that little endian signals have adjacent bits with non-adjacent indices at byte boundaries. 
% Using the example of Sec. \ref{sec:can-basics} for illustration, if the first two bytes are a little endian signal we have indices $8\rightarrow 0$.  
% Our features encode information of neighboring bits and must be extracted from ID traces before endianness is known. 
% Big endian and little endian entail different bit orderings at byte boundaries; consequently, during feature generation we do not know which bits to consider as  neighbors. 
% % non-adjacent bits are within-signal neighbors. % cannot during feature generation know which signals are little or big endian.  
% For the purpose of training/testing the machine learning model we split little endian signals on byte boundaries. 
% This is reconciled in ACTT 2.0's step 2 (Sec. \ref{sec:endianess_opt}), which considers neighboring bits from both little and big endian options at each byte when using this machine learning model as part of an optimization process that  extracts full little endian signals.  
% For evaluation against the signal boundary identification of previous methods, this means they are not penalized for assuming that all signals are big endian.  

% \begin{table}[ht]
% \small
%     \centering
%     \begin{threeparttable}[b]
%         \caption{Local Features}
%         \label{tb:features}
%         \begin{tabular*}{.48\textwidth}{ll}
%             %\addtolength{\tabcolsep}{-2pt}
%             \toprule
%             \textbf{Bit Values }  & \textbf{Bit Flips } \\
%             \midrule
%             $P(B_i = 0)$ & $P(B_i(t_j) \neq B_i(t_{j+1}))$\\
%             $P(B_i = 0 \mid B_{i+1} = 0)$ & $P(B_i(t_j) \neq B_i(t_{j+1}) \mid B_{i+1}(t_j) \neq B_{i+1}(t_{j+1}))$\\

%             $P(B_{i+1} = 0 \mid  B_i = 0)$ & $P(B_{i+1}(t_j) \neq B_{i+1}(t_{j+1}) \mid B_i(t_j) \neq B_i(t_{j+1}) )$\\
%             $P(B_i = 1 \mid  B_{i+1} = 1)$ & $P(B_i(t_j) = B_i(t_{j+1}) \mid B_{i+1}(t_j) = B_{i+1}(t_{j+1}))$\\
%             $P(B_{i+1} = 1 \mid  B_i = 1)$ & $P(B_{i+1}(t_j) = B_{i+1}(t+1) \mid B_i(t) = B_i(t_{j+1}))$\\
%             \midrule
%             \textbf{Benford}  & \textbf{Entropy} \\
%             \midrule
%             $P(B_i, B_{i+1} = 0, 0)$ &  $H(B_i)$ \\
%             $P(B_i, B_{i+1} = 1, 0)$ &  $H(B_i, B_{i+1})$ \\
%             $P(B_i, B_{i+1} = 0, 1)$ &  $H(B_i\dots B_{i+3})$ \\
%             $P(B_i, B_{i+1} = 1, 1)$ &  \\
%             \bottomrule
%         \end{tabular*}
        
%     \end{threeparttable}
% \end{table}



==> CAN-D IEEE/discussion.tex <==
 

  
\subsection{Discussion}
\label{sec:discussion}
\add{Discussion of results and comparisons}
This metric for error penalizes incorrectly classified signed signals more than little endian signals that have been incorrectly classified as multiple big endian signals. The reason for this is that for an incorrectly signed signal, when the signal takes on a negative value (for example -1), this will be very far from the value it takes if it is incorrectly classified as unsigned (max value). However, for little endian signals classified incorrectly as 2 big endian signals, the most significant byte signal will be paired with the 2 byte little endian signal, and once normalized, the $\ell_1$ error will be quite small since most of the information is encoded in the more significant byte. The lease significant byte on the other hand (which will just look like noise vacillating between the min and max value), will be paired with the 0 vector, and will have a medium sized error. Also note that the errors are not weighted by token weight, so while little endian signals are long (must be more than one byte), there are relatively few of them, so they have a somewhat small impact on the scores. 

For TANG, the reason it seems to do so poorly on cutting is because of the strict monotonically decreasing req on transition probabilities. It appears that the last couple LSBs of signals often seem to increase slightly, so it cuts preemptively. The high errors in signal difference can also be attributed to low precision since many additional short spurious signals will impact the score negatively.

For all other methods, the score is significantly worse for the two captures with Little Endian signals (5, 7). 

Note that log 3, whcih is the only one we lose on, has a lot of checksums.



Reminder: Write sentence or two indicating that the main way to push this forward would be to improve the signal boundary classification step. 

==> OLD-ml-eval.tex <==
\subsection{Evaluate Classifiers for Step 1}
\label{sec:eval-step1}
% \subsubsection{Step 1 Evaluation}
% \label{sec:eval-step1}

\textit{Cut prob ML model evaluation, tables, conclusions. Ultimately we chose RF with 100 estimators and these features for our pipeline. }

 \add{Bobby: try to rewrite this nicer, shorter. plan to keep the Table 2, and depending on coding progress, we'll reference to Appendix for feature selection} 
 
% We collected CAN data on six vehicles dated 2013, 2015, 2016 and 2017 of six different makes and using both combustion engine and hybrid vehicles. 
% Data was captured from these vehicles using a Kvaser Leaf Lite VS (www.kvaser.com) providing CAN-to-USB translation to a Linux OS laptop using SocketCan Software (https://elinux.org/Can-utils). 
After capturing and aggregating the data we performed a leave-one-AID-out cross validation across multiple classifiers.
Note that each vehicle is a separate model and trim and that if there were multiple captures from the same vehicles they would be trained together, as testing with a vehicle that we had trained on would give metrics that are not credible. 
Leave-one-AID-out has us training on all the AIDs but one and testing on leftover AID, this process is repeated until each AID is the validation set. 
% The per AID confusion matrix is micro-averaged and reported in Table \ref{tb:aid}.

For our classifiers we used the Python library SciKit \cite{scikit-learn}. 
The general classifiers used were: logistical regression, support-vector machine classifier, decision trees, and random forest. 
We tested two different logistical regression classifiers.
% Both used a max iteration of 10,000 and a constant random state. 
However, one had balanced class weights, the other had no class weights the rest of the parameters were set to default. 
Eight support-vector machine classifiers were tested with either balanced class weight or no class weights, constant random states, and each with a different kernel: radial basis function, linear, polynomial (power of 3), sigmoid. 
Only one decision tree classifier was tested.% and it was configured with a constant random state. 
Four random forest classifiers were included. 
One had 10 estimates with balanced class weights, another with 10 estimators with no balancing, another with 100 estimators with balanced class weights, and another with 100 estimators with no weights. 
Micro-average results from running leave-one-AID-out are listed in Table \ref{tb:aid}.
\begin{table}[ht]
    \centering
    \begin{threeparttable}[b]
        \caption{Micro Average Results of Leave-One-Out by AID}
        \label{tb:aid}
        
        \begin{tabular*}{0.45\textwidth}{llll}
            \toprule
            \textbf{Classifier} & \textbf{F-Score} & \textbf{Precision} & \textbf{Recall} \\ \midrule
            
            Log Reg OVR & 90.2 & 94.2 & 86.6 \\
            Log Reg OVR (bal.) & 86.9 & 82.5 & 91.8 \\
            
            SVC linear & 91.0 & 94.2 & 88.0 \\
            SVC linear (bal.) & 87.5 & 84.3 & 90.9 \\
            SVC poly & 65.3 & \textbf{96.5} & 49.4 \\
            SVC poly (bal.) & 75.7 & 62.8 & \textbf{95.2} \\
            SVC RBF & 91.3 & 95.9 & 87.2 \\
            SVC RBF (bal.) & 90.2 & 87.4 & 93.2 \\
            SVC sigmoid & 60.5 & 62.7& 58.4 \\
            SVC sigmoid (bal.) & 52.6 & 40.4 & 75.4 \\
            
            Decision tree & 89.1 & 89.1 & 89.1 \\
            
            RF - 10 Est. & 92.2 & 94.0 & 90.5 \\
            RF (bal.) - 10 Est. & 91.7 & 94.2 & 89.3 \\
            RF - 100 Est. & \textbf{92.8} & 94.2 & 91.5 \\
            RF (bal.) - 100 Est. & 92.1 & 93.7 & 90.5 \\
            \bottomrule
        \end{tabular*}
        
    \end{threeparttable}
\end{table}


Note, our precision is normally higher than our recall. 
This fact is to be expected since we have biased classes, specifically, a larger amount of instances in our training data where there should not be a cut compared to there being a cut. 
Across the six cars' data we have 3,868 instances of when the bit should not cut to the `right' and 944 instances where the bit should be cut to the `right'; therefore, the base-rate of the data is approximately 4:1.
Because of this imbalance in our class representation we have a biased class issue. 
We attempted to combat this issue by balancing the class weights. 
Balancing class weights allow classes that are disproportionately represented to be better represented. 
However, as one can see in Table \ref{tb:aid} using balancing techniques did not increase our overall F-Score.

An additional attempt to increase our metrics was feature selection. The general idea is to eliminate spurious features, that is features that lower classification abilities. 
We used feature selection algorithms false discovery rate and mutual info  on a random forest classifier.
False discovery rate and mutual info feature selection are provided by Scikit Learn \cite{scikit-learn}. 
In the end feature selection did not have a meaningful impact, metrics did not increase with only select features included. 
Interestingly, near optimal classification metrics are obtained with ultimately few features.
Overall, we exhibited a train classifier that can achieve over 92\% F-Score in tokenzing signals from can data captures. 
The results of this can be seen in Table \ref{tb:selection}. 



The Top 10 Features across all five of the vehicles with False Discovery Rate can be seen in Table \ref{tb:top_fdr} and the top for Mutual Class can be seen in Table \ref{tb:top_mutual}.


% \subsubsection{Step 3 Evaluation}
% \label{sec:eval-step3}
% \textit{Signedness classification model evaluation, tables, conclusions. Ultimately, we chose to use the heuristics in our pipeline rather than any learned model.}

% Here we followed the same setup as Section \ref{sec:eval-step1}.
% Additionally we tested two rule-based algorithms against our machine learning classifiers.
% The Benford Rule and Flip-Based Rule defined in Algorithm \ref{rules}. 
% The parameter $X$ used in Algorithm \ref{rules} is the total feature array discussed in Section \ref{sec:cutprob}

% \smallskip
% \begin{algorithm}[h]
%   \caption{Rules}\label{rules}
%   \label{alg:1} 
%   \begin{algorithmic}
%   \Function{BenfordRule}{$X$}
%     \State $\hat{y} \gets \emptyset$
%     \For{$i$ in $\text{len}(X)$}
%         \If{$(X_{i3} + X_{i2} < .1 )$ \& $(X_{i4} > X_{i3})$}
%             \State $\hat{y}_i \gets \text{True}$
%         \Else
%             \State $\hat{y}_i \gets \text{False}$
%         \EndIf
%     \EndFor
%     \State \textbf{return} $\hat{y}$
%     \EndFunction


%     \smallskip


%   \Function{FlipRule}{$X \text{, flips}$}
%     \State $\hat{y} \gets \emptyset$
%     \For{$i$ in $\text{len}(X)$}
%         \If{$(X_{i3} + X_{i2} = 0$}
%             \State $\hat{y}_i \gets \text{True}$
%         \ElsIf{$\text{flips}_{i} = 0$}
%             \State $\hat{y}_i \gets \text{False}$
%         \ElsIf{$X_{i3} + X_{i2} < .1$}
%             \State $\hat{y}_i \gets \text{True}$
%         \Else
%             \State $\hat{y}_i \gets \text{False}$
%         \EndIf
%     \EndFor
%     \State \textbf{return} $\hat{y}$
%     \EndFunction
%   \end{algorithmic}
% \end{algorithm}

% Note the rule-based algorithms do not actually use the training data. 
% Instead, each will simply apply their heuristic to label the test data.
% Micro Average Results from running leave-one-AID-out are listed in table \ref{tb:signal}



% \begin{table*}[h]
%     \centering
%     \begin{threeparttable}[b]
%         \caption{Micro Average Results of Leave-One-Out Grouped by AID}
%         \label{tb:signal}
        
%         \begin{tabular*}{.45\textwidth}{l l l l}
%             \toprule
%             \textbf{Classifier} & \textbf{F-Score} & \textbf{Precision} & \textbf{Recall} \\ \midrule
%                 Log Reg OVR & 23.5 & 75.0 & 13.9 \\
%                 Log Reg OVR (bal.) & 66.1 & 49.4 & \textbf{100.0} \\
%                 SVC Linear & 69.8 & 72.5 & 67.4 \\
%                 SVC Linear (bal.) & 71.0 & 55.1 & \textbf{100.0} \\
%                 SVC Poly & 72.2 & 89.6 & 60.4\\ 
%                 SVC Poly (bal.) & 65.6 & 49.4 & 97.6 \\ 
%                 SVC RBF & 0.0 & 0.0 & 0.0\\
%                 SVC RBF (bal.) & 64.6 & 47.7 & \textbf{100.0}\\
%                 SVC Sigmoid & 15.1 & 16.6 & 13.9 \\
%                 SVC Sigmoid (bal.) & 18.2 & 11.2 & 48.8 \\
%                 Decision Tree & 87.6 & 84.7 & 90.7\\
%                 RF - 10 Est. & 90.0 & 97.3 & 83.7 \\
%                 RF (bal.) - 10 Est. & 94.1 & 95.2 & 93.0 \\
%                 RF - 100 Est. & 92.8 & 95.1 & 90.7 \\
%                 RF (bal.) - 100 Est. & 92.8 & 95.1 & 90.7 \\
%                 Benford Rule & 95.4 & 93.3 & 97.6 \\
%                 Zero Flip Rule & \textbf{97.6} & \textbf{97.6} & 97.6 \\
%             \bottomrule
%         \end{tabular*}
        
%     \end{threeparttable}
% \end{table*}


% From these results one can see how the rule-based algorithms performed far better than any classifier. 
% However with this specific dataset we only have 408 signals to test on but with tokenization we have 4812 bits to test on.
% With more data the chance of a classifier performing better than the rule will hopefully increase.
% Additionally we believe we can use machine learning to determine the threshold used during the rule based algorithms. 
% For our tests we set it to 0.1, but that was an arbitrary decision that, we believe, can be improved with machine learning. 


==> cutprob.tex <==
\subsection{Learn Signal Boundary Probabilities}
\label{sec:cutprob}



% \begin{figure*}{\linewidth} 
% \begin{minipage}{.31\textwidth}
% % \begin{table}[!h]
% % \small
% %     \centering
%     \begin{threeparttable}
%         \caption{Local Features ($t$ and $t'$ denote subsequent timestamps)}
%         \label{tb:features}
%         \begin{tabular}{l}
%             \toprule
%             \textbf{Bit Values } \\
%             \midrule
%             $P(B_i = 0)$\\
%             $P(B_i = 0 \mid B_{i+1} = 0)$\\
%             $P(B_{i+1} = 0 \mid  B_i = 0)$ \\
%             $P(B_i = 1 \mid  B_{i+1} = 1)$\\
%             $P(B_{i+1} = 1 \mid  B_i = 1)$\\
%             \midrule
%             \textbf{Bit Flips } \\
%             \midrule
%             $P(B_i(t) \neq B_i(t'))$\\
%             $P(B_i(t) \neq B_i(t') \mid B_{i+1}(t) \neq B_{i+1}(t'))$\\
%             $P(B_{i+1}(t) \neq B_{i+1}(t') \mid B_i(t) \neq B_i(t') )$\\
%             $P(B_i(t) = B_i(t') \mid B_{i+1}(t) = B_{i+1}(t'))$\\
%             $P(B_{i+1}(t) = B_{i+1}(t') \mid B_i(t) = B_i(t'))$\\
%             \midrule
%             \textbf{Benford}  \\
%             \midrule
%             $P(B_i, B_{i+1} = 0, 0)$\\
%             $P(B_i, B_{i+1} = 1, 0)$  \\
%             $P(B_i, B_{i+1} = 0, 1)$  \\
%             $P(B_i, B_{i+1} = 1, 1)$ \\
%             \midrule
%             \textbf{Entropy}\\
%             $H(B_i)$\\
%             $H(B_i, B_{i+1})$\\
%             $H(B_i\dots B_{i+3})$ \\
%             \bottomrule
%         \end{tabular}
%      \end{threeparttable}
% %  \end{table}
%  \end{minipage}\quad
% \begin{minipage}{.67\textwidth}
%     \begin{figure*} 
%     \includegraphics[width=\linewidth]{figs/feature_generation_diagram.pdf}
%     \caption{(\textbf{Top}:) Process for creating a feature array from a ID trace. (\textbf{Bottom}:)  Subprocess for creating a feature vector for each bit gap.}
%     \label{fig:feature_gen}
%     \end{figure*}
% \end{minipage}%
% \end{figure*} 
 
 
% \begin{figure*}[H]
%     % \vspace{-1.2cm}
%   \centering
% \begin{minipage}{0.3\textwidth}
% \begin{table}[ht]
% \small
%     \centering
%     \begin{threeparttable}
%         \caption{Local Features ($t$ and $t'$ denote subsequent timestamps)}
%         \label{tb:features}
%         \begin{tabular*}{}{l}
%             %\addtolength{\tabcolsep}{-2pt}
%             \toprule
%             \textbf{Bit Values } \\
%             \midrule
%             $P(B_i = 0)$\\
%             $P(B_i = 0 \mid B_{i+1} = 0)$\\
%             $P(B_{i+1} = 0 \mid  B_i = 0)$ \\
%             $P(B_i = 1 \mid  B_{i+1} = 1)$\\
%             $P(B_{i+1} = 1 \mid  B_i = 1)$\\
%             \midrule
%             \textbf{Bit Flips } \\
%             $P(B_i(t) \neq B_i(t'))$\\
%             $P(B_i(t) \neq B_i(t') \mid B_{i+1}(t) \neq B_{i+1}(t'))$\\
%             $P(B_{i+1}(t) \neq B_{i+1}(t') \mid B_i(t) \neq B_i(t') )$\\
%             $P(B_i(t) = B_i(t') \mid B_{i+1}(t) = B_{i+1}(t'))$\\
%             $P(B_{i+1}(t) = B_{i+1}(t') \mid B_i(t) = B_i(t'))$\\
%             \midrule
%             \textbf{Benford}  \\
%             \midrule
%             $P(B_i, B_{i+1} = 0, 0)$\\
%             $P(B_i, B_{i+1} = 1, 0)$  \\
%             $P(B_i, B_{i+1} = 0, 1)$  \\
%             $P(B_i, B_{i+1} = 1, 1)$ \\
%             \midrule
%             \textbf{Entropy}
%             $H(B_i)$\\
%             $H(B_i, B_{i+1})$\\
%             $H(B_i\dots B_{i+3})$ \\
%             \bottomrule
%         \end{tabular*}
%     \end{threeparttable}
% \end{table}
% \end{minipage}%
%   \includegraphics[width=.7\linewidth]{figs/feature_generation_diagram.pdf}
%   \caption{(\textbf{Top}:) Process for creating a feature array from a ID trace. (\textbf{Bottom}:)  Subprocess for creating a feature vector for each bit gap.}
%   \label{fig:feature_gen}
% %   \vspace{-.7cm}
% \end{figure*}

% \begin{figure*}[h]
%   \centering
%   \includegraphics[width=\linewidth]{figs/feature_generation_diagram.pdf}
%   \caption{Top: Process for creating a feature array for each capture, which calls the 'Bit Feature Generation' subprocess; Bottom: Subprocess for creating a feature vector for each bit}
%   \label{fig:feature_gen}
%   \vspace{-.75cm}
% \end{figure*}

For each ID, the 64-bit message has 63 ``bit gaps'' indexed $(i,i+1)$ for $i = 0, \dots, 62$, and bits $i$ and $i+1$ are either contained in the same signal or span two signals. 
Previous works have focused on identifying signal boundaries using hand-crafted heuristics that leverage only two main features computed from an ID trace: each bit's flip probability and the range of values a candidate signal realizes.
%\textemdash and depended on the overly simplifying assumption that all signals are big endian and unsigned. 
The first step of CAN-D is to build a robust set of features for each gap and leverage well established statistical machinery from supervised machine learning to determine signal boundaries from the many features.  
This subsection describes the features and machine learning research used for this task and is represented in the top row of Fig. \ref{fig:pipeline}. 
In Sec. \ref{sec:eval} we evaluate our binary classification for signal boundary identification against the previous state-of-the-art methods. 
Finally, note that while we frame this as a binary classification problem, labelling each gap as signal boundary or not, the output needed for the second step of the CAN-D pipeline is not binary, but the estimated probability of a boundary at each gap. 


\textbf{Preprocessing}: 
Refer to Fig. \ref{fig:feature_gen}, which depicts the entire feature generation process for each ID trace (top) and then for each gap within the ID trace (bottom).
To build features from an ID trace,  we  first remove the constant bits. 
Sec. \ref{sec:test_data_types}, which discusses the many reasons for this. 
% as: (1) constant bits necessitate an adjacent signal boundary that need not be learned, 
% (2)  many features, which depend on nearby bit values and flips, are not defined for gaps adjacent to constant bits, and 
% (3) this counteracts the bias class problem, giving more adjacent signals to learn from in training. 
Denote the condensed ID trace $B^{\prime id} \in \{0,1\}^{n_{id}\times{m_{id}}}$ where $m_{id}$ is the number of non-constant bits for a given arbitration ID $id$. 
For each remaining $m_{id}-1$ bit gaps, we generate a set of 85 features: 17 features are ``local'' to the gap, examining only bits $i$ and $i+1$,
%and the bit directly to the left of the gap $(i, i+1)$ under inspection,
and the rest are from values of ``neighboring bits'' (e.g. bit $i-1$, bit $i+2$, etc.).

\begin{table}[b]
\small
    \centering
    \begin{threeparttable}[b]
        \caption{Local Features ($t$ and $t'$ denote subsequent timestamps)}
        \label{tb:features}
        \begin{tabular*}{.48\textwidth}{ll}
            %\addtolength{\tabcolsep}{-2pt}
            \toprule
            \textbf{Bit-Value }  & \textbf{Bit-Flip } \\
            \midrule
            $P(B_i = 0)$ & $P(B_i(t) \neq B_i(t'))$\\
            $P(B_i = 0 \mid B_{i+1} = 0)$ & $P(B_i(t) \neq B_i(t') \mid B_{i+1}(t) \neq B_{i+1}(t'))$\\

            $P(B_{i+1} = 0 \mid  B_i = 0)$ & $P(B_{i+1}(t) \neq B_{i+1}(t') \mid B_i(t) \neq B_i(t') )$\\
            $P(B_i = 1 \mid  B_{i+1} = 1)$ & $P(B_i(t) = B_i(t') \mid B_{i+1}(t) = B_{i+1}(t'))$\\
            $P(B_{i+1} = 1 \mid  B_i = 1)$ & $P(B_{i+1}(t) = B_{i+1}(t') \mid B_i(t) = B_i(t'))$\\
            \midrule
            \textbf{Benford}  & \textbf{Entropy} \\
            \midrule
            $P(B_i, B_{i+1} = 0, 0)$ &  $H(B_i)$ \\
            $P(B_i, B_{i+1} = 1, 0)$ &  $H(B_i, B_{i+1})$ \\
            $P(B_i, B_{i+1} = 0, 1)$ &  $H(B_i\dots B_{i+3})$ \\
            $P(B_i, B_{i+1} = 1, 1)$ &  \\
            \bottomrule
        \end{tabular*}
        
    \end{threeparttable}
\end{table}




\textbf{Local Features}:  We first generate the 17 local features for bits $i$ and $i+1$  (see Fig. \ref{fig:feature_gen} Bottom Left), which are denoted $v^{id}_i \in \mathbb{R}^{17}$. 
These local features belong to four categories and are listed in Table \ref{tb:features}.
% These encoding information about the bit $i$, the bit directly to the left of the gap $(i, i+1) $ under inspection.
\textit{Bit-Value}: The first bit-value feature, $P(B_i = 0)$, is motivated by the fact that the distribution of values differs significantly between the most and least significant bits of a signal; e.g., for LSBs $P(B_i = 0) \approx 0.5$ since LSBs frequently alternate values (for both signed and unsigned encodings). 
% only extreme (and therefore likely more unusual) signal values will take on value of 1, whereas LSBs flip more often. 
The next four bit-value features, are conditional bit-value probabilities (e.g. $P(B_{i+1} = 0 \mid  B_i = 0)$). 
These are expected to differ significantly for adjacent bits contained in the same signal vs. those that are part of separate signals, as the former are dependent while the latter are likely independent.  
% ; most notably, if bit $i$ is the LSB of one signal, and bit $i+1$ is the MSB of the adjacent signal, then $P(B_{i+1} = 0 \mid  B_i = 0) \approx 0$ since $P(B_{i+1} = 0) \approx 0$ and $P(B_{i} = 0) \approx .5$ for continuous signals. 
\textit{Bit-Flip}: We compute five analogous features, now for the probability that a bit ``flips'', i.e., alternates value in subsequent messages. 
The main intuition is that LSBs generally alternate values much more often than an adjacent signal's MSB; hence, the bit-flip features should provide good indicators for boundaries. 
Note that this is the feature that previous works build heuristics upon. 
\textit{Benford}: These features are based upon Benford's Law \cite{benfords}, 
%also known as the law of anomalous numbers. Benford's Law is 
an observation regarding the frequency distribution of leading digits $d$ of a base $b$ number, $P(d)=\log_{b} \left(1+\tfrac{1}{d}\right).$ %\log_b(d+1)-\log_b(d)
In base $b=10$, it states that $d=1$ appears as the significant digit $\smalltilde 30\%$ of the time, while $d=9$ appears as the leading significant digit less than $\smalltilde 5\%$.
While the law is trivial for base $b=2$, as an MSB is necessarily 1, we harness the intuition that the significant digits have a distinct distribution and include the distribution of 
%the gap's adjacent pair of bits 
the pair of bits $i$ and $i+1$ as local features. 
\textit{Entropy}: For the final three local features, we consider the entropy of bits $[i,\dots, i+j]$ for  $j \in \{0, 1, 3\}$. 
% The idea behind these features is to capture the amount of uncertainty in a short sequence of bits. 
We expect that sequences of bits that are part of the same physical signal will have very low entropy; whereas, sequences that contain bits from multiple signals will have higher entropy. 
% \add{One more sentence of explanation on entropy feature, why we expect this, and perhaps something about the entropy of checksums which violate the continuity assumpiton that all of the other features are based upon?}


\textbf{Neighboring bits' features}:  
We then forward/backward to neighboring bits (see Fig. \ref{fig:feature_gen} Bottom Right) and compute the same features for gaps $(i-1, i)$ and $(i+1, i+2)$;  thus, we add 34 more features by adding $v^{id}_{i-1}$ and $v^{id}_{i+1}$ to our feature set.  
In initial testing we experimented with adding more look forward/backward features and found that 1 in each direction was sufficient.
Finally, we another 34 difference features $v^{id}_{i}-v^{id}_{i-1}$ and $v^{id}_{i+1}-v^{id}_{i}$, yielding an 85-length feature vector for gap $(i, i+1)$. 

\textbf{Targets}: 
From a known DBC and a matching CAN log, we create a binary vector for each ID $y^{id}\in \{0,1\}^{m_{id}-1}$ giving the labels for training/testing. 
This is straightforward for big endian signals, yet, little endian signals have adjacent bits with non-adjacent indices at byte boundaries (see Eq. \ref{eq:bit-orderings}). 
%% Moved to next section: % Using the example of Sec. \ref{sec:can-basics} for illustration, if the first two bytes are a little endian signal we have neighboring indices $8\rightarrow 0$.  
% Our features require information from neighboring bits, but must be extracted from ID traces before endianness is known; yet endianness determines bit orders at byte boundaries (Eq. \ref{eq:bit-orderings}) . 
% Since big/little endian entail different bit orderings
%at byte boundaries; consequently, during feature generation 
% we do not know which bits to consider as  neighbors. 
% non-adjacent bits are within-signal neighbors. % cannot during feature generation know which signals are little or big endian.  
For training and testing the  model we split little endian signals on byte boundaries. 
For signal extraction, this is reconciled in CAN-D's step 2 (Sec. \ref{sec:endianess_opt}), which considers bit orderings of both endianness
%options at each byte when using this machine learning model as part of 
and uses an optimization process that accommodates extraction of full little endian signals.  
% When evaluating signal boundary identification, this means previous methods are not penalized for assuming that all signals are big endian.  



\textbf{Classifier}: 
We experimented with several classifiers and parameters including Decision Trees, Random Forests, Support Vector Classifiers, and Logistic Regression using Python's SciKit library.
% \cite{scikit-learn}. 
We also experimented with using balanced class weights, since we have high bias  towards the negative class (non-boundary gaps). 
See Sec. \ref{sec:dataset} for a description of data used. 
To examine the accuracy of the classifiers, we used Leave One (ID) Out Cross Validation (LOOCV), removing each ID from training and using it for testing, then microaveraging results. 
We found that Random Forest Regression with 100 Estimators and balanced class weights yielded the best results, with micro-averaged 94\% precision and 91.5\% recall for an F-Score of 93\%. 
Table \ref{tb:boundary_classifier_results} in \hyperref[sec:appendix]{Appendix} itemizes results for all the classifiers tested. 



The next step of our algorithm requires the inputs to be probabilities rather than binary labels, so for step 2 we use the classifier's un-thresholded output, a number in [0,1] interpreted as the probability of a cut at  gap $(i, i+1)$. 


% Following training, the model can then be exported to predict signal boundaries on a new dataset, which would be done online. 
% This process is shown in the white section of the first panel of Fig. \ref{fig:pipeline}. 

% After training, we let $f^{id}(i) \in [0,1]$ denote the output of the model, 
% which is the probability of a cut between bits $i$ and $i+1$ for ID $id$ in a given log. 



% \subsection{Tokenization Prediction}
% We use a trained classifier and a feature vector from unlabeled candata $X'$ into targets $y'$.
% % We describe the necessary steps to apply our trained model assuming one has a CAN data capture from a vehicle that they would like to tokenize. 
% Following the same process of aggregating the capture into ID traces, one can then generate a feature array based on the ID traces. 
% Once the feature array is generated it is fed to the trained classifier, and a prediction array is returned for each ID which can be defined as $P \in [0,1]^{b}$ with $b$ being the number of non-constant bits of the specific ID trace. 


% \begin{figure}[ht]
%     \includegraphics[width=.5\textwidth]{figs/bit_cut_feature_extraction_and_labeling_process.pdf}
%     \caption{As supervised binary classification is used for learning signal boundaries, the diagram depicts (\textbf{top}:)  how a CAN log is transformed into a feature vector array and (\textbf{bottom}:) how the corresponding DBC is transformed into a binary array of labels of the signal boundaries. 
%     \fix{in figure, change "bit cut" to "signal boundary" }
%     \fix{change figure headers to say signal boundary, remove ks, and use word log instead of capture} 
%     \fix{transpose figures, so that processes move from top to bottom, put side by side, and move next to \ref{fig:feature_gen}}}
%     \label{fig:feature_extraction_labeling}
% \end{figure}



% The tokenization pipeline consists of four main components: (1) data pre-processing, (2) feature and target generation, (3) model training, (4) tokenization prediction.


% Based on Assumption 4, we consider constant bits to necessarily delimit signals, and thus any 

% It is imperative that we capture CAN data that encompasses all of the vehicles functionalities so that all the bits are being exercised in their defined signals. 
% If not, some signals' most significant bits may not change and seem to appear constant, and get discarded mistakenly. 

% Therefore any valid signal must contain any contiguous set of bits that does not contain constant bits. 
% After grouping and filtering the ID traces, features can be calculated for each bit per trace. 

% and build $X \in {id} \in \mathbb{R}^{85}$. This entire Feature Generation process is depicted in  Fig. \ref{fig:feature_gen} (top). 
% The subprocess for generating these feature for each bit is described in the following sections \ref{sec:base_features}-\ref{sec:non_base_features}, and is depicted in Fig. \ref{fig:feature_gen} (bottom). 


%  are part of the same signal or separate signals based on characteristics of a bit's value, how its value changes over time, and how these characteristics relate to those of the surrounding bits. 
% Formally, we define a set of features $X_i$ for bit $i$, and try to predict $y_i \in \{0,1\}$ where $y_i = 0$ denotes that bits $i$ and $i+1$ are part of the same signal, and $y_i=1$ denotes that there is a signal boundary between bits $i$ and $i+1$.
% We build this set of features and ground truth labels, and train a classification model offline. 
% This is shown in the top left gray portion of Fig. \ref{fig:pipeline}. This consists of two main components, "Signal Boundary Feature Extraction Process" and "Signal Boundary Labeling Process", which are illustrated in Fig. \ref{fig:feature_extraction_labeling}, and explained in \ref{sec:bit_cut_feature_extraction}-\ref{sec:non_base_features} and \ref{sec:bit_cut_labeling} respectively. 

% \subsubsection{Signal Boundary Feature Extraction}
% \label{sec:bit_cut_feature_extraction}


% To build features, we first separate the sequence of data fields in a log by ID, building a set of \textit{ID traces}. 
% We define an ID \textit{trace} $B^{id} \in \{0,1\}^{n_{id}\times64}$ to be the set of $n_{id}$ 64-bit messages sent on a particular arbitration $id$ over the course of a CAN log.


% We denote the $i$\textsuperscript{th} bit of the message sent at time $t$ as $B^{id}_i(t)$, where $i \in [0,...63]$ and bits are numbered in order of transmission on the bus (normal, not sawtooth numbering). 
%Note that, a message can have fewer than 8 bytes of data, so we pad any shorter messages with zeros. 
% We then remove all of the constant bits from each ID trace, we are left with \textit{non-constant ID trace} $B^{\prime id} \in \{0,1\}^{n_{id}\times{m_{id}}}$ where $m_{id}$ is the number of non-constant bits for a given arbitration ID $id$. 
%The reason why we use the non-constant traces $B^{\prime id}$ is because our features depend on how bit values change, and based on Assumption 4, we consider constant bits to necessarily delimit signals. 
%\add{Furthermore, because the most significant bits of signals are unchanging when extreme values are not reached, constant bits will naturally delimit signals. We smash signals together to make for better training data. Explain further in \ref{sec:eval-step1}}

% $for each bit $i$ in the nonconstant trace $B^{\prime id}$ for ID $id$. These base features, which are listed in Table \ref{tb:features} fall into four feature categories: bit value probabilities, bit flip probabilities, Benford state probabilities, and entropy. 

% \add{Note that many of these features are combinations of one another; we plan to do feature selection, and put in some redundancies in order to determine which features were the most important}

% This subsection describe how we convert the arrays of parsed candata into a feature array $X$ and DBCs into a target vector $y$.
% After grouping and filtering the can data into ID traces, features can be calculated for each bit position $j = 0, \ldots 63$ per trace; that is for each trace, for each $j = 0, \ldots 63$ we will compute a feature vector.
% Overall we compute 100 features, the first twenty are base features which are listed in Table \ref{tb:features}. 
% \medskip


% \textit{\underline{Bit Value Probabilities}} \\
% We compute 5 features relating to the probability of a bits value, and the conditional probability of its value given the value of the bit to its right (also condition in opposite direction). 
% bits that are towards the right end of a signal (least significant) than for bits that are towards the left end (most significant). 
 
%$P(B_i = 0) \approx .5$ for the least significant bit of a continuous signal as it will flip between 0 and 1 every time the value of the signal is incremented or decremented by 1. Similarly, for the most significant bit,  $P(B_i = 0) \approx 1$ since only extreme (and therefore likely more unusual) signal values will take on value of 1. 

% For example, if bits $i$ and $i+1$ are part of the same signal $P(B_{i+1} = 0 \mid  B_i = 0) \approx .5$ because each bit will take on value 0 roughly half the time that the next less significant bit will. However, if this is unlikely to be true if they are from different signals, most notable if bit $i$ is the lsb of one signal, and bit $i+1$ is the msb of the adjacent signal, then $P(B_{i+1} = 0 \mid  B_i = 0) \approx 0$ since $P(B_{i+1} = 0) \approx 0$ and $P(B_{i} = 0) \approx .5$. 

% \medskip
% \textit{\underline{Bit Flip Probabilities}} \\


% Similarly to the bit value features, we compute 5 bit flip probability features which are based on the probability of a bits value flipping between two successive messages, as well as the probability of a bits value flipping conditioned on whether the bit to its right flips. The motivations are similar to those of the bit value features: the non-conditional probability feature, $P(B_i(t) \neq B_i(t+1))$, serves as an indicator of the significance of a bit within a signal (we expect lsbs to flip almost every time, and msbs to flip very rarely), and the conditional probability features distinguish adjacent bits that fall on opposite sides of a signal boundary (e.g. we expect a bit to flip every 
% time a bit to its right flips if they are part of the same signal, but very rarely if they are not).

% \medskip

% While there is a specific formula for calculating whether the leading digit of a set of numbers in an arbitrary base satisfies Benford's law for, the case for base 2 is trivial, and we instead simply adopt the general idea \textemdash large leading significant digits occur much less frequency than small ones. 
% In our features, we consider the probability distribution of each pair of adjacent bits, with the motivation that the two most significant bits of a signal will have a different probability distribution than less significant pairs.  

% \medskip

% \textit{\underline{Entropy}} \\


%After generating this base features list, we will then generate features that allow the consideration of the base features for bits further along or behind in the message, that is,
% Without these look forward/backward features a cut may not be realized since we are attempting to predict whether to cut between bits $i$ and $i+1$, and a strong feature may be related to the characteristics of bit $i-1$.

% we compute the differences between the base features of the current bit $i$ and the corresponding feature to the left, $i-1$, and to the right, $i+1$. We then add these 34 \textit{difference features} $\delta(v^{id}_{i-1}, v^{id}_{i})$, $\delta(v^{id}_{i}, v^{id}_{i+1})$ to our feature set. 





% \subsubsection{Signal Boundary Labeling}
% \label{sec:bit_cut_labeling}

% % For training and validation one must have DBCs for the captures to provide labels. 
% For a given log, we obtain the ground truth labels for cuts,$y$, from a DBC for that vehicle (see Fig.\ref{fig:feature_extraction_labeling} (bottom)). We extract the message definitions for each of the IDs, and then create a label vector 
% $y \in \{0,1\}^{m_{id}}$, where each element $y_i$ denotes whether or not the gap to the right of bit $i$ is a signal boundary. Note that this vector of length $m_{id}$, because we do not include bits that are constant in a log, even if they are defined in the DBC. 


% For training a machine learning classifier, a sufficient amount of labeled data is necessary to get valid results. 
% Therefore, the algorithm will need to allow multiple CAN captures from different vehicles to be fed into the feature generation. 
% Note that each capture's features are generated in isolation; they are not merged until each feature set is calculated per ID. 
% Merging the information beforehand would skew results as different captures would be taken at different times and some cars have the same IDs which would artificially inflate each ID trace. 

% This process of generating a feature array will be performed on each ID trace for capture.
% When finished there will be a feature array $f \in \mathbb{R}^{m\times100}$ where $m$ is the total number of non-constant bits across all the ID's in the captures.
% It is important that if we have multiple captures from one vehicle those captures should be merged before feature generation into one larger capture.
% Note, an ($n+1$-bit) message has $n$ gaps between adjacent bits that will be labeled as a ``cut'' meaning where a signal starts/ends.  

% \subsubsection{Predicting Boundary Probabilities}

% Armed with these features and labels, we seek to train a supervised algorithm to accurately predict the cuts for a new data log. For training successful vehicle-agnostic classifier, we require  sufficient amount of labeled data from a variety of vehicle makes and years. In order to train a model, we aggregate each of the feature arrays $X$ and and label vectors $y$, which we then use to train a classifier.



% After loading all the captures, a \textit{full feature array} containing multiple vehicles' captures can be generated. 
% This array can be defined as $X \in \mathbb{R}^{M\times100}$ where $M$ is the total number of non-constant bits across all captures. 
% $X$ is the concatenation of the feature arrays, $X^{id, k}$ for each ID and data capture. 
% A \textit{full target array} containing multiple vehicles' captures is also generated, this array can be defined as $y \in \{0,1\}^M$.
% $y$ is the concatenation of the target array, $t$ from each vehicle.




% \begin{table*}[h]
%     \centering
%     \begin{threeparttable}[b]
%         \caption{Base Features}
%         \label{tb:features}
%         \begin{tabular}{c c c c}
%             \toprule
%             \textbf{Bit Value Prob}  & \textbf{Bit Flip Prob} & \textbf{Benford State Prob}  & \textbf{Entropy}\\
%             \midrule
%             $P(B_i = 0)$ & $P(B_i(t) \neq B_i(t+1))$ &  $P(B_i, B_{i+1} = 0, 0$) &  $H(B_i)$ \\
%             $P(B_i = 0 \mid B_{i+1} = 0)$ & $P(B_i(t) \neq B_i(t+1) \mid B_{i+1}(t) \neq B_{i+1}(t+1))$ & $P(B_i, B_{i+1} = 1, 0$) &  $H(B_i, B_{i+1})$ \\
%             $P(B_{i+1} = 0 \mid  B_i = 0)$ & $P(B_{i+1}(t) \neq B_{i+1}(t+1) \mid B_i(t) \neq B_i(t+1))$ &   $P(B_i, B_{i+1} = 0, 1$) &  $H(B_i\dots B_{i+3})$ \\
%             $P(B_i = 1 \mid  B_{i+1} = 1)$ & $P(B_i(t) = B_i(t+1))$  &  $P(B_i, B_{i+1} = 1, 1$) &  \\
%             $P(B_{i+1} = 1 \mid  B_i = 1)$ & $P(B_i(t) \neq B_i(t+1) \mid B_{i+1}(t) = B_{i+1}(t+1))$ &&\\
%              & $P(B_i(t) = B_i(t+1) \mid B_{i+1}(t) \neq B_{i+1}(t+1))$&&\\
%              & $B_{i+1}(t) \neq B_{i+1}(t+1) \mid P(B_i(t) \neq B_i(t+1))$&&\\
%             \bottomrule
%         \end{tabular}
        
%     \end{threeparttable}
% \end{table*}

% \begin{table*}[ht]
%     \centering
%     \begin{threeparttable}[b]
%         \caption{Base Features}
%         % \label{tb:features}
%         \begin{tabular}{c c c c}
%             \toprule
%             \textbf{Bit Flip Probability}  & \textbf{Count Probability} & \textbf{Entropy} & \textbf{Benford State Probability}  \\ 
%             \midrule
%           $P(b_i\, \text{ flips})$  & $P(b_i = 1\, |\, b_{i+1} = 1)$ & $H(b_{i} \ldots b_{i+7})$ & $P(b_{i},b_{i+1} = 0,0)$\\ 
%             $P(b_i\, \text{ flips}\, |\, b_{i+1}\, \text{ flips})$  & $P(b_{i+1} = 1\, |\, b_i = 1)$ & $H(b_{i} \ldots b_{i+3})$ & $P(b_{i},b_{i+1} = 0,1)$\\
%             $P(b_{i+1}\, \text{ flips}\, |\, b_i\, \text{ flips})$  & $P(b_i = 0)$ & $H(b_{i}, b_{i+1})$ & $P(b_{i},b_{i+1} = 1,0)$  \\
%             $P(b_i\, \neg\, \text{ flips})$ &  $P(b_i = 0\, |\, b_{i+1} = 0)$ & $H(b_{i})$ & $P(b_{i},b_{i+1} = 1,1)$ \\
%             $P(b_i\, \text{ flips}\, |\, b_{i+1}\, \neg \,\text{flips})$ & $P(b_{i+1} = 0\, |\, b_{i} = 0)$  \\
%             $P(b_i\, \neg \,\text{ flips}\, |\, b_{i+1}\, \text{flips})$ &   \\
%             $P(b_{i+1}\, \neg \,\text{ flips}\, |\, b_i\, \neg\, \text{ flips})$ & \\ \bottomrule
%         \end{tabular}
        
%     \end{threeparttable}
% \end{table*}



% From a known DBC and a matching CAN log, we create a binary vector for each ID $y^{id}\in \{0,1\}^{m_{id}-1}$ giving the labels for training/testing. 
% While this is straightforward for big endian signals, note that little endian signals have adjacent bits with non-adjacent indices at byte boundaries. 
% Using the example of Sec. \ref{sec:can-basics} for illustration, if the first two bytes are a little endian signal we have indices $8\rightarrow 0$.  
% Our features encode information of neighboring bits and must be extracted from ID traces before endianness is known. 
% Big endian and little endian entail different bit orderings at byte boundaries; consequently, during feature generation we do not know which bits to consider as  neighbors. 
% % non-adjacent bits are within-signal neighbors. % cannot during feature generation know which signals are little or big endian.  
% For the purpose of training/testing the machine learning model we split little endian signals on byte boundaries. 
% This is reconciled in ACTT 2.0's step 2 (Sec. \ref{sec:endianess_opt}), which considers neighboring bits from both little and big endian options at each byte when using this machine learning model as part of an optimization process that  extracts full little endian signals.  
% For evaluation against the signal boundary identification of previous methods, this means they are not penalized for assuming that all signals are big endian.  

% \begin{table}[ht]
% \small
%     \centering
%     \begin{threeparttable}[b]
%         \caption{Local Features}
%         \label{tb:features}
%         \begin{tabular*}{.48\textwidth}{ll}
%             %\addtolength{\tabcolsep}{-2pt}
%             \toprule
%             \textbf{Bit Values }  & \textbf{Bit Flips } \\
%             \midrule
%             $P(B_i = 0)$ & $P(B_i(t_j) \neq B_i(t_{j+1}))$\\
%             $P(B_i = 0 \mid B_{i+1} = 0)$ & $P(B_i(t_j) \neq B_i(t_{j+1}) \mid B_{i+1}(t_j) \neq B_{i+1}(t_{j+1}))$\\

%             $P(B_{i+1} = 0 \mid  B_i = 0)$ & $P(B_{i+1}(t_j) \neq B_{i+1}(t_{j+1}) \mid B_i(t_j) \neq B_i(t_{j+1}) )$\\
%             $P(B_i = 1 \mid  B_{i+1} = 1)$ & $P(B_i(t_j) = B_i(t_{j+1}) \mid B_{i+1}(t_j) = B_{i+1}(t_{j+1}))$\\
%             $P(B_{i+1} = 1 \mid  B_i = 1)$ & $P(B_{i+1}(t_j) = B_{i+1}(t+1) \mid B_i(t) = B_i(t_{j+1}))$\\
%             \midrule
%             \textbf{Benford}  & \textbf{Entropy} \\
%             \midrule
%             $P(B_i, B_{i+1} = 0, 0)$ &  $H(B_i)$ \\
%             $P(B_i, B_{i+1} = 1, 0)$ &  $H(B_i, B_{i+1})$ \\
%             $P(B_i, B_{i+1} = 0, 1)$ &  $H(B_i\dots B_{i+3})$ \\
%             $P(B_i, B_{i+1} = 1, 1)$ &  \\
%             \bottomrule
%         \end{tabular*}
        
%     \end{threeparttable}
% \end{table}



==> discussion.tex <==
 

  
\subsection{Discussion}
\label{sec:discussion}
\add{Discussion of results and comparisons}
This metric for error penalizes incorrectly classified signed signals more than little endian signals that have been incorrectly classified as multiple big endian signals. The reason for this is that for an incorrectly signed signal, when the signal takes on a negative value (for example -1), this will be very far from the value it takes if it is incorrectly classified as unsigned (max value). However, for little endian signals classified incorrectly as 2 big endian signals, the most significant byte signal will be paired with the 2 byte little endian signal, and once normalized, the $\ell_1$ error will be quite small since most of the information is encoded in the more significant byte. The lease significant byte on the other hand (which will just look like noise vacillating between the min and max value), will be paired with the 0 vector, and will have a medium sized error. Also note that the errors are not weighted by token weight, so while little endian signals are long (must be more than one byte), there are relatively few of them, so they have a somewhat small impact on the scores. 

For TANG, the reason it seems to do so poorly on cutting is because of the strict monotonically decreasing req on transition probabilities. It appears that the last couple LSBs of signals often seem to increase slightly, so it cuts preemptively. The high errors in signal difference can also be attributed to low precision since many additional short spurious signals will impact the score negatively.

For all other methods, the score is significantly worse for the two captures with Little Endian signals (5, 7). 

Note that log 3, whcih is the only one we lose on, has a lot of checksums.



Reminder: Write sentence or two indicating that the main way to push this forward would be to improve the signal boundary classification step. 
